On the Evolution of Knowledge Graphs: A Survey and Perspective

Knowledge graphs (KGs) are structured representations of diversified knowledge. They are widely used in various intelligent applications. In this article, we provide a comprehensive survey on the evolution of various types of knowledge graphs (i.e., static KGs, dynamic KGs, temporal KGs, and event KGs) and techniques for knowledge extraction and reasoning. Furthermore, we introduce the practical applications of different types of KGs, including a case study in financial analysis. Finally, we propose our perspective on the future directions of knowledge engineering, including the potential of combining the power of knowledge graphs and large language models (LLMs), and the evolution of knowledge extraction, reasoning, and representation.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/bak/sec1_intro.tex <==
\IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}
% % Computer Society journal (but not conference!) papers do something unusual
% % with the very first section heading (almost always called "Introduction").
% % They place it ABOVE the main text! IEEEtran.cls does not automatically do
% % this for you, but you can achieve this effect with the provided
% % \IEEEraisesectionheading{} command. Note the need to keep any \label that
% % is to refer to the section immediately after \section in the above as
% % \IEEEraisesectionheading puts \section within a raised box.
% % The very first letter is a 2 line initial drop letter followed
% % by the rest of the first word in caps (small caps for compsoc).
% % 
% % form to use if the first word consists of a single letter:
% % \IEEEPARstart{A}{demo} file is ....
% % 
% % form to use if you need the single drop letter followed by
% % normal text (unknown if ever used by the IEEE):
% % \IEEEPARstart{A}{}demo file is ....
% % 
% % Some journals put the first two words in caps:
% % \IEEEPARstart{T}{his demo} file is ....
% % 
% % Here we have the typical use of a "T" for an initial drop letter
% % and "HIS" in caps to complete the first word.
% \IEEEPARstart{T}{his} demo file is intended to serve as a ``starter file''
% for IEEE Computer Society journal papers produced under \LaTeX\ using
% IEEEtran.cls version 1.8b and later.
% % You must have at least 2 lines in the paragraph with the drop letter
% % (should never be an issue)
% I wish you the best of success.

% \hfill mds
 
% \hfill August 26, 2015






%### 引入：

% 简述知识图谱，知识推理相关概念

% ### 介绍我们的动机：

% 知识驱动型AI是AI技术未来的重要发展方向。由于现实世界的知识是不断变化的，如何学习表示变化的知识以及发掘知识的变化规律是AI领域的一大难题。顺应这种需求，知识图谱作为近年来新起的知识表示形式，逐渐地从静态知识图谱发展为动态知识图谱、时态知识图谱以及最新的事件知识图谱。相应地，基于知识图谱的知识推理技术也从静态的学习进化到了时态的学习。因此，我们需要从发展的角度，来回顾知识图谱的演变和应用于不同类型知识图谱的知识推理技术，并展望知识图谱和知识推理技术的未来发展方向以及潜在的应用价值。

% ### 贡献：

% - 一个developmental review关于知识图谱和知识图谱推理技术
% - 设想并定义了下一代知识图谱 - causal knowledge graph
% - new taxonomy-根据知识图谱类型来对相应的知识图谱推理技术进行分类（静态-动态-时态-因果），以及全方面的review
% - 总结和展望。causal knowledge graph和causal reasoning的应用前景

\IEEEPARstart{K}{nowledge} graph (KG) is a widely-used knowledge representation technology in artificial intelligence research. It can organize huge amounts of scattered data into structured knowledge. 
% Recent years, with the fast increment of the volume of Internet data, the demand for fast and accurate access to high-quality information is growing, which drives the birth and development of many large-scale KGs. 
Typical KGs including Google Knowledge Graph~\cite{googleKG}, DBpedia~\cite{dbpedia}, Freebase~\cite{freebase} and YAGO~\cite{YAGO}, have been widely used in a variety of intelligent applications, such as search engines~\cite{ehrlinger2016survey}, question answering systems~\cite{ji2020survey}, recommendation systems~\cite{survey1}, etc.

\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{img/fig_kgs.png}
	\caption{Examples of four categories of the knowledge graph, i.e., static, dynamic, temporal, and event knowledge graph.}
         % \vspace{-10pt}
	\label{fig:fig_kgs}
\end{figure}

\begin{figure*}[t]
	\centering
	\includegraphics[width=2\columnwidth]{img/fig_sub.png}
	\caption{General framework of the survey.}
         % \vspace{-10pt}
	\label{fig:fig_sub}
\end{figure*}

A Knowledge Graph (KG) is depicted as a graph where nodes represent entities that describing either real-world objects or abstract concepts, and edges denote relations that signifying semantic or logical connections between these entities.
Therefore, the basic building blocks of a KG are facts shaped like (\textit{subject entity}, \textit{relation}, \textit{object entity}), which are also known as triples ($e_s$, $r$, $e_o$).


Although the form of fact triples facilitates the representation of static knowledge, most real-world knowledge elements are always evolving or changing. Thus, static KGs (SKGs) where triples are never updated or updated very infrequently, are limited due to the timeliness of the knowledge they hold~\cite{ATiSE}. 
% To solve this problem, many dynamic KGs (DKGs) continuously collect new knowledge from the Internet or other data sources by manual or automated methods, and delete invalid triples and add new emerging entities, relations and triples to ensure the timeliness of knowledge. 
% Although DKGs guarantee the validness and timeliness of facts they store, it is difficult for users to query the historical facts occuring at a specific time over such KGs, e.g., "\textit{who have served as the president of the U.S. since 2000 ?}". Either static or dynamic KGs do not reflect the temporal characteristics of real-world knowledge very well. Thus, temporal KGs (TKGs) like ICEWS~\cite{ICEWS} and Wikidata~\cite{Wikidata} have drawn more and more interest recently. In TKGs, facts are represent as time-aware quadruples ($e_s$, $r$, $e_o$, $t$) where $t$ denotes the timestamp. 
To solve this problem, many dynamic KGs (DKGs) continuously collect and update knowledge to ensure the timeliness of knowledge. Moreover, temporal KGs (TKGs) such as ICEWS~\cite{ICEWS}, GDELT~\cite{GDELT}, YAGO3~\cite{YAGO3} and Wikidata~\cite{Wikidata} which attach time information into triple facts have drawn more and more interest recently.
Besides entity-centric knowledge, events are also an essential kind of knowledge in the world, which trigger the spring up of event-centric knowledge representation form such as Event KG (EKG)~\cite{event-centric}. Noteworthy, events are dynamic and temporal in nature and relations between events and facts are often temporal or causal ones. The four different categories of KG are shown in Figure~\ref{fig:fig_kgs}.

A vast amount of knowledge exists in unstructured data sources.
Knowledge extraction (KGE), which focuses on automatically extracting structured information from unstructured data, is one of the key technologies of knowledge graph construction. Knowledge extraction for different types of KGs involves various NLP techniques, including named entity recognition (NER)~\cite{ner_}, relation extraction~\cite{REsurvey1}, event extraction and rule extraction.
These knowledge extraction techniques developed rapidly in recent years with the rise of large language models (LLMs), and they are extensively reviewed in this paper.

In addition, most KGs reviewed in this paper are suffering from the problem of incompleteness, and it severely limits the metric of KG application to downstream tasks. Thus, KG reasoning (KGR), a task that aims to predict and complete missing facts in KGs, has become one of the research hot spots in KG studies. With the development of KGs, KGR techniques have also evolved from static learning methods to temporal learning methods. According to the types of target KGs, we classify the existing KGR methods into three categories, i.e., static KGR (SKGR) methods, dynamic KGR (DKGR) methods and temporal KGR (TKGR) methods. We will discuss event KGR (EKGR) as a part of future work in this paper, since this task needs more research in the future. 

% Moreover, LLMs are also widely used in knowledge reasoning tasks. One view on this is that pre-trained language models are themselves large knowledge bases. The popularity of ChatGPT~\footnote{https://openai.com/blog/chatgpt} has further prompted some thoughts from the KG community: 1. what are the similarities and differences between KGs and LLMs in processing and organizing knowledge?; 2. how can KGs be combined with generative LLMs such as ChatGPT? These two questions will be discussed in this paper.

Although there are several survey papers focusing on knowledge graphs and the relevant techniques of knowledge extraction and KGR, they each only focus on technologies related to a single type of KGs and thus do not study the difference and connection between the types of their target KGs.  
The goal of this survey is to provide a comprehensive and up-to-date overview of KGs from an evolving perspective (i.e., SKG$\rightarrow$DKG$\rightarrow$TKG$\rightarrow$EKG), and highlight promising future research directions. Our contributions can be summarized as follows:

\begin{itemize}
    \item \textbf{Comprehensive Review.} We study the various KGs from an evolution perspective, and provide a comprehensive review of knowledge extraction and reasoning techniques for different types of KGs. 
    \item \textbf{New perspectives and insights on future direction.} We introduce our perspectives in the future directions of knowledge engineering, especially the connection to LLMs.%大语言模型对KG技术的影响，基于因果关系的知识图谱推理，新技术在金融和医疗等领域的应用. 
\end{itemize}

The article is organized and shown in Figure~\ref{fig:fig_sub}.
Sec.~\ref{sec:introduction} introduces the formal evolution of KGs, as well as relevant definitions and notations; Sec.~\ref{sec:3} and Sec.~\ref{sec:4} review the knowledge extraction and reasoning techniques applied to different types of KGs; Sec.~\ref{sec:5} illustrates a case study of KGs in financial analysis and other applications;
% Sec.~\ref{sec:6} illustrates the applications of KGs through a case analysis of financial KGs;
Sec.~\ref{sec:6} discusses future research directions about knowledge engineering.
% and conclude the paper in Sec.~\ref{sec:7}.






==> sections/bak/sec2_background.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.7\columnwidth]{img/kg_evo.pdf}
	\caption{The formal evolution history of KGs.}
         % \vspace{-10pt}
	\label{fig:kg_evo}
\end{figure*}

\section{Evolution of Knowledge Graphs}\label{sec:preliminary}
The development of knowledge graphs can be traced back to the birth of expert systems in the last century. After that, the concept of knowledge graphs was gradually formed after the development of the World Wide Web 1.0 era and the Semantic Web. Starting in 2006, the emergence
of large-scale Wikipedia-like rich-structure knowledge resources and advances in web-scale information
extraction methods have led to tremendous progress in knowledge extraction methods, which are automated and operated at the web-scale. Currently, automatically-built KGs have become powerful assets for semantic search, big data analysis, intelligent recommendations, and data integration, and are being widely used in large industries and various domains.

Early KGs were mainly used to store static knowledge. As the increasing demand of downstream tasks to the timeliness of knowledge, KGs that can continuously update knowledge or store time information of facts have emerged. Nevertheless, entity-centric KGs are still unable to elegantly represent the event information that appears in news texts. Thus, event-centric KGs have been proposed, and become popular in specific domains, such as finance and tourism.

Based on this observation, we divide the formal evolution of KGs into four stages, corresponding to the emergence of static KGs (SKGs), dynamic KGs (DKGs), the temporal KGs (KGs) stage, and event KGs (EKGs), respectively. In this section, we first summarize the notation as shown in Table~\ref{table:notation}, then we will provide definitions of the four types of KGs, and their typical representatives, as well as their application scenarios.

\begin{table}
\centering
\caption{Overview of Knowledge Graph Reasoning Methods}
\label{table:notation}
\begin{tabular}{cc}
\toprule
Notation & Explanation \\
\midrule
$\mathcal{SKG}$ & Static knowledge graph\\
$\mathcal{DKG}$ & Dynamic knowledge graph\\
$\mathcal{TKG}$ & Temporal knowledge graph \\
$\mathcal{EKG}$ & Event knowledge graph \\
$\mathcal{E}_n$ & Entity set\\
$\mathcal{E}_v$ & Event set\\
$\mathcal{R}$ & Relation set\\
$\mathcal{F}$ & The set of facts\\
$\mathcal{T}$ & The set of the time stamps\\
$\mathcal{F}_t$ & The set of facts at time $t$ \\
$\left(e_s, r_p, e_o\right)$ & Fact of the head, relation, tail.\\
$\left(e_s, r_p, e_o, t\right)$ & Fact of the head, relation, tail, timestamp\\
% $\left(e_s^q, r_p^q, e_o^q\right)$ & Queried fact of head, relation, tail\\
% $\left(e_s^q, r_p^q, e_o^q, t^q\right)$ & Queried fact of head, relation, tail, timestamp\\
% $\mathbf{h}$ & Embedding of head entity\\
% $\mathbf{r}$ & Embedding of relation\\
% $\mathbf{t}$ & Embedding of tail entity\\
\bottomrule
\end{tabular}
\end{table}


\subsection{Static Knowledge Graphs}
The first generation of KGs is static graphical representations that present knowledge in the form of entities and relations between entities, as shown in Figure~\ref{fig:fig_skg}. The formal definition is declared as follows,
\par\smallskip

\noindent\textbf{Definition 1. Static Knowledge Graph.}
~\textit{
A Static Knowledge Graph is defined as $\mathcal{SKG}=\{\mathcal{E}_{n},\mathcal{R},\mathcal{F}\}$, where $\mathcal{E}_{n}$ and $\mathcal{R}$ represent the sets of entities and relations, respectively. $\mathcal{F}\subseteq\mathcal{E}_{n}\times\mathcal{R}\times\mathcal{E}_{n}$ is a set of facts $\{(e_{s},r_{p},e_{o})\}$, where $e_{s}, e_{o}\in\mathcal{E}_{n}$ and $r_{p}\in\mathcal{R}$. A fact ${(e_{s},r_{p},e_{o})}$ represents that relation $r_p$ exists between subject entity $e_s$ and object entity $e_{o}$ at some unspecified time.
}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\columnwidth]{img/fig_skg.png}
	\caption{Examples of a static knowledge graph.}
         % \vspace{-10pt}
	\label{fig:fig_skg}
\end{figure}

A few examples of SKGs include Kinship~\cite{kinship}, HowNet~\cite{dong2003hownet}, WordNet~\cite{wordnet}, and Freebase~\cite{freebase}. 
Kinship database is a small-size relational database, consisting of 24 unique names in two families. HowNet is a semantic knowledge base, designed to capture the meaning of words and concepts in Chinese. These two KGs are static representations of relationships between specific entities and concepts, and are not updated after their creation.
WordNet is a lexical database of English words and concepts, which includes synonyms and hypernyms. 
%Cyc contains a large amonut of common-sense knowledge. 
Freebase was designed to be an open and shared repository of structured data about a wide range of topics, including people, places, organizations, and more. Since they have no longer been updated for a long time, it can be regarded as SKGs.

SKGs are useful for many applications, such as information retrieval and question answering, where a fixed set of relations between entities is required. However, they are not suitable for applications that require up-to-date information, such as news articles or social media feeds.


\subsection{Dynamic Knowledge Graphs}
The second generation of KGs introduced the concept of change and updates to the graph, guaranteeing the timeliness of knowledge and enabling the extensibility of the graph, as shown in Figure~\ref{fig:fig_dkg}. The formal definition is declared as follows,
\par\smallskip

\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\columnwidth]{img/fig_dkg.png}
	\caption{Examples of a dynamic knowledge graph.}
         % \vspace{-10pt}
	\label{fig:fig_dkg}
\end{figure}

\noindent\textbf{Definition 2. Dynamic Knowledge Graph.}
~\textit{
A Dynamic Knowledge Graph is defined as $\mathcal{DKG}=\{\mathcal{E}_{n},\mathcal{R},\mathcal{F}\}$, where $\mathcal{E}_{n}$ and $\mathcal{R}$ represent the dynamic sets of entities and relations, respectively. $\mathcal{F}\subseteq\mathcal{E}_{n}\times\mathcal{R}\times\mathcal{E}_{n}$ is a dynamic set of facts $\{(e_{s},r_{p},e_{o})\}$, where $e_{s}, e_{o}\in\mathcal{E}_{n}$ and $r_{p}\in\mathcal{R}$. A fact ${(e_{s},r_{p},e_{o})}$ represents that relation $r_p$ exists between subject entity $e_s$ and object entity $e_{o}$ at the time of the latest update.
}

Most KGs are dynamic and evolving. For example, DBpedia~\cite{dbpedia} is a DKG that is created by extracting structured data from Wikipedia~\cite{wikipedia}. It is updated regularly to reflect changes in Wikipedia. Similarly, many large-scale KGs like Google Knowledge Graph~\cite{googleKG}, NELL~\cite{nell}, Linked Open Data~\cite{LinkedOpenData}, OpenCyc~\cite{Opencyc}, ConceptNet~\cite{conceptnet} and UMLS~\cite{UMLS}, continuously updated over time, even in real-time, to reflect changes in the underlying data. These graphs are designed to be more flexible and adaptable than SKGs, allowing them to better handle data that is constantly changing and evolving. It is worth noting that a separate version of a DKG can be viewed as an SKG. And a DKG that is no longer updated will also degenerate into an SKG. Therefore, an SKG can be viewed as a special case of a DKG, i.e., \textbf{Definition 2} subsumes \textbf{Definition 1}.

DKGs are being used in various applications, including search engines, recommendation systems, chatbots, and more. By continuously updating the KGs with the latest data, these systems can provide more accurate and relevant results to users. However, DKGs can not be applied in some applications such as historical analysis, trend analysis and forecasting, due to the loss of historical data. 


\subsection{Temporal Knowledge Graphs}
The third generation of KGs adds a temporal dimension to the knowledge, allowing for the representation of time-varying relations between entities. The temporal knowledge graphs are designed to capture and represent knowledge that changes over time, and tend to be dynamic in nature with their time-sensitivity, as shown in Figure~\ref{fig:fig_tkg}. The formal definition is declared as follows,
\par\smallskip

\noindent\textbf{Definition 3. Temporal Knowledge Graph.}
~\textit{
A Temporal Knowledge Graph is defined as $\mathcal{TKG}=\{\mathcal{E}_{n},\mathcal{R},\mathcal{T},\mathcal{F}\}$, where $\mathcal{E}_{n}$, $\mathcal{R}$ and $\mathcal{T}$ represent the extendable sets of entities, relations and timestamps, respectively. $\mathcal{F}\subseteq\mathcal{E}_{n}\times\mathcal{R}\times\mathcal{E}_{n}\times\mathcal{T}$ is an extendable set of facts $\{(e_{s},r_{p},e_{o},t)\}$, where $e_{s}, e_{o}\in\mathcal{E}_{n}$, $r_{p}\in\mathcal{R}$ and $t\in\mathcal{T}$. A fact ${(e_{s},r_{p},e_{o},t)}$ represents that relation $r_p$ exists between subject entity $e_s$ and object entity $e_{o}$ at time $t$. $t$ is sometimes unknown and can be represented in different forms, e.g., time points or time intervals.
}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.9\columnwidth]{img/fig_tkg.png}
	\caption{Examples of a temporal knowledge graph.}
         % \vspace{-10pt}
	\label{fig:fig_tkg}
\end{figure}

SKGs and DKGs represent facts in the form of triples, shaped like (\textit{Donald Trump}, \textit{president of}, \textit{USA}). The time spans when facts hold are unknown. Thus, one can not use SKGs or DKGs to tackle time-sensitive tasks, like time-aware link prediction, forecasting and others. A lot of large-scale TKGs like Wikidata~\cite{Wikidata}, YAGO~\cite{YAGO3} associate fact triples with valid time
annotations.
Some event databases, e.g., ICEWS~\cite{ICEWS} and GDELT~\cite{GDELT} can also be taken as TKGs since they decompose event news into fact quadruples and store them. Such TKGs provide rich temporal information, but not every fact in a TKG includes a time stamp. Thus, DKGs can be regarded as special cases of TKGs, where all-time information is unobtainable. In another words, \textbf{Definition 3} subsumes \textbf{Definition 2}.

Overall, TKGs offer a more comprehensive view of data over time, which is useful for a wide range of applications, including temporal query answering, and predictive analysis. On the other hand, some TKGs are extracted from event news, but do not effectively represent event information due to their entity-centric representations.

\subsection{Event Knowledge Graphs}
The most recent generation of KGs focuses on representing and understanding events, which are time-bound occurrences that involve multiple entities and relations, enabling the representation of complex, time-varying relations between entities and events, as shown in Figure~\ref{fig:fig_ekg}. The formal definition is declared as follows,
\par\smallskip

\noindent\textbf{Definition 4. Event Knowledge Graph.}
~\textit{
An Event Knowledge Graph is defined as $\mathcal{EKG}=\{\mathcal{E},\mathcal{R},\mathcal{T},\mathcal{F}\}$. $\mathcal{E}=\mathcal{E}_{n}\cup\mathcal{E}_{v}$ is the node set, where $\mathcal{E}_{v}$ is an extendable event set. $\mathcal{R}$ represents the sets of relations between entities and events. $\mathcal{F}\subseteq\mathcal{E}\times\mathcal{R}\times\mathcal{E}\times\mathcal{T}$ is an extendable set of facts $\{(e_{s},r_{p},e_{o},t)\}$, where $e_{s}, e_{o}\in\mathcal{E}$ and $r_{p}\in\mathcal{R}$. A fact $\{(e_{s},r_{p},e_{o},t)\}$ represents that relation $r$ exists between subject node $e_s$ and object node $e_{o}$ at time $t$. $t$ is sometimes unknown and can be represented in different forms. $r$ can be an entity-entity relation $r_{en\mbox{-}en}\in\mathcal{R}_{en\mbox{-}en}$, or an event-event relation $r_{ev\mbox{-}ev}\in\mathcal{R}_{ev\mbox{-}ev}$, or a relation $r_{en\mbox{-}ev}\in\mathcal{R}_{en\mbox{-}ev}$ between an entity and an event, where $\mathcal{R}=\mathcal{R}_{en\mbox{-}en}\cup\mathcal{R}_{ev\mbox{-}ev}\cup\mathcal{R}_{en\mbox{-}ev}$.
}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\columnwidth]{img/fig_ekg.png}
	\caption{Examples of an event knowledge graph.}
         % \vspace{-10pt}
	\label{fig:fig_ekg}
\end{figure}

EEG~\cite{eeg} is an EKG, where event nodes are abstract, generalized and semantically complete verb phrases and edges represent temporal and causal relationships between them.  EventKG~\cite{eventkg} is a multilingual event-centric TKG that aggregates event-centric information and temporal relations for historical and contemporary events. ELG~\cite{elg} is an EKG, which mainly focuses on schema-level event knowledge. Besides, EvGraph~\cite{event-centric} is an automatical construction pipeline that structures news stories into EKGs. Compared with TKGs, EKGs contain one more node type (i.e., event nodes) and two more relation types (entity-event relations, event-event relations). Thus, \textbf{Definition 4} subsumes \textbf{Definition 3}.

Basic applications on EKG include script event prediction, timeline generation and inductive reasoning~\cite{eventkg_review}. Furthermore, EKG can facilitate downstream event-related applications such as financial quantitative investments and text generation.

==> sections/bak/sec3.1_NER_RE.tex <==
\section{Knowledge Extraction}\label{sec:3}
The construction of different types of KGs relies on various knowledge extraction techniques. The construction of SKGs requires factual triples extracted from text. Therefore, their knowledge extraction processes mainly include named entity recognition (NER) and relation extraction (RE). Meanwhile, the construction of DKGs requires dynamic knowledge extraction from the ever-changing real-world information.
The construction of TKGs and EKGs additionally requires event extraction to obtain the corresponding temporal and event information. Besides, logical rules between relations in KGs can be regarded as a special kind of knowledge in addition to factual knowledge and rule discovery over different types of KGs requires different rule extraction techniques. With the rise of large language models (LLMs) and their strong natural language understanding capabilities, LLMs are widely used in various knowledge extraction tasks. In this section, we will review the above-mentioned knowledge extraction techniques and the applications of LLMs in these techniques respectively.

\begin{figure*}[t]
	\centering
	\includegraphics[width=1.8\columnwidth]{img/sx/sx-LLM.pdf}
	\caption{Comparison of LMs. (a) Representative models are word2vec~\cite{wordembed1} and GloVe~\cite{glove}. These models pretrain word embeddings in some corpus and output a vocabulary list. People get specific word embeddings by looking up in the table. As the embeddings are pre-trained and fixed, they are static. (b) The representative model is BERT~\cite{bert}. BERT utilizes a Transformer Encoder to extract features of tokens in the input sequence and output word representations. It is contextualized because the context information can be captured thanks to the bi-directional settings. BERT is typically used for discriminative tasks such as text classification and named entity recognition. (c) Representative models are GPT~\cite{GPT} and BART~\cite{BART}. These models are fed a sequence and output a sequence. They often employ Transformer decoder blocks for generative tasks like text generation and machine translation. They can capture contextualized information, but only preceding context information if a decoder block is used.}
         % \vspace{-10pt}
	\label{fig:fig_LLM}
\end{figure*}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.95\columnwidth]{img/sx/sx-NER.png}
	\caption{Discriminative and generative NER methods. Discriminative models try to tag the tokens by classification and combine the taggers to recognize entities, while generative models focus on generating a new sequence with additional token markers.}
         % \vspace{-10pt}
	\label{fig:fig_NER}
\end{figure}

\subsection{Named Entity Recognition}\label{sec:3.1}
%介绍NER概念,NER任务流程以及传统方法（CRF，PointerNetwork）以及深度学习方法BiLSTM-based or CNN-based
Named Entity Recognition is a task that extracts entities from text. The extracted types of entities usually cover CARDINAL, ORDINAL and DATE to PERSON, ORG(organization) and LOC(location). In the past, sequence tagging methods were often adopted to tag each token in the text by BIO or BIOES tagging system, such as CRF~\cite{CRF} or Pointer Network~\cite{PointerNetwork}, and then, entities were generated by the combination of taggers. With the development of deep learning, more and more deep neural network (DNN) based models are proposed. 

In general, there are two kinds of DNN-based models, RNN and CNN-based models, some of which are followed by a CRF layer. For instance, Andrej et al.~\cite{BiLSTM_NER} provide a Bi-LSTM model using multiple independent Bi-LSTMs to provide diversity. Experiments on the CoNLL 2003 NER dataset prove the sufficiently good performance. Moreover, Emma et al.~\cite{CNN_based_NER} propose ID-CNNs, employing fixed-depth convolutions for parallelism to conduct NER tasks. Results show that ID-CNNs achieve higher accuracy with 8x faster test time speeds. These DNN-based models try to identify patterns related to the named entities and predict the presence of these patterns.

% LM-based methods进行 NER 的流程，引出下面阐述LM-based methods的方法分类：static embedding and contextual embedding
Recently, language models (LM) have attracted much attention for natural language processing tasks. In general, LM can be divided into discriminative models and generative models, where the former aims to predict the probability of a word and classification, while the latter focuses on generating a new sequence. Moreover, according to the types of embeddings, models can be classified into static embeddings-based methods and contextualized embeddings-based methods (As Figure~\ref{fig:fig_LLM} shows). Recently, researchers have focused on accomplishing NER tasks based on these language models. Discriminative models try to tag and classify entities while generative models generate a new sequence with additional token markers (As Figure~\ref{fig:fig_NER} shows).
%基于语言模型static embeddings(static, token-level,  fail to capture context) GloVe, word2vec, Fasttext

\subsubsection{Static and discriminative LM-based Method}
Ever since the inception of word2vec~\cite{wordembed1} in 2013, a plethora of subsequent word representation techniques have been introduced. Prominent among these are GloVe~\cite{glove} and fastText~\cite{fasttext1}. These methods are proficient in generating compact word vectors, thereby serving as distributed word representations. Within the domain of Named Entity Recognition (NER), these embeddings typically find their application as inputs to decoding mechanisms, such as Conditional Random Fields (CRF) or Pointer Networks.

Through the utilization of a variety of distributed word representations, numerous scholars undertake the reevaluation of Named Entity Recognition (NER) tasks. To illustrate, Nguyen et al.\cite{word2vec_NER} employ word2vec embeddings refined through the training of a vast corpus comprising 100 billion words from the Google News corpus. This strategic selection aims to assess the resilience of Recurrent Neural Network (RNN)-based mention detection algorithms. In contrast, Ma et al.\cite{glove_NER} harness 100-dimensional GloVe embeddings meticulously derived from Wikipedia and web corpora, effectively integrating them with two additional established embeddings. Their conscientious endeavors culminate in achieving preeminent outcomes on the CoNLL 2003 dataset, showcasing an impressive precision rate of 91.21\%. Diverging from these approaches, Li et al.\cite{glove_NER2} propose a novel paradigm, the BNN-CNN model, which generates word embeddings through the fusion of GloVe-initialized embeddings and supplementary embeddings tailored to capture morphological insights. By employing these advanced embeddings as input, their model outperforms competing models on the OntoNotes 5.0 dataset. Furthermore, the model designed by Wang et al.\cite{fasttext_NER} incorporates fastText embeddings trained on expansive corpora such as Common Crawl and Wikipedia, subsequently achieving a top-ranking position in the MS Arabic-Egyptian NER task.

Owing to the efficacy of the adept embeddings, the aforementioned methods exhibit superior performance compared to conventional approaches reliant on rudimentary features. Nonetheless, it is imperative to acknowledge that the aforementioned embeddings remain static in nature. This signifies that the words are trained within pre-established corpora, with a fixed vocabulary inventory. Consequently, the word embeddings encompassed within this catalog are unable to encapsulate contextual nuances pertinent to distinct textual contexts within alternate NER tasks. Thus, to address this limitation, certain techniques grounded in contextualized LM embeddings have been introduced.

%基于语言模型的上下文embedding
\subsubsection{Contextualized and discriminative LM-based Method}
%Approaches based on character-level LM embeddings: Flair
%Approaches based on word-level LM embeddings: ELMo,Bert
Diverging from their static counterparts, contextualized LM embeddings possess the ability to encompass contextual information. Broadly speaking, these contextualized LM embeddings can be bifurcated into two distinct categories: character-level and word-level contextualized LM embeddings. Character-level contextualized LM embeddings, exemplified by Flair~\cite{flair}, endeavor to decipher the distinctive attributes characterizing the distribution across characters. Conversely, word-level contextualized LM embeddings adopt a holistic approach, treating individual words as cohesive units rather than deconstructing them into constituent characters. Illustrative instances of word-level contextualized LM embeddings include ELMo~\cite{ELMO} and BERT~\cite{bert}.

For character-level LM embeddings in NER tasks, an approach is proposed by Alan et al.~\cite{flair}, who utilize Flair embeddings to represent distributions over characters and achieve the state-of-the-art performance on four NER tasks on the CoNLL03 dataset. 
Furthermore, certain investigations are geared towards embedding individual words, enriched with their contextual nuances, into cohesive vectors. For instance, Li et al.~\cite{bert_NER} leverage BERT embeddings across diverse NER tasks and datasets. The empirical findings affirm the commendable efficacy of BERT embeddings in yielding favorable outcomes. Diverging from BERT's utilization of bidirectional Transformer models, ELMo capitalizes on bidirectional LSTM models to engender contextualized word embeddings. In this context, Xia et al.~\cite{elmo_ner} harness ELMo embeddings as integral components of entity features, shaping the foundation for conducting NER tasks within a classification framework. Empirical experimentation underscores the potency of their model, yielding a notable enhancement of 4.4\% in F1 scores across non-overlapping NER tasks.

In summation, these contextualized embeddings adeptly integrate contextual information at both character and word levels. Despite their resource-intensive demands in terms of computation, training data, and time, they consistently exhibit impressive performance across diverse forms of entity recognition tasks. Beyond these discriminative models, an additional avenue explored within the ambit of NER tasks involves the introduction of generative language models.

\subsubsection{Contextualized and generative LM-based Method}
A generative language model represents an approach capable of generating coherent new text content rooted in a given input, often referred to as a prompt. This method operates by acquiring an understanding of the probability distribution inherent in historical texts, enabling it to predict the likelihood of forthcoming words. In recent times, an increasing number of influential generative language models have been unveiled, including GPT~\cite{GPT} and BART~\cite{BART}.

Generative language models commonly transform the Named Entity Recognition (NER) task into a sequential-to-sequential generative endeavor. In this approach, an input sequence is provided, and the model generates an output sequence that includes identified entities along with their corresponding entity types. Recent developments have introduced NER methods grounded in generative language models~\cite{ANL_NER, TANL, deepstruct, UGF_NER}. For instance, Ben et al.~\cite{ANL_NER} introduce a generative framework wherein the model produces an augmented sequence, not only reiterating the input sentence but also incorporating supplementary markers for token spans. Building upon this foundation, Paolini et al.~\cite{TANL} propose an innovative framework, Translation between Augmented Natural Languages (TANL). Diverging from prior work, they employ dynamic programming for the alignment of entities in the output and the original text, thus augmenting the resilience of the generation process. Similarly, Wang et al.~\cite{deepstruct} also regard NER as a task within the broader spectrum of structure prediction. They present DeepStruct, a pre-trained language model designed to generate structures from text, encompassing entities embedded within the text. Furthermore, Yan et al.~\cite{UGF_NER} endeavor to unify various NER subtasks within a generative framework. Here, they employ BART in an encoder-decoder architecture to generate the token indices within the sequence. In summary, these NER methodologies harness generative models to create alternative sequences encompassing the anticipated entities. While these approaches leverage the adept generative capabilities of the models, it is essential to enhance the robustness and precision of the generation process to avert the extraction of erroneous entities.

In summary, entities within natural language text can be effectively recognized through the utilization of the aforementioned deep learning methodologies. Beyond conventional Convolutional Neural Networks (CNN) or Recurrent Neural Networks (RNN), an array of language models presents viable alternatives. These models can be further categorized into three domains: those relying on static embeddings, those grounded in contextualized embeddings, and those stemming from generative language models. Broadly speaking, the models based on Deep Neural Networks (DNN) and either static or contextualized LM embeddings fall under the category of discriminative models. These models commonly discern entities through sequence labeling mechanisms. In contrast, generative models approach NER tasks as endeavors in sequence generation. Discriminative models generally exhibit a propensity for yielding superior, more accurate outcomes. However, they necessitate substantial volumes of labeled data. On the other hand, generative models present a contrasting advantage—they demand fewer labeled samples. Nevertheless, it is imperative to remain vigilant regarding the potential pitfalls of erroneous generation outcomes.

\subsection{Relation Extraction}\label{sec:3.2}
%该段介绍RE的定义和分类，包括Pipeline和Joint。
Relation Extraction (RE) encompasses the endeavor of identifying connections between entities within textual content. Generally, methods geared toward relation extraction can be classified into two distinct categories based on their interplay with Named Entity Recognition (NER) tasks. These categories are commonly known as the pipeline approach and joint extraction.

The pipeline approach involves a sequential progression wherein entities are initially recognized, followed by the extraction of relations linking them. In this scenario, the two tasks remain mutually independent. Here, relation extraction is often referred to as relation classification, focusing on determining the specific relationships between entities. In contrast, the joint extraction approach seeks to amalgamate these two tasks. The objective is to concurrently tackle both entity recognition and relation extraction, ultimately generating a comprehensive list of triples that encapsulate the entities along with their corresponding relationships.


\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{img/sx/sx-RE.png}
	\caption{Pipeline-based and Joint-based RE methods. Pipeline-based RE first recognizes the pair of entities in the text and then classify the relation between them. Joint-based RE try to find the triple in the text jointly. Typically, the total loss is composed of the losses of recognizing subject, object, and relation.}
         % \vspace{-10pt}
	\label{fig:fig_RE}
\end{figure}

\subsubsection{Pipeline-based Method}
%Pipeline(实际就是关系分类)：
%传统基于DNN的RE，远程监督RE（PCNN…）一嘴带过
%基于LM的模型

In the pipeline approach, traditional methods can be categorized into two main classes: feature-based and kernel-based methods. Within these classes, the task of relation extraction is often treated as a multi-class classification challenge. For instance, Rink et al.~\cite{RE_featurebased} combine lexical and semantic features for relation classification, employing these features as inputs to SVM classifiers. This effort yields an F1 score of 82.19\% and an accuracy of 77.92\%. Conversely, Tazvan et al.~\cite{RE_kernelbased} propose a kernel-based approach utilizing three distinct subsequence patterns. Experimental results across two corpora affirm the efficacy of their method. Both feature-based and kernel-based strategies aim to derive representations for entity pairs, subsequently employing classifiers to discern relationships.

With the ascendancy of deep learning, the application of deep neural networks for relation classification has gained traction, diminishing the reliance on intricate feature engineering. Zeng et al.~\cite{RE_NNbased} leverage convolutional deep neural networks to extract features at the lexical and sentence levels, achieving superior performance compared to traditional methods. Addressing the scarcity of labeled relational data, distant supervision techniques have been proposed to generate training data leveraging existing knowledge bases. For instance, Zeng et al.~\cite{distant} introduce a model involving piecewise convolutional neural networks (PCNNs) coupled with multi-instance learning (MIL), addressing data scarcity and mitigating the complexity of feature engineering.

More recently, relation extraction driven by language models has garnered considerable attention. For instance, Wu et al.~\cite{RE_bert} harness the pre-trained BERT model, augmenting it with entity information to excel in RE tasks. Wu et al.~\cite{RE_TRE} introduce TRE, leveraging pre-trained representations and self-attentive architecture to achieve state-of-the-art results on publicly available relational datasets. Soares et al.~\cite{RE_match} harness task-agnostic relation representations from deep Transformers, emphasizing that models initialized with their defined representations and tuned on relational datasets yield superior outcomes. Generative language models also hold a pivotal role in relation extraction. For instance, Cobot et al.~\cite{REBEL} propose REBEL, a BART-based model capable of end-to-end extraction of over 200 relation types. Additionally, Zeng et al.~\cite{copyRLL} introduce copyRLL, integrating reinforcement learning into a seq-to-seq model to account for the extraction order. Experiments on publicly available datasets attest to the efficacy of copyRLL.

In essence, these relation extraction methods following the pipeline approach are centered around a classification task, given the availability of entities and a predefined set of relations. Various methods are designed to enhance the precision and effectiveness of this classification endeavor. However, some scholars posit that pipeline methods might propagate errors from both phases. As a result, certain methods aim to jointly extract entities and relations, producing triples simultaneously.


\subsubsection{Joint-based Method}
%Joint：
%传统方法：传统基于深度学习的方法
In the context of joint extraction, it is discernible that the approaches can be categorized into two primary types: those predicated on deep learning (non-language models) and those rooted in language models. Among the deep learning-based methods, the prevalent strategy involves the utilization of models such as Recurrent Neural Networks (RNN), with parameters shared across both Named Entity Recognition (NER) and Relation Extraction (RE) tasks. For instance, Miwa et al.~\cite{RE_LSTM_RNN} introduce an LSTM-RNN model capable of jointly extracting entities and relations, leveraging parameter sharing. Their approach yields performance improvements on ACE2005 and ACE2004 datasets when compared to other end-to-end extraction methods. In a similar vein, Katiyar et al.~\cite{RE_joint_LSTM} present an LSTM model enriched with attention mechanisms. The resulting model surpasses the end-to-end SPTree model, demonstrating an advantage due to the absence of dependency trees. Experiments conducted on the ACE dataset substantiate the efficacy of their model in entity and relation extraction. In a departure from the extract-then-classify paradigm prevalent in prior joint extraction methods, Yu et al.~\cite{RE_Joint_NDS} propose an alternative that decomposes joint extraction into two interrelated subtasks and subsequently transforms these subtasks into sequence labeling problems. Their rationale stems from concerns regarding the lack of interaction awareness and redundant entities in previous extract-then-classify approaches. Their method attains state-of-the-art performance across three relational datasets.

%LM-based models
In the realm of LM-based joint extraction, it is commonplace to employ pre-trained models as encoders for generating representations. For instance, Wei et al.~\cite{RE_joint_CASREL} leverage a BERT-based encoder, integrating subject and relation object tagging for the extraction of relational triples. Their approach surpasses baselines by a substantial margin of 17.5 and 30.2 absolute F1 score values on NYT and WebNLG datasets. Furthermore, Eberts et al.~\cite{SpERT} introduce SpERT, an attention model geared towards reasoning over BERT embeddings. Ablation studies affirm the advantageous impact of pre-training. Moreover, Sui et al.~\cite{RE_joint_SetPredictionNetworks} underscore the notion of simultaneously outputting triples, driven by their belief that relational triples within a sentence lack a specific order. They employ BERT as a sentence encoder and channel-generated embeddings through a multi-head inter-attention module, ultimately accomplishing the set prediction task. Empirical evaluations on two datasets affirm the prowess of their approach. Furthermore, generative language models have found applicability in joint extraction. For instance, Nayak et al.~\cite{CGT} introduce a contrastive triple extraction technique harnessed with generative transformers, mitigating concerns over long-term dependencies and erroneous generation. Their method yields enhanced results across three public datasets. Huang et al.~\cite{TEMPGEN} frame RE as a template generation challenge and incorporate a cross-attention copy mechanism. Experimental findings across two datasets substantiate their claim to state-of-the-art outcomes. In summary, joint extraction methods excel at simultaneously extracting entities and relations, harnessing the potential for information and interaction amplification between entities and relations to augment performance. Nevertheless, they must be cautiously employed, as there exists the possibility of error propagation.

\subsection{Dynamic Knowledge Extraction}\label{sec:sec3.5}
% Added by SX

The aforementioned methods predominantly target the extraction of information or knowledge from static datasets. Nonetheless, in the dynamic realm of the real world, information is subject to constant change. Consequently, devising strategies for extracting information in an online and dynamic fashion assumes paramount importance. Researchers consistently grapple with the challenge of automatically and continuously acquiring knowledge from open information sources. Figure~\ref{fig:fig_DKE} shows an example of dynamic knowledge extraction and completion of knowledge graphs.

\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{img/sx/sx-DKE.png}
	\caption{An example of dynamic knowledge extraction. By NER and RE, triples are extracted from all kinds of open information, and knowledge graph is dynamically updated by these new facts and entities.}
         % \vspace{-10pt}
	\label{fig:fig_DKE}
\end{figure}

Broadly, there exist two categories of methods addressing the challenge of dynamic knowledge extraction: automatic extraction and never-ending learning. In the realm of automatic extraction, Etzioni et al.~\cite{knowitall} present "KnownItAll," a system designed to autonomously extract facts from web text. Over the course of four days, the system successfully accumulated a total of 54,753 facts. Furthermore, Schemitz et al.~\cite{ollie} introduce "Ollie" for open information extraction. Ollie addresses two limitations in prior efforts: the extraction of relations limited to verbs and the disregard for the context of extracted relations. Empirical results showcase the elevated AUC scores achieved by Ollie. Xin et al.~\cite{knowledge-vault} introduce "Knowledge Vault," a framework for the automatic generation of knowledge graphs by amalgamating information extracted from web content with pre-existing knowledge from established knowledge bases. In the context of never-ending learning, Carlson et al.~\cite{Carlson_NELL} propose the "Never-Ending Language Learner" (NELL) to progressively extract information from the web on a daily basis and improve its performance incrementally. Similarly, Mitchell et al.~\cite{Never_ending_learning} present "Never-ending learning," a system designed to perpetually acquire information and enhance reading comprehension skills. NELL, initiated in January 2010, has diligently been amassing knowledge, resulting in the construction of a knowledge base comprising over 80 million facts by 2015. The authors of NELL offer URLs and Twitter links to facilitate tracking the system's growth.

In summation, these two categories of methods endeavor to achieve the goal of dynamic knowledge extraction. With the advent of large generative language models, the possibility arises of harnessing their capabilities to automate and perpetuate the extraction of information, thereby constructing knowledge graphs in an ongoing and endless manner.


==> sections/bak/sec3.3_Event_RULE_extraction.tex <==
\subsection{Event Extraction}\label{sec:sec3.3}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\columnwidth]{img/RULE_Event/ExmapleEventy.png}
	\caption{Examples of Event Extraction.}
         % \vspace{-10pt}
	\label{fig:fig_ee}
\end{figure}

% \begin{figure*}[htbp]
% \centering
% \begin{minipage}[t]{0.48\textwidth}
% \centering
% \includegraphics[width=4cm]{img/RULE_Event/NNmethodForEE.png}
% \caption{Illustrations of NN based methods for Event Extraction. NN based methods requires word embedding inputs, and process of one instance with predicted trigger 'attend' and candidate argument 'conference'. The aggregation layer can be attention layer or pooling layer.}
% \end{minipage}
% \begin{minipage}[t]{0.48\textwidth}
% \centering
% \includegraphics[width=8cm]{img/RULE_Event/LLMbasedEE.png}
% \caption{Illustrations of LLM based methods for Event Extraction. Many models such as PLMEE use LLM to find and label Trigger to identify Argument.In this exmaple, LLM finds the Trigger "attend", and use this information to indentify Argument "conference"}
% \end{minipage}
% \end{figure*}


% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=1\columnwidth]{img/RULE_Event/Event_combine.png}
% 	\caption{
% }
%          % \vspace{-10pt}
% 	\label{fig:fig_ekg}
% \end{figure}

Event extraction is an information extraction task that focuses on identifying events and their associated information from unstructured or semi-structured data. This task involves detecting trigger words, identifying event arguments, and linking them together to coherently represent the event. At the document level, event extraction involves identifying events across an entire document or a large corpus of documents. Open-domain event extraction involves extracting events across a wide range of topics, while closed-domain event extraction is focused on a specific domain or topic. Trigger detection is another key aspect of event extraction and involves identifying words or phrases that signal the occurrence of an event. These triggers can be identified through various techniques, including rule-based methods, machine learning algorithms, or a combination. Event arguments refer to the entities or concepts that are involved in the event, such as the agent or patient. These arguments can be identified through various techniques, including syntactic parsing, semantic role labeling, and named entity recognition. To improve the accuracy of event extraction, various approaches have been developed, such as using labeled data to train machine learning models, generating synthetic data to augment existing datasets, using graph-based models to capture complex relationships between events and arguments, and using causal inference techniques to model the causal relationships between events. Overall, event extraction is a challenging task that requires sophisticated natural language processing techniques and a deep understanding of the structure and semantics of the language. However, it has significant potential for applications in information retrieval, knowledge management, and social media analysis.

Time mining is the process of extracting valuable information and knowledge from large amounts of time series data. The extraction of events is often accompanied by the mining of time-series information, such as natural disasters, traffic accidents, and stock market fluctuations, from time series data. Zhang et al.~\cite{zhang2022knowledge} proposed a Knowledge Enhanced method for Event and TempRel Extraction, incorporating temporal commonsense knowledge. 
\subsubsection{Neural Network based Methods}
Traditional approaches to event extraction rely on handcrafted features, such as part-of-speech tags and syntactic dependencies, to identify event triggers and their arguments. These features are then used to train machine learning models, such as recurrent neural networks (RNN, CNN), to classify events and their arguments. Despite their success in early event extraction systems, these methods are limited by their dependence on handcrafted features and their inability to capture complex relationships between events and their arguments. This methods~\cite{nguyen2016modeling, ghaeini2018event, chen2016event} tried to use neural network models to try to solve the problem in event extraction,  R. Ghaeini et al~\cite{nguyen2016modeling} used a forward-backward recurrent neural network (RNN) to detect event trigger words and classify them into different event types, Ghaeini et al.~\cite{ghaeini2018event} introduced skip-gram models to represent event triggers and employs convolutional neural networks (CNNs) to capture local context information for event detection. Nguyen et al.~\cite{nguyen2018graph} proposed graph convolutional networks (GCNs) to capture the dependencies between event triggers and their arguments. The model also employs argument-aware pooling to capture the importance of different arguments in event detection. Recent work~\cite{du2021excar} presented a Conditional Markov Neural Logic Network to represent causal relationships between events and incorporates knowledge graphs to enhance its causal reasoning capabilities. The model provides a transparent approach to analyzing events and their causal relationships

\subsubsection{Large Language Model-based Methods}
In recent years, the performance of event extraction has significantly improved with the use of large language models such as BERT, RoBERTa, and GPT, as shown in Figure~\ref{fig:LLMbasedEE}. Event extraction is the task of identifying events and their relevant information (such as triggers, arguments, and temporal expressions) from text data. In recent years, there has been significant interest in using pre-trained language models (such as BERT and GPT) for event extraction due to their ability to capture contextual information and improve the performance of the extraction process. In addition, approaches such as prompt, which is proposed around the larger language model, also help the event extraction task to be more closely aligned with the language representation, ~\cite{yang2019exploring} presented a study on exploring pre-trained language models for event extraction and generation. The authors showed that fine-tuning BERT on a task-specific dataset can lead to significant improvements in event extraction performance. Tang et al.~\cite{tang2020exploring} proposed a multitask learning approach that jointly trains a neural event classifier and an explanation decoder. The event classifier predicts event types and arguments, while the explanation decoder generates explanations for the model's predictions to increase interpretability. Chen et al.~\cite{chen2022ergo} introduced ERGO, an event relational graph transformer for document-level event causality identification. The model uses a graph-based approach to capture the dependencies between events and infer their causal relationships. Li et al.~\cite{li2022kipt} presented KiPT, a knowledge-injected prompt tuning approach for event detection. KiPT uses prompts to guide the model toward relevant information and leverages external knowledge sources to improve performance. Du et al.~\cite{du2022graph} proposed a graph-enhanced BERT model for event prediction. The model incorporates a graph convolutional network to capture the relationships between events and their arguments. Zhou et al.~\cite{zhou2022eventbert} presented EventBERT, a pre-trained model for event correlation reasoning. The model uses a two-stage approach to identify events and their relationships and can be fine-tuned for various downstream tasks. Fincke et al.~\cite{fincke2022language} proposed language model priming for cross-lingual event extraction. The model leverages pre-trained language models to generate context-aware representations for event extraction across multiple languages. Han et al.~\cite{han2020econet} introduced ECONET, a method for effective continual pre-training of language models for event temporal reasoning. The model is pre-trained on a large corpus of event-related text data and can be fine-tuned for specific event extraction tasks. 
 
Training data scarcity is a major challenge in event extraction, as it requires large amounts of annotated data to train models effectively. With the development of large models, more and more papers use the generalization and understanding capabilities of the model to perform event extraction with low resources Annotating data for event extraction is a laborious and time-consuming process, as it involves identifying event triggers, arguments, and attributes, and linking them together. This process requires domain expertise and can be challenging, particularly for complex events.

To address this challenge, researchers have explored various approaches, including transfer learning, data augmentation, weak supervision, and few-shot learning. Transfer learning involves leveraging pre-trained models to learn representations from large amounts of unlabeled data, which can then be fine-tuned on a smaller set of annotated data for event extraction. Data augmentation techniques such as back-translation, synonym replacement, and word swapping can generate synthetic data to supplement existing annotated data. Weak supervision techniques use heuristics or patterns to automatically label data, which can be used to train models for event extraction.

Several studies have explored these approaches and achieved promising results. For example, ~\cite{liu2022incremental} used a pre-trained prompt language model and few-shot learning to improve event extraction performance with limited labeled data. Many of the data enhancement methods take into account the use of context,  ~\cite{zhang2022knowledge} proposed a temporal relation extraction approach, achieving competitive results with minimal annotated data. while data scarcity remains a challenge in event extraction, there are promising approaches that can mitigate this issue and improve the accuracy and robustness of event extraction models.

\subsection{Rule Extraction}\label{sec:sec3.4}

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=1\columnwidth]{img/RULE_Event/Rule.png}
% 	\caption{Examples of Rule Extraction.}
%          % \vspace{-10pt}
% 	\label{fig:fig_ekg}
% \end{figure}
% AMIE~\cite{AMIE} is an representative symbolic reasoning method that focuses on mining association rules in ontological knowledge bases, even in the presence of incomplete evidence. By utilizing a unique approach that accounts for missing or uncertain information, AMIE overcomes the challenges typically encountered in traditional association rule mining techniques. Based on AMIE, AMIE+~\cite{AMIE+} improves the reasoning efficiency by revising both the rule extending process and the metrics defined in the rule pruning process.

% These method are meaningful tries of adopting symbolic way for knowledge reasoning, however, symbolic reasoning methods predominantly depend on search algorithms, diverse pruning techniques, and effective database operations. However, these methods exhibit several constraints: firstly, the stringent matching criteria and discrete logic operations employed during rule searching make symbolic methods less tolerant of ambiguous and noisy data; secondly, the pre-defined evaluation metrics and rule structures limit the expressiveness of the learned rules.
There is a consensus that knowledge graphs can represent knowledge in a symbolic form, and the potential for applying symbolic reasoning methods in static knowledge graphs is immense. Rule mining is a process of extracting useful knowledge in the form of rules from given datasets, especially for knowledge graphs. In the context of Knowledge Graphs, rule mining refers to the task of discovering logical rules that describe patterns and regularities in the data represented by a KG. One of the main advantages of rule mining in KGs is its ability to provide an explainable way to derive new facts and complete the existing KG. Unlike deep learning models, rules are explicit symbolic knowledge that can be easily interpreted and understood by humans. Moreover, rules mined from KGs can help to identify potential errors and inconsistencies in the KG, as a fact that contradicts a high-confidence rule is likely to be incorrect.

Since 2014, much work has focused on how to use logic rules to mine the knowledge base. Pouya et al.~\cite{omran2018scalable} proposed a new inference module to carry out the link prediction task. Yang et al.~\cite{yang2017differentiable} Learns logical rules in a differentiable way for knowledge base reasoning using a neural network architecture. Yang et al.~\cite{yang2019learn} combined neural networks and logic-based methods for knowledge representation and reasoning, using a graph neural network to represent entities and relations and learning logical rules to capture regularities in the data. Ruleformer~\cite{xu2022ruleformer} mined context-aware rules from knowledge graphs, while AnyBURL~\cite{meilicke2019introduction} supported knowledge base completion, rule learning, candidate ranking, prediction, evaluation, and explanation. DRUM~\cite{sadeghian2019drum} performed differentiable rule mining, AMIE~\cite{AMIE} is a representative symbolic reasoning method that focuses on mining association rules in ontological knowledge bases, even in incomplete evidence. By utilizing a unique approach that accounts for missing or uncertain information, AMIE overcomes the challenges typically encountered in traditional association rule mining techniques. Based on AMIE, AMIE+~\cite{AMIE+} improved the reasoning efficiency by revising both the rule-extending process and the metrics defined in the rule-pruning process. RLogic~\cite{cheng2022rlogic} utilized temporal inductive logic reasoning to recursively learn logical rules from knowledge graphs. These methods provide more accurate and efficient reasoning over large and complex knowledge graphs and have shown promising results in various applications.

\begin{figure}[h]
	\centering
	\includegraphics[width=1\columnwidth]{img/RULE_Event/LLM4EE.png}
	\caption{Illustrations of methods for event extraction based on LLM. Many models, such as PLMEE, utilize a two-stage process: trigger extraction and argument extraction. In the first stage, the LLM is employed to identify trigger tokens. In the second stage, these identified trigger tokens are labeled within segment embedding and then fed back into the LLM as input. Lastly, a classifier is applied to each token to discern the argument. For instance, during the trigger extraction phase, the LLM identifies the trigger "attend" and labels it in the segment embedding. Subsequently, the classifier labels the word "conference" with a "1", designating "conference" as the argument.}
         % \vspace{-10pt}
	\label{fig:LLMbasedEE}
\end{figure}

\begin{table}[t]
\begin{center}
\caption{Overview of Knowledge extraction methods}\label{table:KG_extraction}
\footnotesize
\renewcommand{\arraystretch}{0.8} % 减少行间距
\setlength{\tabcolsep}{4pt} % 减少列间距
\begin{tabular}{l|l|p{2.7cm}|p{4cm}|p{4cm}}
\toprule
 \textbf{Extraction Techniques}& \textbf{KG Type} & \textbf{Method Category} & \textbf{Description} & \textbf{Representative Methods} \cr 
 
 %%%%%NER
\midrule
 \multirow{3}{=}{Named Entity Recognition}&\multirow{3}{*}{All types}& Static \& Discriminative&Static embeddings are utilized in sequence labeling tasks and taggers are employed to identify and consolidate entities& word2vec \cite{word2vec_NER}, GloVe\cite{glove_NER},\cite{glove_NER2}, fastText\cite{fasttext_NER}... \cr
 \cmidrule{3-5}
 & & Contextualized \& Discriminative & Contextualized embeddings capture the contextual information in a sequence & Flair\cite{flair}, BERT\cite{bert_NER}, ELMo\cite{elmo_ner} ... \cr
 \cmidrule{3-5}
 & & Contextualized \& Generative & Additional token markers are generated to represent the entity types within the generative sequence & ANL\cite{ANL_NER}, TANL\cite{TANL}, DEEPSTRUCT\cite{deepstruct}, UGF\cite{UGF_NER}... \cr
 
 %%%%%RE
\midrule
 % \multirow{3}{*}{Relation Extraction}&\multirow{3}{*}{All types}& Pipeline-based& & Joint-based&Method1, Method2 \cr
\multirow{2}{=}{Relation Extraction}&\multirow{2}{*}{All types}& Pipeline-based& As a pipeline, entities are initially identified, followed by the subsequent relation classification & Feature-based\cite{RE_featurebased}, Kernel-based\cite{RE_kernelbased}, CNN-based\cite{RE_NNbased}, PCNN+MIL\cite{distant}, BERT\cite{RE_bert}, TRE\cite{RE_TRE}, Soares, et al.\cite{RE_match}, REBEL\cite{REBEL}, CopyRLL\cite{copyRLL}... \cr
\cmidrule{3-5}
 & & Joint-based & Triples comprising entities and their corresponding relations are jointly generated as output & SPTree\cite{RE_LSTM_RNN}, Katiyar et al.\cite{RE_joint_LSTM}, NDS\cite{RE_Joint_NDS}, CASREL\cite{RE_joint_CASREL}, SpERT\cite{SpERT}, Sui et al.\cite{RE_joint_SetPredictionNetworks}, CGT\cite{CGT}, TEMPGEN\cite{TEMPGEN}...
 \cr

 %%%%%DKE
\midrule
\multirow{1}{=}{Dynamic Knowledge Extraction}&\multirow{1}{*}{DKG}& --- &Entities are relations are dynamically or automatically extracted from open information & KnownItAll\cite{knowitall}, Ollie\cite{ollie}, Knowledge Vault\cite{knowledge-vault}, NELL\cite{Carlson_NELL}, \cite{Never_ending_learning}...\cr
% \cmidrule{3-5}
 

\midrule
 \multirow{2}{=}{Event Extraction}&\multirow{3}{*}{EKG}& Neural network based&Neural networks such as RNN classify text utterances at the token level. For document-level event extraction it performs better & ED-CNN\cite{nguyen2016modeling}, GCN-ED\cite{ghaeini2018event}, FBRNNs\cite{chen2016event} \cr
 \cmidrule{3-5}
 & & Large Language Model-based &Large Language Model conducts multi-stage extraction of a sentence by virtue of a powerful model transfer ability, For low resource case event extraction it performs better. & EventBERT\cite{zhou2022eventbert}, PLMEE\cite{yang2019exploring} \cr


\midrule
 \multirow{1}{=}{Rule Extraction}&\multirow{3}{*}{All types}& ----&Uncover patterns of co-occurrence or dependency between different items based on their occurrence in transactions or events. & AMIE\cite{AMIE}, RLvLR\cite{omran2018scalable}, Neural LP\cite{yang2017differentiable}, DRUM \cite{sadeghian2019drum}, Ruleformer\cite{xu2022ruleformer}, NLIL\cite{yang2019learn} \cr
 

\bottomrule
\end{tabular}
\end{center}
\end{table}

==> sections/bak/sec4.1_SKGR.tex <==
\section{Knowledge Reasoning}\label{sec:4}
Considering the intrinsic limitations of collected data, knowledge extraction alone is insufficient to capture the full spectrum of knowledge. These limitations underscore the need for KG reasoning to supplement the KG by inferring missing entities and relationships. Moreover, KGR also enhances downstream tasks by leveraging the constructed KG. Thus, KGR is also essential for creating a comprehensive and effective KG.


Early work on KGR mainly focus on SKGR. However, these approaches are not applicable to other types of KGs. To this end, multiple works are subsequently proposed for DKGR and TKGR. In this chapter, we review all three types of KGR techniques.


\subsection{Static Knowledge Graph Reasoning}\label{sec:4.1}
In this section, we present an overview of classic papers on static knowledge inference in knowledge graphs. These approaches can be categorized into five primary groups: matrix decomposition-based, translation-based, graph neural network-based, large language model-based, and neural-symbolic based methods.
The formal definition is declared as follows,
\par\smallskip

\noindent\textbf{Definition 5. Static Knowledge Graph Reasoning.}
~\textit{
Given a static knowledge graph $\mathcal{SKG}=(\mathcal{E}{n},\mathcal{R},\mathcal{F})$, Static Knowledge Graph Reasoning is a task that seeks to utilize the existing facts encapsulated in $\mathcal{F}$ to infer a queried fact $(e_s^q, r_p^q, e_o^q)$, where $e_s^q, e_o^q\in\mathcal{E}_n$ and $r_p^q\in\mathcal{R}$.
}

\subsubsection{Matrix Decomposition-based Method}\label{sec:4.1.1}
Matrix decomposition-based techniques have been widely employed for static knowledge reasoning in knowledge graphs. By decomposing the adjacency matrix or other related matrices of the knowledge graph into latent factors, these methods represent entities and relations in a low-dimensional latent space, enabling efficient computation of similarity and relationship prediction.

RESCAL~\cite{RESCAL} is a classical matrix decomposition-based knowledge reasoning method, which employs a three-way tensor factorization method for modeling multi-relational data in knowledge graphs. By capturing the interactions between latent factors for each entity and relation, RESCAL has demonstrated superior performance in knowledge reasoning. It can be formally expressed as follows:

$$
\hat{Y}_{ijk} = \mathbf{e}_i^T \mathbf{R}_k \mathbf{e}_j,
$$
where $\hat{Y}_{ijk}$ signifies the predicted score for the triple $(i, j, k)$, with $i$ and $j$ representing entities and k indicating a relation. $\mathbf{e}_i$ and $\mathbf{e}_j$ correspond to the embedding vectors of entities i and j, respectively, while $\mathbf{R}_k$ denotes the relation matrix for relation $k$. The superscript $T$ represents the matrix transpose operation.

Considering the high computational complexity of RESCAL, the DisMult~\cite{DISTMULT} was proposed, which is a simplified version of the RESCAL model that represents relations as diagonal matrices. By reducing the number of parameters, DistMult achieves comparable performance to RESCAL but with lower computational complexity.
Considering the differences between entities and relations in static knowledge graphs, the ComplEx~\cite{ComplEx} extends RESCAL by using complex-valued embeddings to represent entities and relations. By capturing asymmetric relationships through complex conjugate operations, ComplEx can effectively model knowledge graphs with complex relational structures. 
SimplE~\cite{SimplE} is also a representative matrix decomposition method, which employs a simple bilinear form for modeling relations between entity pairs. SimplE incorporates inverse relations into the model, enabling the learning of symmetric and asymmetric relational patterns in the knowledge graph.

Matrix decomposition-based methods offer advantages in modeling static knowledge reasoning in knowledge graphs by capturing latent semantics and patterns in the data. These approaches enable efficient computation of similarity and relationship prediction through low-dimensional latent space representations. However, they face limitations in terms of scalability and handling sparsity, which may hinder their applicability in large-scale knowledge graphs or those with complex relational structures.

\subsubsection{Translation-based Method}\label{sec:4.1.2}
Translation-based methods represent entities and relationships as vectors in a continuous space, and reasoning is performed by translating entity vectors along relationship vectors.

TransE~\cite{TransE} is a classic and basic algorithm that learns entity and relationship embeddings by minimizing the distance between the head entity plus the relationship and the tail entity for each true triple. Specifically, given the vectors $\mathbf{h}, \mathbf{r}, \mathbf{t}$, the scoring function is:
$$
f(h, r, t)=-\|\mathbf{h}+\mathbf{r}-\mathbf{t}\|_{1 / 2},
$$
where $\|\cdot\|_{1 / 2}$ means that the distance can be $L_1$ or $L_2$ distance.

TransE is simple and computationally efficient, making it a popular choice for knowledge graph reasoning tasks. However, TransE has difficulties modeling complex relationships, such as one-to-many or many-to-many.

Based on the TransE, TransH~\cite{TransH} extends TransE by projecting entities onto relation-specific hyperplanes before performing translations. This allows TransH to model complex relationships more effectively than TransE.
TransR~\cite{TransR} further improves upon TransE and TransH by learning separate entity and relationship spaces. TransR projects entities into relation-specific spaces using relation matrices, allowing it to capture more complex relationship patterns.
RotatE~\cite{RotatE} extends TransE by using complex-valued embeddings and representing relationships as rotations. This allows it to capture more complex relationship patterns while retaining the simplicity and scalability of TransE.

In conclusion, Translation-based methods for knowledge graph reasoning are simple, computationally efficient, and scalable, making them suitable for a wide range of applications. However, they face difficulties in modeling complex relationships and handling noisy or incomplete data.

\subsubsection{GNN-based Method}\label{sec:4.1.3}
This is achieved by gathering and integrating information from neighboring nodes within the knowledge graph. The majority of GNN-based methodologies can be encapsulated by the following formulation:

% $$
% H_t^{l+1} \leftarrow \underset{\forall (s,r,t) \in \mathcal{Q}}{\text { \textbf{AGG} }} (\text { \textbf{ATT} }(H_s^{l}, H_r^{l}, H_t^{l},) \cdot \text { \textbf{MSG} }(H_s^{l}) )||{\text { \textbf{SELF} }}(H_t^{l}),
% $$
\begin{equation}
\small
H_t^{l+1} \leftarrow \underset{\forall (s,r,t) \in \mathcal{Q}}{\text{\textbf{AGG}}} \left( \text{\textbf{ATT}}(H_s^{l}, H_r^{l}, H_t^{l}) \cdot \text{\textbf{MSG}}(H_s^{l}) \right) || \text{\textbf{SELF}}(H_t^{l}),
\end{equation}
where $H$ represents the entity embeddings that have been learned. The abbreviations MSG, ATT, AGG, and SELF stand for message passing, attention mechanism, aggregation, and self-loop mechanism, respectively. Each of these components plays a vital role in the successful operation of GNN-based methods.

GCN~\cite{GCN} is the fundamental model of the GNN-based method, however, it lacks of ability to model multi-relational data.
R-GCN~\cite{RGCN} is a pioneering GNN-based method for knowledge graph reasoning. It extends traditional graph convolutional networks to handle multi-relational data. R-GCN effectively captures local graph structure, but it can suffer from scalability issues and over-smoothing in deep architectures.
CompGCN~\cite{CompGCN} explicitly models the composition of relations in knowledge graphs. CompGCN learns embeddings by composing entity and relation embeddings in the neighborhood of each entity. This enables it to better capture complex relationships and reason about compositions of multiple relations.

In conclusion, GNN-based methods for knowledge graph reasoning can effectively capture local graph structure and complex relationships, making them a suitable choice for various applications. However, they may face challenges related to scalability, over-smoothing, computational complexity, and parameter tuning.

\subsubsection{Large language models-based Method}\label{sec:4.1.4}
Large Language Models (LLMs) have exhibited considerable potential in the field of static knowledge graph reasoning. This potential stems from their inherent ability to store and retrieve factual data that is acquired during the pre-training phase. The primary methodology involves converting the triple path into a coherent textual sequence, subsequently utilizing the pre-trained LLMs to carry out reasoning tasks.

BERT~\cite{bert} is one of the widely adopted basic language models for knowledge graph reasoning. 
Based on BERT, K-BERT~\cite{KBERT} is an extension of the BERT model that incorporates external knowledge from knowledge graphs during pre-training. By injecting structured knowledge, K-BERT can perform better on knowledge graph reasoning tasks compared to the original BERT. 

KG-BERT~\cite{KG-BERT} also uses BERT to encode the textual contents of entities and relationships (e.g., their description text and names) to get the contextualized representations of triples. 
% Then, the BERT is fine-tuned by projecting the representations into a scoring function space for the triplet classification task. 
Coupled with pre-trained word embedding in LLMs, KG-BERT can easily generalize to unseen components. However, KG-BERT has a large room to improve.
MTL-KGC~\cite{DBLP:conf/coling/KimHKS20} added two fine-tuning tasks based on KG-BERT and made the results better. 
StAR~\cite{StAR} augments the textual encoder BERT with graph embedding techniques to enhance its structured knowledge and solves the problem of the efficiency of KG-BERT by reusing graph elements’ embeddings.
CKBC~\cite{CKBC} encodes the various attention weights into the structural representation of the triples and utilizes the triple classification task to fine-tune BERT, which is the same as KG-BERT. The representations of entities and relations in CKBC are a combination of contextual representations from BERT and structural representations from GNN.
Considering the knowledge required by BERT may vary dynamically based on the particular text, CokeBERT ~\cite{CokeBERT} dynamically selects and embeds contextual knowledge based on the actual context of triples.

To improve the learning efficiency of LLM-based methods, SimKGC~\cite{SimKGC} introduces three types of negatives: in-batch negatives, pre-batch negatives, and self-negatives which act as a simple form of hard negatives. 
SimKGC also proposes a re-ranking strategy to reduce the reliance on semantic match of LLM-based methods.
ERNIE~\cite{ERINE} is another large pre-trained language model that explicitly incorporates knowledge graph information. ERNIE uses a dynamic masking strategy during pre-training to better capture the relationships between entities. This enables ERNIE to perform well on knowledge graph reasoning tasks.
% Other LLM-based methods such as KG-BERT~\cite{KG-BERT}, StAR~\cite{StAR} are also dedicated to introducing LLM with the tremendous knowledge via pre-train for knowledge reasoning, and achieves superior performance, which demonstrates the potential ability of LLM for knowledge reasoning. 
% Besides, recent study BERTRL~\cite{BERTRL} also preforms the inductive reasoning ability of LLM for knowledge reasoning.

In conclusion, large language models incorporating knowledge graph information show promise for knowledge graph reasoning tasks, capturing rich semantic information and leveraging pre-trained knowledge. However, they may face challenges related to scalability, memory limitations, computational complexity, and prompt design.

\subsubsection{Neural-Symbolic Method}\label{sec:4.1.5}
The above static knowledge graph reasoning method all based on neural network models, which suffer the interpretable and unreliable problems, and can not be adopted in some real-world scenarios such as medical, finance, and military which have high reliability demands.

% There is a consensus that knowledge graphs can represent knowledge in a symbolic form, and the potential for applying symbolic reasoning methods in static knowledge graphs is immense.
% AMIE~\cite{AMIE} is an representative symbolic reasoning method that focuses on mining association rules in ontological knowledge bases, even in the presence of incomplete evidence. By utilizing a unique approach that accounts for missing or uncertain information, AMIE overcomes the challenges typically encountered in traditional association rule mining techniques. Based on AMIE, AMIE+~\cite{AMIE+} improves the reasoning efficiency by revising both the rule extending process and the metrics defined in the rule pruning process.

% These method are meaningful tries of adopting symbolic way for knowledge reasoning, however, symbolic reasoning methods predominantly depend on search algorithms, diverse pruning techniques, and effective database operations. However, these methods exhibit several constraints: firstly, the stringent matching criteria and discrete logic operations employed during rule searching make symbolic methods less tolerant of ambiguous and noisy data; secondly, the pre-defined evaluation metrics and rule structures limit the expressiveness of the learned rules.

Recently, there have been studies attempting to combine neural and symbolic ways of knowledge reasoning, aiming to leverage the strengths of both paradigms.
We follow the study~\cite{zhang2021neural} and divide relevant methods into symbolic-driven neural reasoning methods and neural-driven symbolic reasoning methods.

Symbolic-driven neural reasoning methods leverage symbolic reasoning to guide and enhance the learning process of neural networks. 
KALE~\cite{KALE} is a symbolic-driven neural reasoning method that integrates first-order logical rules into neural embeddings. KALE encodes logical rules into the neural model by transforming them into soft constraints, which helps to improve the expressiveness and reasoning capabilities of the embeddings. RUGE~\cite{RUGE} is another symbolic-driven neural reasoning approach that incorporates first-order logical rules into the learning process of neural embeddings. RUGE uses rules to guide the training of embeddings, making them more interpretable and capable of handling complex reasoning tasks. 

% KALE, RUGE

Neural-driven symbolic reasoning aims to derive the logic rules, where the neural networks are incorporated to deal with the uncertainty and the ambiguity of data, and also reduce the search space in symbolic reasoning.
PRA~\cite{PRA} is a neural-driven symbolic reasoning method that learns to reason over knowledge graphs by exploring paths between entities. PRA employs a neural network to learn the importance of different paths, allowing it to make predictions about relationships in the graph.
MINERVA~\cite{MINERVA} is a neural-driven symbolic reasoning method that uses a reinforcement learning-based approach to explore a knowledge graph. It employs a neural network to guide the search for relevant paths between entities, enabling it to handle multi-hop reasoning tasks effectively.
GraIL~\cite{GraIL} is another neural-driven symbolic reasoning approach that uses graph neural networks to learn first-order logic rules for knowledge graph reasoning. 
%PRA, MINERVA, GraIL

In conclusion, neural-symbolic methods for knowledge graph reasoning offer a more interpretable and explainable way of reasoning, making them suitable for various applications that require transparency and understanding. However, they may face challenges related to scalability, computational complexity, implementation complexity, and sensitivity to data quality.

==> sections/bak/sec4.2_DKGR.tex <==
% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=1\columnwidth]{img/DKG/framework.pdf}
% 	\caption{The categorization of DKGR.}
% 	\label{fig:DKGR_framework}
% \end{figure}
\subsection{Dynamic Knowledge Graph Reasoning}\label{sec:4.2_}

Traditional knowledge graph reasoning methods are under a closed-world assumption, so these models are designed for a fixed set of entities and relations and are unable to consider unseen components.
% How and Why is an Answer (Still) Correct? Maintaining Provenance in Dynamic Knowledge Graphs
However, new entities and relations emerge continuously in the ever-changing real world due to several reasons, such as improvements to the knowledge extraction techniques and refinement/enrichment of information. 
Dynamic knowledge graph reasoning aims to deal with emerging entities and relations, which may influence the semantics of existing entities and relations, and predicts the missing links among emerging entities and existing entities.
The formal definition is declared as follows,
\par\smallskip

\noindent\textbf{Definition 6. Dynamic Knowledge Graph Reasoning.}
~\textit{
Given a dynamic knowledge graph $\mathcal{DKG}=\{\mathcal{E}{n},\mathcal{R},\mathcal{F}\}$, the task of Dynamic Knowledge Graph Reasoning seeks to exploit the existing facts in $\mathcal{F}$, which are updated dynamically, to infer a queried fact $(e_s^q, r_p^q, e_o^q)$, where $e_s^q, e_o^q\in\mathcal{E}_n$ and $r_p^q\in\mathcal{R}$.}

We categorized the existing methods according to their modeling perspectives: GNN-based methods and LLM-based methods. In the GNN-based methods, they use GNN or its variants to model emerging entities and relations and the source of the inductive ability can be further divided into four categories: the structure of graphs, relation rules, embedding aggregators and meta-learning. In the LLM-based methods, the entities and relations of the edges in KGs are usually converted into natural language, serving as the input of LLMs, and the powerful understanding ability of LLMs benefits these models. They can be categorized into two groups: depending on one single edge (triple-level) and depending on paths composed of edges (path-level).

With the changing of DKGs, there is a certain probability that unseen entities and relations are long-tail. Therefore, the representations of unseen relations and entities cannot be sufficiently trained given limited training instances (few-shot setting). Thus, few-shot KGR methods are aimed to improve the generalization ability to infer unseen relations with a few facts.


\subsubsection{GNN-Based Methods}
% 讲一下这些方法通常都是怎么做的
GNN and its variants have been widely used for dynamic knowledge reasoning in dynamic knowledge graphs (DKGs), since GNN can model entities and relations based on the connecting structure and has the potential to handle knowledge out of distribution.
Because of the advantages above, GNN-based DKGR methods capture the transferable knowledge in DKGs through rich structure information and transfer it to new entities and relations, obtaining trusted representations for reasoning tasks over DKGs, such as inductive link prediction. In Figure~\ref{fig:inductive ability}, we categorize the GNN-based methods into four categories, according to four sources of their inductive ability. 

\textbf{Inductive Ability Provided by the Structure of Graphs.}
Subgraphs consisting of the local neighborhood of a particular triplet in DKGs have been proven to contain the logical evidence needed to deduce the relation between the target nodes.
GraIL~\cite{GraIL} proposes to learn entity-independent relational semantics and aggregates the representation of nodes by GNN, so GraIL can be naturally generalized to unseen nodes. GraIL also introduces a series of new fully-inductive benchmark datasets for the inductive relation prediction problem, by sampling disjoint subgraphs from the KGs in four traditional transductive datasets. The subgraph representation $\mathbf{h}_\mathcal{G}{\left(u, v, r_{t}\right)}$ in GraIL is as follows:

$$
\mathbf{h}_\mathcal{G}{\left(u, v, r_{t}\right)}=\frac{1}{|\mathcal{V}|} \sum_{i \in \mathcal{V}} \mathbf{h}_{i},
$$
where $|\mathcal{V}|$ denotes the set of vertices in graph $\mathcal{G}_{\left(u, v, r_{t}\right)}$, $\mathbf{h}_{i}$ is the latent representation of node in subgraph $\mathcal{G}_{\left(u, v, r_{t}\right)}$.
Following GraIL, CoMPILE~\cite{DBLP:conf/aaai/MaiZY021} further considers the directed nature of the extracted subgraph structure to enable a sufficient flow of relation information. Therefore, CoMPILE can naturally handle asymmetric and anti-symmetric relations in subgraphs.
These two approaches require generating one subgraph for each target triple, which is a significant bottleneck in practice.
INDIGO~\cite{DBLP:conf/nips/LiuGHK21} constructs a node-annotated graph, where nodes represent pairs of constants and two nodes are connected only if their pairs share a constant, and the original KG is fully encoded into a GNN in a transparent way. 
Once the types and relations in KGs are fixed, the dimension of nodes in the node-annotated graph does not depend on the input KG, making the inductive capabilities of GNN fully exploited.
\begin{figure}[h]
	\centering
	\includegraphics[width=1\columnwidth]{img/DKG/inductive_ability.png}
	\caption{Four sources of inductive ability in GNN-Based DKGR Methods.}
	\label{fig:inductive ability}
\end{figure}

\textbf{Inductive Ability Provided by Relation Rules.}
Rule mining uses observed co-occurrences of frequent patterns in KGs to determine logical rules, which can transfer reasoning to unseen facts.

NeuralLP~\cite{yang2017differentiable} is the first end-to-end differentiable approach to learning the structure of logical rules. DRUM~\cite{sadeghian2019drum} further attaches the found rules with confidence scores by bidirectional RNNs.
TACT~\cite{TACT} categorizes topology-aware correlations between relations into seven topological patterns, and learns their importance in an entity-independent manner for inductive link prediction.

PathCon~\cite{DBLP:conf/kdd/0004RL21} leverages relational context and relational paths to directly pass relational messages among edges iteratively to aggregate neighborhood information. PathCon is applicable to the inductive settings since nodes temporarily store the messages from their neighbor edges.
% 结合1和2：Relational Message Passing for Fully Inductive KGC：结合GraIL和关系建模（关系消息传递）
Combining GraIL and PathCon, RMPI~\cite{DBLP:journals/corr/abs-2210-03994} conducts relational message passing over subgraphs for fully-inductive KGC and further proposes new techniques on graph transformation, graph pruning, relation-aware neighborhood attention, addressing empty subgraphs, etc.


\textbf{Inductive Ability Provided by Embedding Aggregators.}
Recent efforts suggest that training a neighborhood aggregator like conventional GNN may help embed new entities inductively via their existing neighbors, so many methods modify GNN as an embedding aggregator in various ways.
LAN~\cite{LAN} introduces a novel aggregator, which addresses the properties by aggregating neighbors with both rules- and network-based attention weights, to facilitate inductive KG embedding.
ROLAND~\cite{DBLP:conf/kdd/YouDL22} views the node embeddings at different GNN layers as hierarchical node states and then recurrently updates them, easily repurposing any static GNN to dynamic graphs.
SE-GNN~\cite{SE-GNN} studies KGE extrapolation problems from a data-relevant and model-independent view and proposes a GNN-based KGE method modeling the semantic evidence.

\textbf{Inductive Ability Provided by Meta-Learning.}
Inspired by the ability of “learning to learn” brought by meta-learning, researchers formulated a set of tasks consisting of support triples and query triples to mimic the link prediction task in the emerging KG, and used GNN to embed unseen components in each task.
HRFN~\cite{10.1145/3459637.3482367} concentrates on effectively embedding out-of-knowledge-base entities by a two-stage model, where coarse-grained pre-representation and fine-tuning aim at emerging entities are used.
MaKEr~\cite{MaKEr} and MorsE~\cite{MorsE} propose a problem called inductive knowledge graph embedding. They train knowledge graph embedding models based on meta-learning on a set of entities that can generalize to unseen entities for either in-KG(i.e., link prediction) or out-of-KG tasks(i.e., question answering). The meta-training objective in MorsE is:
$$
\min _{\theta, \phi, \mathrm{R}} \sum_{i=1}^{m} \mathcal{L}_{i}=\min _{\theta, \phi, \mathrm{R}} \sum_{i=1}^{m} \mathcal{L}\left(Q_{i} \mid f_{\theta, \phi}\left(G_{i}\right), \mathbf{R}\right),
$$
where $\mathrm{R}$ is the relation embedding matrix for all relations, $f_{\theta, \phi}\left(G_{i}\right)$ is used for outputting entity embedding matrix for
entities in the current task, \{ $\theta, \phi$, $\mathrm{R}$\} are learnable parameters;
$m$ denotes the number of all sampled tasks.


In conclusion, GNN-based methods are under an encoder-decoder framework and are able to take advantage of the connectivity structure to generate the representation of emerging entities and relations. GNN and its variants, such as R-GCN and GAT, provide insightful semantic information or rule patterns for these methods and use relation-specific transformation to model the directed nature of DKGs, making GNN-based methods explainability over DGKs, scalability and suitable for various applications. However, GNN-based methods may face challenges related to computational complexity and over-smoothing, and they are restricted by the original framework of GNN.

\subsubsection{LLM-Based Methods}
% 4.基于LLM的方法 KGBERT、MTL-KGC、StAR、LMKE、SimKGC、BERTRL
The proposal of Large Language Models (LLMs) indicates that general semantic knowledge which widely exists in open source corpus can be encoded into the parameters of LLMs via pre-training and fine-tuning. Current LLM-based works research how to integrate KG-specific knowledge into the inductive ability of LLMs and attempt to convert from a data-driven way to a knowledge-driven way. In Figure~\ref{fig:DKGR_LLM}, LLM-based DKGR methods are classified into two categories: triple-level methods and path-level methods.

\textbf{Triple-level Methods.}
Before the proposal of LLMs, DKRL~\cite{DBLP:conf/aaai/XieLJLS16} explores the continuous bag-of-words (CBOW) model to maximize the likelihood of predicting the description text of entities. 
LLM-based models mentioned in Section~\ref{sec:4.1.4} like KG-BERT, StAR, CKBC can also be used in DKGR since they are able to deal with unseen entities via the pre-trained prior knowledge in LLMs.
Some recent works conduct experiments in the inductive setting for DKGR.
For example, KEPLER~\cite{KEPLER} encodes textual entity descriptions with BERT as their embeddings and aligns them to the symbol space of KGs, then KEPLER jointly optimizes the knowledge embedding objective and the masked language modeling (MLM) objective. For a a relational triplet $(h, r, t)$, KEPLER encodes each part with BERT E:

$$
\begin{aligned}
\mathbf{h} & =\mathrm{E}_{<\mathrm{s}>}\left(\text { text }_{h}\right) \\
\mathbf{t} & =\mathrm{E}_{<\mathrm{s}>}\left(\text { text }_{t}\right), \\
\mathbf{r} & =\mathbf{T}_{r},
\end{aligned}
$$
where $\text { text }_{h}$ and $\text { text }_{t}$ are the descriptions
for $h$ and $t$, with a special token $<s>$ at the beginning. $T$ is the relation embeddings and
$\mathbf{h}, \mathbf{t}, \mathbf{r}$ are the embeddings for $h, t and r$.
In KEPLER, knowledge embeddings provide factual knowledge for PLMs, while informative text data also benefit knowledge embeddings.
Experimental results illustrate the effectiveness of LLM-based methods in DKGR.

\textbf{Path-level Methods.}
In addition to using BERT for encoding a single triple, there are also many methods leveraging BERT to mine rules in DKGs. The rules here are presented in the form of natural language rather than traditional symbolic rules.

BERTRL~\cite{BERTRL} concatenates the paths consisting of constructed triples into textual information and combines it with the pre-trained prior knowledge, forming rule-like reasoning evidence. The BERT in BERTRL is used as a score function to score the probability that the candidate relational triple is true.
Bi-Link~\cite{Bi-Link} searches for relational prompts according to learned syntactical patterns via BERT and comes up with probabilistic syntax prompts for link predictions. Bi-Link also uses contrastive learning for bidirectional linking between forward prediction and backward prediction to express symmetric relations.

In conclusion, the pre-trained LLMs have shown that factual knowledge inside KGs can be recovered from PLMs, so LLM-based methods convert edges or relation paths connecting subject and object into natural language form. LLMs enable LLM-based DKGs methods to have language comprehension skills and be able to deal with emerging entities and relations in the semantic space. 
However, LLM-based DKGR methods may face the shortcomings of high GPU memory and the static property of LLMs may not catch up with the dynamic property of DKGs for the rapid update of DKGs.
\begin{figure}[h]
	\centering
	\includegraphics[width=1\columnwidth]{img/DKG/LLM.png}
	\caption{Two categories of LLM-Based DKGR Methods.}
	\label{fig:DKGR_LLM}
\end{figure}

\subsubsection{Few-Shot Knowledge Graph Reasoning}

To learn the representation of the components in KGs, previous methods usually represent relations and entities based on a large amount of training data. In contrast, few-shot knowledge graph reasoning mainly relies on transferring and adapting learned knowledge. In this section, we introduced the original proposal of few-shot learning, a main way of few-shot learning called meta Learning and some other new proposed few-shot learning methods.

\textbf{The Original Proposal of Few-shot Learning.}
GMatching~\cite{DBLP:conf/emnlp/XiongYCGW18} is the first to propose the task of predicting long-tail relations and formulate it as one-shot relational learning.
GMatching learns a matching metric to discover similar triples for target triples. Once trained, GMatching can be adapted to any new relations without fine-tuning, achieving one-shot learning.
For zero-shot(new-added) relations, ZSGAN~\cite{DBLP:conf/aaai/QinWCZXW20} is able to generate text category representations from text descriptions by setting adversarial learning goals.
However, FSRL~\cite{DBLP:conf/aaai/ZhangYHJLC20} thinks works of one-shot and zero-shot learning limit the generalizability of models and do not fully use the supervisory information, so FSRL proposes to discover facts of new relations with few-shot references which is more suitable for practical scenarios. FSRL mainly uses a heterogeneous graph structure encoder based on the attention mechanism and aggregates the few-shot reference set based on LSTM.
FAAN~\cite{FAAN} formally proposes the notion of dynamic properties in few-shot KG completion for the first time and designs an adaptive attention network to adapt dynamic entity representations in different tasks.

\textbf{Meta-learning-based Few-shot Learning Methods.}
Meta-learning for the few-shot setting aims to capture transferable relation-specific meta-information and is suitable and well-performing for dynamic knowledge graphs, since emerging relations usually have few links.
MetaR~\cite{MetaR} proposes relation meta and gradient meta with common and shares knowledge to predict new facts about the target relation, which only has a few observed associative triples.
The gradient meta $G_{\mathcal{T}_{r}}$ for relation meta $R_{\mathcal{T}_{r}}$ in MetaR is regarded as the gradient of $R_{\mathcal{T}_{r}}$ based on the loss $L$, so that relation meta can be updated as follows:

$$
\begin{aligned}
G_{\mathcal{T}_{r}}=\nabla_{R_{\mathcal{T}_{r}}} L\\
R_{\mathcal{T}_{r}}^{\prime}=R_{\mathcal{T}_{r}}-\beta G_{\mathcal{T}_{r}},
\end{aligned}
$$
where $\beta$ indicates the step size of the gradient meta when operating on relation meta.

Meta-KGR~\cite{Meta-KGR} proposes a meta-based RL framework, where the learned meta-knowledge on normal relations provides well-initialized parameters of new models for few-shot relations and the multi-hop reasoning offers interpretability for the results. 
Based on Meta-KGR, FIRE~\cite{DBLP:conf/emnlp/Zhang0S0C20} further performs heterogeneous structure encoding and knowledge-aware search space pruning in the reinforcement learning process, outperforming Meta-KGR.

\textbf{New Proposed Few-shot Learning Methods.}
GEN~\cite{GEN} proposes an inductive learning module to extrapolate knowledge in the support set and then considers inter-relationships between unseen entities in the transductive learning module.
P-INT~\cite{DBLP:conf/emnlp/XuZKDCLL21} leverages the paths that can expressively encode the relation of two few-shot entities and calculates the interactions of the paths.
ADK-KG~\cite{DBLP:conf/sdm/0002QYZ22} uses pre-trained entity and relation embeddings and the optimized parameters can be fast adapted for few-shot relations.
Niu et al.~\cite{DBLP:conf/sigir/NiuLTGDLWSHS21} proposes a gated neighbor aggregator to filter the noise neighbors, capturing the most valuable contextual semantics of few-shot relations, and considers complex relations simultaneously.
REFORM~\cite{REFORM} points out that plenty of errors could be inevitably incorporated in most existing large-scale KGs and proposes an error mitigation module to study error-aware few-shot KG completion.
GMUC~\cite{DBLP:conf/dasfaa/ZhangWQ21} leverages Gaussian metric learning to capture uncertain semantic information and to complete few-shot uncertain knowledge graphs.
Yao et al.~\cite{DBLP:conf/coling/Yao0X022} proposes a data augmentation technique from inter-task view to generate new tasks for few-shot knowledge graph completion, and from intra-task view to enrich the support or query set for an individual task. The proposed framework can be applied to a number of existing few-shot knowledge graph completion models.

In conclusion, few-shot DKG reasoning is a relatively new research area and the meta-learning approach fixes the challenges of data limitation, to a certain extent. However, the dynamic properties in few-shot learning have not been widely researched. Therefore, there is much room to exploit for researchers in the future.






















==> sections/bak/sec4.3_TKGR.tex <==
\subsection{Temporal Knowledge Graph Reasoning}\label{sec:4.3}
Both static or dynamic knowledge graphs only record the knowledge graph at a certain time or the latest state, and cannot reflect the evolution process of the relations between entities at different times. Different from them, the temporal knowledge graph records the valid time of knowledge. 
 The formal definition of temporal knowledge graph reasoning (TKGR) is defined as follows:
\par\smallskip

\noindent\textbf{Definition 7. Temporal Knowledge Graph Reasoning.}
~\textit{
Given a temporal knowledge graph $\mathcal{TKG}=\{\mathcal{E}_{n},\mathcal{R},\mathcal{T},\mathcal{F}\}$, the task of Temporal Knowledge Graph Reasoning aims to utilize the existing facts in $\mathcal{F}$, each with associated temporal information from $\mathcal{T}$, to infer a queried fact $(e_s^q, r_p^q, e_o^q, t^q)$, where $e_s^q, e_o^q\in \mathcal{E}_{n}$, $r_p^q\in\mathcal{R}$ and $t^q\in\mathcal{T}$.}

\begin{figure}[h]
	\centering
	\includegraphics[width=1\columnwidth]{img/tkg/TKGC_TKGP.png}
	\caption{The illustration of temporal knowledge graph completion and temporal knowledge graph prediction.}
	\label{fig:tkgc_tkgp}
\end{figure}

The temporal knowledge graph reasoning includes two parts as shown in Figure~\ref{fig:tkgc_tkgp}: The temporal knowledge graph completion(explaining the TKG at some past time), and the temporal knowledge graph prediction (predicting the state of TKG at a given future time)~\cite{vila1994survey}.

In this section, we classify the methods for temporal knowledge graph reasoning into two categories: completion methods and prediction methods.

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=1\columnwidth]{img/tkg/TKG_framework.pdf}
% 	\caption{The categorization of Temporal Knowledge Graph Reasoning.}
% 	\label{fig:figure_TKG_framework}
% \end{figure}

\subsubsection{Temporal Knowledge Graph Completion}
The temporal knowledge graph completion methods aim to understand the time information and integrate it into the semantic and structural information in the knowledge graph. The temporal knowledge graph completion methods can be divided into two parts: tensor decomposition-based completion methods and translation-based completion methods.

\textbf{Tensor Decomposition-based Completion Methods.}
The tensor decomposition-based completion methods learn the evolution law of the entire graph. As the temporal knowledge graph is represented as a sequence of static snapshots, which can be modeled as a sequence of matrices or high-dimensional tensors. The tensor decomposition-based completion methods can be divided into CP decomposition methods~\cite{1927The} and Tucker decomposition methods~\cite{tucker1966some}. The former decomposes high-dimensional tensors into a series of rank tensors, and the latter considers the core tensor, which represents the main properties of the original tensor. When the core tensor is a hyper-diagonal matrix, Tucker decomposition is a special case of CP decomposition.

Lacroix et al.~\cite{lacroix2020tensor} represented the temporal knowledge graph as a four-dimensional tensor 
% $\mathcal{TKG} \in R^{|E|\times|R|\times|E|\times|T|}$
and extends the ComplEX~\cite{ComplEx} to the temporal knowledge graph reasoning, proposing the CP decomposition method TComplEX. Compared to CP decomposition, Tucker decomposition has better reasoning performance, but its decomposition efficiency is lower due to the operations involving the core tensor.  ~\cite{tresp2017embedding} and ConT~\cite{ma2019embedding} used a 4th-order Tucker decomposition to obtain the representations of entities, relations, and time information. ~\cite{shao2022tucker} adds temporal regularization constraints in adjacent time representation based on Tucker decomposition. Considering that different relations may have different temporal properties, such as the periodic feature of relations, and temporal dependencies among different relations. Based on   ~\cite{tresp2017embedding}, TIMEPLEX~\cite{TIMEPLEX} considers the periodicity scores and temporal dependency scores of the relations in the reasoning procedure.

% In summary, tensor decomposition-based inference methods learn the evolution rules of temporal knowledge graphs from the entire graph perspective and obtain semantic representations of entities, relationships, and time by decomposition. This type of method is relatively mature and has stable performance. However, tensor decomposition algorithms have high time complexity and occupy a large amount of computing resources, making it difficult to apply to large-scale knowledge graph data. Moreover, this type of method has poor flexibility and can only learn representations for entities and time points that appear in the training set, lacking generalization representation ability and limited application performance.

\textbf{Translation-based Completion Methods.}
% This type of method is similar to the translation-based representation method of static knowledge graphs. 
The representations of entities, relations, and temporal information are not decomposed from snapshots of the knowledge graph but are learned in the form of vectors or other representations.
Translation-based reasoning methods can be divided into two types: reasoning with explicitly represented time information and implicitly represented time information.

\textit{Completion with Explicitly Represented Time Information.}
Reasoning methods with explicit time information represent the temporal information in TKGs in the form of temporal transition matrices, embedded vectors, and time mapping matrices.
Time representation is independent of the representation of entities and relations and represents the evolutionary information of the TKG at each snapshot from a macroscopic level.
The representation of entities and relations is static and remains unchanged, independent of time information.

\cite{TAE2016} observes that the temporal knowledge sequence of the same entity: \textit{(Albert Einstein, born in, Ulm, 1879)}, \textit{(Albert Einstein, awarded, Nobel Prize in Physics, 1922)}, and \textit{(Albert Einstein, passed away in, Princeton, 1955)} represents the temporal sequence of \textit{born in, awarded, passed away}. The time-aware embedding (TAE) incorporates the temporal information of relationships using a temporal matrix to learn relationship representations that contain temporal information.  TAE-ILP~\cite{jiang2016towards} considers the valid time intervals of knowledge and uses the Integer Linear Programming technique to restrict the temporal knowledge of shared head entities to non-overlapping time intervals.
TTransE ~\cite{leblay} learns the time representation based on the static knowledge reasoning method TransE, and combines the representation of entities, relations, and time information to calculate the confidence of the temporal knowledge. 

%TODO 这里补一个HyTE的示意图
\begin{figure}[h]
	\centering
	\includegraphics[width=1\columnwidth]{img/tkg/HyTE.pdf}
	\caption{The illustration of HyTE.}
	\label{fig:figure_HyTE}
\end{figure}

HyTE \cite{HyTE} designs the time hyperplane to reflect the entity and relation information at a specific time. As shown in Figure~\ref{fig:figure_HyTE}, in the reasoning process, HyTE projects the head entity, relationship, and tail entity vectors $e_h$, $e_r$, and $e_t$ to the corresponding time hyperplane $T_1$, $T_2$ to obtain the entity and relationship representation at different time.
% This time modeling method can effectively help the model to distinguish time-sensitive relationships, such as "born in" and "passed away in" relationships, and achieve better performance in knowledge-level reasoning tasks, especially relationship prediction tasks. 
To reflect the evolutionary process of entity information in the temporal knowledge graph, TeRo~\cite{TERO} defines the entity representation at different moments as rotation in the complex vector space, which is the Hermitian dot product of entity and time vectors, to reflect the evolutionary process of entities.

% %TODO 这里补一个TOKEI的示意图
% \begin{figure*}[h]
% 	\centering
% 	\includegraphics[width=1.7\columnwidth]{img/tkg/TOKEI.pdf}
% 	\caption{The illustration of TOKEI.}
% 	\label{fig:figure_TOKEI}
% \end{figure*}


% , for example, temporal information such as \textit{(Germany, capital, Berlin, 1980s)} and \textit{(Germany, capital, Berlin, January 16, 1989)} have granularities at the level of decade and day, respectively.
Considering time information in knowledge graphs can be represented at different granularities, TOKEI~\cite{leblay2020towards} designs the hierarchical temporal matrix that is adaptable to different time granularities  (e.g., year-month-day or year-quarter-month-week-day).
% As shown in Figure~\ref{fig:figure_TOKEI}, the same entity or relation is represented by different temporal matrices for \textit{1980s} and \textit{January 16, 1989} at different time granularities to calculate the knowledge confidence score.
TA-TRANSE~\cite{TA-TransE}  takes into account that time sequences at different granularities are of unequal lengths, such as [\textit{1989}] and [\textit{1989, January, 16th}]. It uses the LSTM to encode the time sequences as the temporal information of knowledge.
% This approach can effectively inject time information into relations and achieves better performance in entity inference tasks compared to static knowledge reasoning models.
However, the aforementioned methods ignore the correlation between temporal information. TeLM~\cite{TeLM}  introduces a temporal smoothing mechanism into the loss function, which constrains the change in the representation of adjacent moments to reflect the temporal correlation.  TIME2BOX~\cite{cai2021time} and RTGE~\cite{RTGE} both design temporal smoothing mechanisms to constrain the change in adjacent time vectors. 
% Experimental results demonstrate that the temporal smoothing mechanism effectively captures the temporal correlation information, and that the embeddings of adjacent temporal information are closer in high-dimensional space, indicating a better representation of the temporal correlation.

% In summary, in the temporal knowledge graph reasoning methods with explicit representation of time, the representation of time is independent of the representation of entities and relations, and it contains macroscopic evolutionary information of the temporal knowledge graph at that moment. This type of method requires training the corresponding representation for all temporal information in the training set and is not suitable for knowledge graphs that are frequently changing and have rich temporal information. When the granularity of temporal information is too fine, although it can improve the reasoning performance of the model, it can also result in a large amount of training computational overhead.

\textit{Completion with Implicitly Time Information.}
The completion methods implicitly represented the time information, and model the evolution of entities or relations with time as functions, which reflects the evolution trend of each entity at each moment. The time information is incorporated in the representation of entities or relationships. 

TRESCAL~\cite{leblay} extends the static knowledge graph reasoning method RESCAL~\cite{RESCAL} to temporal knowledge graph reasoning. TRESCAL considers that the information of relations evolves over time, and the temporal information depends on the existence of the relationship, i.e., the relation-temporal matrix $W_{r,t}$ is trained at different temporal information. 
% However, the combination of relationship and time is enormous, which means that TRESCAL has high temporal and spatial complexity, and cannot learn the correlation of time information.
Diachronic embedding ~\cite{DE-SimplE} regards representations of entity and relation as a series of time functions, which use parameterized Fourier functions to encode the entity and relation representations at time spots.
% , and this encoding method has been proven to reflect the correlation between time information, effectively modeling the linear and periodic changes in the evolution process.
% , and significantly reducing the number of model parameters.
% Compared to the TTransE and HyTE models, the MRR indicator in the entity inference task is increased by an average of 19.4\%. 

Furthermore, ATiSE~\cite{ATiSE} considers uncertainty in the time functions and adds random noise to the representation of entities and relations to simulate random interference factors. It conducts reasoning by learning the parameters of a multi-dimensional Gaussian distribution composed of three factors: linear trend, periodic trend, and noise. 
% The above reasoning methods directly model entities and relationships as functions of time, making the reasoning process a black box without interpretability. 
T-GAP~\cite{T-GAP} designs an interpretable mechanism: starting from the target entity $u$ in the incomplete knowledge $(u,r,?,t)$, T-GAP iteratively expands the subgraph using attention pruning strategies and updates the representations and attention scores of each entity in the subgraph through a time-aware graph neural network. 
% The attention score can explain the reasoning process to some extent. 
After the expansion process ends, the entity with the highest attention score in the subgraph is chosen as the correct answer for completion. 
% In summary, reasoning with implicitly represented time information assumes that the representation of entities or relationships dynamically changes over time, and does not require an explicit representation method specifically designed for time. Such methods model the evolution features of specific entities or relationships over time at a microscopic level, which has greater flexibility. However, when the observable time span of the knowledge graph is large, it is often difficult to train high-quality entity representations~\cite{T-GAP}.

\subsubsection{Temporal Knowledge Graph Prediction}
Temporal knowledge graph prediction methods aim to learn the evolution patterns of TKG historical information to predict future states.
These methods can be further categorized into three types: path-based prediction methods, point process-based prediction methods, and sequence network-based prediction methods.

\textbf{Path-based Prediction Methods}
Due to the graph nature of temporal knowledge graphs, the sampled time-constrained random walk paths in temporal knowledge graphs can be viewed as multi-hop relations between entities to represent reasoning rules.
% As the relationships between entities have temporal dynamics, time constraints should be considered when collecting traversal paths. Based on the constraints obeyed during path collection, path-based reasoning methods can be divided into snapshot-based path reasoning and temporal-constraint-based path reasoning. For the former, the temporal information within a path is the same because the collected paths are constrained within a snapshot. For the latter, the temporal information within a path follows certain rules to reflect the evolution of the graph.
The path-based prediction methods of temporal knowledge graphs believe that the temporal walks~\cite{nguyen2018dynamic} in the graph reflect the evolution rules of knowledge.
% These methods consider the unidirectional property of time when sampling paths, and sample paths that follow temporal constraints to learn the unidirectional evolution rules of the knowledge graph over time in order to predict the future.

 In an $L$-length temporal walk  $(v_{1}, v_{2}, t_{1}), (v_{2}, v_{3}, t_{2}), ..., (v_{L}, v_{L+1}, t_L)$, the adjacent temporal edges should satisfy the temporal-ordered constraint $t_1 \leq t_2 \leq ... \leq t_L$, ensuring that the walk contains the temporal dependency information between entities.
% Experimental results show that compared to random walk methods that do not consider temporal constraints, CTDNE improves the AUC score by 15.6\% in knowledge reasoning tasks.
TLogic ~\cite{TLogic} considers the temporal properties of multi-hop relation reasoning and proposes the Cyclic Temporal Logical Rule, represented as:

$P_1(u, z_1, t) \wedge P_2(z_1, z_2, t+1) \wedge \ldots \wedge P_n(z_{n-1}, v, t+(n-1)) \\
\rightarrow P(u, v, t+n), $

The Cyclic Temporal Logical Rule (CTL) strictly follows the temporal-ordered constraint to collect temporal walks and represents the evolution feature of multi-hop relation reasoning. TLogic learns the confidence of cyclic temporal logical rules through statistical frequency and selects high-confidence paths as reasoning rules, such as: $(E_1, instigates, E_2, t) \wedge (E_2, declares, E_1, t+1) \wedge (E_1, instigates, E_2, t+2) \rightarrow (E_1, protests, E_2, t+3)$.

% When the graph data is sparse, the efficiency of random walk-based temporal path sampling methods is low, and it is necessary to design specific sampling methods for different reasoning tasks to improve model training efficiency. T-EDGE~\cite{T-edge} designed a temporal constraint sampling method for weighted graphs, where entities connected by high-weight edges have a higher probability of being sampled. FiGTNE~\cite{liu2020towards} proposed a time-enhanced random walk sampling method, which dynamically changes the sampling probability based on the number of times an entity has been sampled to avoid bias in path collection and better capture the evolutionary patterns of temporal knowledge graphs. ATGEB~\cite{wu2021node} believes that the activity level of entity evolution is uneven, and ranks the active time of entities, and uses DBSCAN for unsupervised clustering to obtain several active time periods for sampling walks within those periods.

% The above methods are all heuristic path sampling methods, which cannot learn patterns from data and adaptively sample temporal paths. HIN\_DRL~\cite{meilian2020hin_drl} considers that different types of entities in the knowledge graph have different characteristics, and these characteristics will continue to evolve. Therefore, HIN\_DRL proposes a meta-path sampling method that combines entity type and temporal information. During sampling, the transition probability between entities is dynamically calculated based on their entity type and the temporal information of their relationships. Experimental results show that, compared with random walk sampling methods, HIN\_DRL can capture rich semantic and evolutionary information in the graph. TITer~\cite{sun2021timetraveler} and CluSTeR~\cite{li2021search} design reinforcement learning-based temporal path sampling methods, which design policy functions to encourage the efficient search for inference paths that lead to the correct answer.

% DHNE~\cite{yin2019dhne} is applied to dynamic node classification tasks by constructing a Historical-Current subgraph of the target entity's neighbors prior to time t, which includes the target entity's neighbor information at the current time t and historical snapshots. DHNE learns the weight of the influence of the historical neighbors in the Historical subgraph $(G_{t-1}, G_{t-2}, G_{t-3})$ on the target entity at time t and adaptively samples time-constrained meta-paths based on the influence weight in the Historical-Current subgraph. The Skip-Gram path encoding method is used to calculate the vector representation of entity t at time t, in order to predict the entity's category at time $t+1$.

To extract reasoning rules from sampled temporal paths, it is necessary to encode temporal information in the paths. 
% The Skip-gram based temporal path encoding method can only learn co-occurrence relationships among entities in the sampled paths, but cannot reflect time information such as the time difference between adjacent temporal edges and the temporal order between edges. 
TITer~\cite{sun2021timetraveler} and CluSTeR~\cite{li2021search} use LSTM-based temporal path encoders to learn temporal order relationships. xERTE~\cite{han2021explainable} collects temporal paths from the target entity and propagates attention scores along the paths while continuously expanding the query subgraph. xERTE designs a temporal relation graph attention mechanism to guide expansion in the direction that benefits query prediction and the expanded subgraph can be viewed as an explanation for predicting the entity.

% In summary, the temporal path reasoning method based on temporal constraints samples paths with temporal dependency relationships to mine reasoning rules contained in the paths. Temporal paths are essentially a chain of events that contains part of the evolution rules of the knowledge graph. However, only the temporal order between adjacent temporal edges is guaranteed in the event chain, and it cannot ensure the existence of causal relationships between events. Extracting purer causal relationships from temporal paths can help to mine the essential rules of knowledge graph evolution.

\textbf{Temporal Point Process-based Prediction Methods.}
The temporal Point Process (TPP) is a probabilistic method for predicting future events. The TPP-based prediction methods treat the occurrences and disappearances of relations between entities as sequences of events, where the event probability depends on the historical evolution characteristics of relevant entities.

In TPP-based prediction methods, the expected existence probability of knowledge at time $t$ is represented as the product of the conditional intensity function and the survival function, i.e., $f(t)=S(t)\lambda(t)$. The survival function $S(t)$ evaluates the conditional probability that events do not exist in the time window $[t, t+\Delta t)$. 
 The conditional intensity function $\lambda(t)$ represents the expected existence probability in the time window $[t, t+\Delta t)$ at time $t$, given the event history information $H(t)$.

$$\lambda (t | H(t)){dt}=\mathbb{E}[N(t, t+dt) | H(t)]$$


% The conditional intensity function is key to the temporal point process, providing the ability to predict the future based on historical data. 
% Different methods such as Poisson Process, Hawkes Process, Rayleigh Process, and Neural Point Process~\cite{yan2019modeling} have proposed different modeling methods for the conditional intensity function.

% When inferring temporal knowledge $(u,v,t)$ for a single relationship, temporal point process-based methods first use historical interaction data of entities to calculate the vector representations of entities, $u_t$ and $v_t$, using temporal point process methods at time t. By calculating the dot product of entity vectors, the conditional intensity function of temporal edges is computed, and the expected occurrence probability is calculated in conjunction with the survival function. In 2016, Dai et al.~\cite{dai2016deep} proposed the Deep Coevolutionary Network, which was the first to use temporal point processes for relation inference tasks. They proposed a framework based on the interaction process to continuously update the representations of user and item entities, using an RNN model to encode the evolution of user and item representations, and using the joint non-negative likelihood probability function based on Rayleigh processes to calculate the loss. By modeling the evolution information in the knowledge graph, the deep coevolutionary network achieved better results than traditional temporal point process inference methods in item recommendation and click time recommendation (corresponding to entity inference and time point inference tasks, respectively) in the recommendation system. HTNE~\cite{HTNE} used attention mechanisms to model the influence of historical neighbors on entities at different time periods and used Hawkes processes to model the sequential generation process of entity neighbors. MTNE~\cite{huang2020motif} believed that the mesoscopic dynamic structure can better model the evolutionary interaction process of knowledge, and used the open triad motif based on Hawkes processes to reconstruct the probability as the loss function to train entity representations and learn the evolutionary rules contained in the mesoscopic dynamic structure.

Know-evolve~\cite{Know-evolve} first applies TPP to multi-relation reasoning. It treats transient knowledge $(u,r,v,t)$ as a probability event. It uses a loss function based on a multivariate Rayleigh point process to model the event probability.
The Graph Hawkes Neural Network (GHNN)~\cite{han2020graph}  can effectively aggregate information from current entity neighbors to predict the future.
% Unlike the parameterized temporal point process models mentioned above that rely on hand-designed conditional intensity functions, neural point process methods use neural networks to simulate the conditional intensity function. When prior knowledge is lacking or data features are numerous, the distribution is complex, and the true conditional intensity function cannot be predicted, neural networks can fit the true conditional intensity function from a data-driven perspective, mining hidden temporal knowledge evolution patterns and leading to stronger prediction performance.

For effectively learning the evolution of temporal knowledge graphs in a data-driven approach rather than the pre-defined conditional intensity function, neural temporal point processes have become a popular research direction for TPP-based prediction methods. 
% Representative works including DyRep, M$^2$DNE, TDIG, and EvoKG have discovered the applications of neural temporal point processes mechanism.
%TODO 这里补一个DyRep的示意图
% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=1\columnwidth]{img/figure_DyRep.png}
% 	\caption{TBD DyRep}
% 	\label{fig:figure_DyRep}
% \end{figure}

DyRep~\cite{trivedi2018dyrep} models both long-term(association) and short-term(communication) knowledge between individuals in social networks. The former reflects the changes in the network topology, representing stable relations, while the latter represents temporary, instant interactions. The events that occur are propagated through three information propagation modes: Localized Embedding Propagation, Self-propagation, and Exogenous Drive.
DyRep uses neural networks to model the conditional intensity function $\lambda_k^{(u,v)}(t)$, which calculates the probability of the existence of associated knowledge between entities (u,v) at time t (k denotes the relation type). 
% The model parameters are updated using a loss function based on conditional density and survival probability. Here, $w_k$ is the vector representation of the relationship type $k$, and $\psi_k$ is the scalar time-scale parameter corresponding to the relationship type $k$:

% \begin{equation}
% \begin{gathered}
% \lambda_k^{u, v}(t)=f_k\left(g_k^{u, v}(\bar{t})\right) \\
% g_k^{u, v}(\bar{t})=\omega_k^T \cdot\left[z^u(\bar{t}) ; z^v(\bar{t})\right] \\
% f_k(x)=\psi_k \log \left(1+\exp \left(\frac{x}{\psi_k}\right)\right)
% \end{gathered}
% \end{equation}

% Empirical studies show that due to modeling more complex information propagation mechanisms, DyRep achieves better performance than the Know-evolve model in both relationship inference tasks and time point inference tasks.

M$^2$DNE~\cite{lu2019temporal} learns entity representations by modeling evolutionary trends at both macro and micro levels. At the macro level, M$^2$DNE imposes temporal dependency constraints on entity representations, such as the number of newly added knowledge at time $t$ is determined by the number of knowledge at $t-1$. At the micro level, M$^2$DNE captures the evolutionary patterns of entity pairs, using a neural network-based conditional intensity function to calculate the probability of knowledge.
Similarly, TDIG~\cite{TDIG} and EvoKG~\cite{EvoKG}  both use graph neural networks and gated recurrent neural networks to model neural temporal point processes for tasks such as relation inference and temporal information reasoning.

% In summary, inference methods based on temporal point processes treat temporal knowledge as an asynchronous event sequence in the continuous time domain and use the conditional intensity function and survival function in the loss function to calculate the confidence of knowledge at time $t$. Since time is a parameter of the density function, this type of method belongs to the interpolation inference method ~\cite{dai2016deep} and can predict the probability of knowledge occurrence at any time with flexibility in the prediction format. However, this type of method has the cold-start problem~\cite{liu2020towards}, and cannot learn high-quality representations for entities with sparse knowledge, leading to poor inference performance.

\textbf{Sequence Neural Network-based Prediction Methods.}
Due to the powerful learning ability of neural networks, both static and dynamic knowledge reasoning methods based on neural networks have been proven to effectively learn semantic and structural features of knowledge graphs for reasoning. 
% Inference methods based on sequence neural networks view temporal knowledge graphs as discrete dynamic graphs, and use neural networks to extract features of snapshot sequences in the discrete dynamic graphs to learn the evolution information.
Sequence neural network-based prediction methods consist of snapshot encoders and temporal encoders: snapshot encoders extract representations of entities at different times from the snapshot sequence; temporal encoders integrate the snapshot representations to learn the entity evolution information from them.

% These methods assume that the constantly changing entity representations reflect the evolution pattern of the temporal knowledge graph, and attempt to explore this evolution pattern from the representations of entities at different times. 
Based on the types of temporal encoders, these methods can be divided into RNN-based temporal encoding methods and self-attention-based temporal encoding methods.

% Dyngraph2vec~\cite{goyal2020dyngraph2vec} proposed uses the autoencoder to extract knowledge graph snapshot features, and simply concatenates the entity representations at time $t$ and before as historical information. The latter two combinations both use RNN as the temporal encoder. Compared to the simple concatenation of the sequence, RNN can better capture the temporal dependencies between snapshots and achieve better performance in relationship inference tasks. 

\textit{RNN-based Temporal Encoding Methods.} RE\_NET~\cite{jin2019recurrent} aggregates the representations of entity neighbors in historical time steps, concatenates them with the vector representations of the head entity $s$ and relation $r$, encodes the evolving information through RNN to obtain the latest representation of the tail entity, which is used to predict the correct entity in the next time step.
To better learn the topological features of knowledge graphs at each stage, RE-GCN~\cite{RE-GCN} uses a relation-aware graph convolutional network (RGCN) to encode snapshot features in the knowledge graph and then learns the evolution patterns of features through a recurrent neural network. 
CEN~\cite{CEN} considers the length diversity and temporal variability of temporal patterns. It encodes multiple lengths using a relation-aware graph convolutional network to model the length diversity and trains the model online to address temporal variability. 
HiSMatch~\cite{HiSMatch} uses relation-aware graph neural networks and recurrent neural networks to distinguish between graph sequences relevant to queries and those relevant to candidate entities and proposes a matching framework for temporal reasoning. 
However, recurrent neural networks suffer from the problem of information forgetting when encoding long-distance temporal information and perform poorly in multi-step prediction tasks~\cite{DGNN5}.

% \textbf{CNN-based temporal encoding methods.} Convolutional neural networks (CNNs) have the excellent capability for extracting local features, and the weight-sharing feature can effectively reduce the number of model parameters. STGCN~\cite{STGCN} uses Graph CNN and Temporal CNN modules to respectively extract and fuse spatial and temporal features in traffic networks for predicting dynamic changes in traffic flow.
% % Compared to traditional sequence prediction models such as ARIMA, STGCN increased the MAPE indicator by 5.5\% while reducing the number of parameters.
% DynGraphGAN~\cite{xiong2019dyngraphgan} and TNDCN~\cite{wang2020generic} also use CNNs to encode the temporal sequence features in the evolution process of knowledge graphs. However, the local feature perception of CNNs leads to limited effectiveness in encoding long-distance time series.



\begin{table*}[t]
\begin{center}
\caption{Overview of Knowledge Graph Reasoning Methods.}\label{table:KG_Reasoning}
\footnotesize
\renewcommand{\arraystretch}{0.8} % 减少行间距
\setlength{\tabcolsep}{4pt} % 减少列间距
\begin{tabular}{l|p{3.6cm}|p{6cm}|p{5cm}}
\toprule
 \textbf{KG Type} & \textbf{Method Category} & \textbf{Description} & \textbf{Representative Methods} \cr 
\midrule
 \multirow{10}{*}{Static KG}& Matrix decomposition-based Methods& Adopt matrix decomposition operations to obtain the embedding of entities and relations & RESCAL\cite{RESCAL}, DISTMULT\cite{DISTMULT}, ComplEx\cite{ComplEx}, SimplE\cite{SimplE}
 \cr
 \cmidrule{2-4}
 & Translation-based Methods& Model relations as translation operations in the embedding space & TransE\cite{TransE}, TransH\cite{TransH}, TransR\cite{TransR}, RotatE\cite{RotatE} \cr
 \cmidrule{2-4}
 & GNN-based Methods& Use GNNs with aggregation operation to obtain the embeddings for reasoning & GCN\cite{GCN}, R-GCN\cite{RGCN}, CompGCN\cite{CompGCN} \cr
 \cmidrule{2-4}
 & LLM-based Methods& Transform KG into sequence, and adopt pre-trained LLMs for reasoning & KBERT\cite{KBERT}, CKBC\cite{CKBC}, KG-BERT\cite{KG-BERT}, StAR\cite{StAR}, MTL-KGC\cite{DBLP:conf/coling/KimHKS20} \cr
 \cmidrule{2-4}
 & Neural-symbolic & Combine the advantages of neural networks and symbolic logic reasoning & KALE\cite{KALE}, RUGE\cite{RUGE}, PRA\cite{PRA}, MINERVA\cite{MINERVA}, GraIL\cite{GraIL} \cr
\midrule

 \multirow{6}{*}{Dynamic KG}& 
 GNN-based Methods& Use GNN to capture inductive information and transfer it to new components  & DRUM~\cite{sadeghian2019drum}, TACT~\cite{TACT}, LAN~\cite{LAN}, MaKEr~\cite{MaKEr}, SE-GNN~\cite{SE-GNN} \cr
 \cmidrule{2-4}
 & LLM-based Methods& Convert DKG into sentences and obtain pre-trained prior knowledge from LLMs  & KEPLER~\cite{KEPLER}, BERTRL\cite{BERTRL}, Bi-Link~\cite{Bi-Link}   \cr
 \cmidrule{2-4}
 & Few-shot Methods& Transfer and adapt learned knowledge from various views to few-shot entities & FAAN~\cite{FAAN},  MetaR~\cite{MetaR}, Meta-KGR~\cite{Meta-KGR}, GEN~\cite{GEN}, REFORM~\cite{REFORM}  \cr

\midrule
 \multirow{16}{*}{Temporal KG}& Tensor Decomposition-based Completion Methods & The temporal information is regarded as one dimension of the TKG high-dimensional tensor, and the  temporal representation is obtained through tensor decomposition & TComplEX~\cite{lacroix2020tensor}, ~\cite{tresp2017embedding}, ConT~\cite{ma2019embedding},~\cite{shao2022tucker}, TIMEPLEX~\cite{TIMEPLEX}, TeLM~\cite{TeLM}, TGEOME~\cite{TGeomE}  \cr
 \cmidrule{2-4}
 & Translation-based Completion Methods & Temporal information is independent of the representation of entities and relationships and is explicitly represented as trainable vectors or projection matrices & TAE\cite{TAE2016}, TTransE~\cite{leblay}, HyTE\cite{HyTE}, TeRo~\cite{TERO}, TOKEI~\cite{leblay2020towards}, TA-TRANSE~\cite{TA-TransE}, TRESCAL~\cite{leblay}, DE~\cite{DE-SimplE}, ATiSE~\cite{ATiSE}  \cr
  \cmidrule{2-4}
 & Path-based Prediction Methods & The acquisition of temporal walks indicates the evolution law of TKG & TLogic ~\cite{TLogic}, TITer~\cite{sun2021timetraveler}, CluSTeR~\cite{li2021search}, xERTE~\cite{han2021explainable}  \cr
  \cmidrule{2-4}
 & Temporal Point Process-based Prediction Methods & The temporal knowledge as asynchronous events in a continuous time domain, and model the occurring probability of events  through temporal point process & Know-evolve~\cite{Know-evolve}, GHNN~\cite{han2020graph}, DyRep~\cite{trivedi2018dyrep}, M$^2$DNE~\cite{lu2019temporal}, TDIG~\cite{TDIG}, EvoKG~\cite{EvoKG}  \cr
  \cmidrule{2-4}
  & Sequence Neural Network-based Prediction Methods & The snapshot encoder outputs the representation of different time entities and relations, and the temporal encoder learns the evolution law in the TKG & RE\_NET~\cite{jin2019recurrent}, RE-GCN~\cite{RE-GCN}, CEN~\cite{CEN}, TeMP~\cite{TeMP}, DySAT~\cite{DGNN5}, DANE~\cite{xu2020embedding}, DACHA~\cite{chen2021dacha}, HIP~\cite{he2021hip} \cr
\bottomrule
\end{tabular}
\end{center}
\end{table*}

%TBD Temp, DySAT
\textit{Self-attention-based Temporal Encoding Methods.} The self-attention mechanism can effectively alleviate the forgetting problem in encoding long-distance time series. TeMP \cite{TeMP} uses R-GCN\cite{RGCN} as the snapshot encoder to extract the historical vector sequence of the target entity s, $x_{s,t-\tau},\ldots,x_{s,t-1},x_{s,t}$; based on the self-attention mechanism, the temporal encoder aggregates the historical vector sequence with weights to obtain the vector representation $z_{s,t}$ of entity s at time t. 
% The self-attention mechanism for time information can perceive the information of the entire time series, and can encode long-distance time information to alleviate the forgetting problem. In addition, TeMP also designs historical weight coefficients $\alpha_s$ to comprehensively consider the current entity encoding information and historical entity encoding information at the current time. 
Furthermore, DySAT\cite{DGNN5}  proposes a structural-temporal attention mechanism. The structure self-attention mechanism extracts features from the entity neighborhoods in each snapshot and aggregates them with weights, while the temporal self-attention mechanism captures the evolution law by flexibly weighting the historical entity representations of multiple time steps. Moreover, DANE\cite{xu2020embedding}, DACHA\cite{chen2021dacha}, HIP\cite{he2021hip} also design structure-temporal self-attention mechanisms, which are applied to the entity and relation prediction tasks.

% In summary, due to the powerful learning ability of neural networks, inference methods based on sequence neural network models can effectively learn the dynamic evolution patterns of entities. However, such methods strongly rely on training data, and the model performance is poor when the training data is insufficient. In addition, the lack of interpretability in inference due to the black-box nature of neural networks is also a problem for this type of method.

% \begin{table*}[t]
% \begin{center}
% \caption{Summary of Knowledge Graph Reasoning Methods}\label{table:KG_reasoning}
% \begin{tabular}{l|p{2cm}|p{1cm}|p{4cm}|p{2cm}|p{2cm}}
% \toprule
%  KG Type & Method & Year & Description & Technique & Learning Style (X) \cr 
% \midrule
% \multirow{4}{*}{SKG} & RESCAL~\cite{RESCAL} & 2018 & XXXXX & Matrix Decomposition & Inductive\cr
% \cmidrule{2-6}
% & Method B & YYYY & XXXXX & Technique B & Transductive\cr
% \cmidrule{2-6}
% & ... & ... & ... & ... & ...\cr
% \midrule
% \multirow{4}{*}{DKG} & Method C & YYYY & XXXXX & Technique C & Inductive\cr
% \cmidrule{2-6}
% & Method D & YYYY & XXXXX & Technique D & Transductive\cr
% \cmidrule{2-6}
% & ... & ... & ... & ... & ...\cr
% \midrule
% \multirow{4}{*}{TKG} &  TComplEX & 2020 & Representing the temporal knowledge graph as a four-dimensional tensor and using CP decomposition method & Tensor Decomposition-based Completion Method & Inductive\cr
% \cmidrule{2-6}1111111111111111111111111111111111111111112
% & TIMEPLEX & 2020 &  Considering the periodicity
% scores and temporal dependency scores of the relations in
% the reasoning procedure & Tensor Decomposition-based Completion Method & Transductive\cr
% \midrule
% & HyTE & 2018 &  Designing the time hyperplane to reflect the entity and relation information at a specific time & Translation-based Completion Method & Transductive\cr
% \midrule
% & TOKEI & 2020 &  Designs the hierarchical temporal matrix that is adaptable to different time granularities  & Translation-based Completion Method & Transductive\cr
% \midrule
% & TRESCAL & 2018 &  Considering that the information
% of relations evolves over time, and the temporal information depends on the existence of the relationship  & Translation-based Completion Method & Transductive\cr
% \midrule
% & TLogic & 2022 & Considering the temporal properties
% of multi-hop relation reasoning and proposes the Cyclic
% Temporal Logical Rule  & Path-based Prediction Method & Inductive\cr
% \midrule
% & Know-evolve & 2019 & Treating knowledge (u, r, v, t) as a probability event, and uses a loss function based on a multivariate Rayleigh point process  & Temporal Point Process-based Prediction Method & Transductive\cr
% \midrule
% & RE\_NET & 2019 & Encoding the
% history information through RNN to obtain the latest
% representation of the tail entity  & Sequence Neural Network-based Prediction & Transductive\cr
% \midrule
% & TeMP & 2021 & Using R-GCN as the snapshot encoder to extract the historical vector sequence of the target entity & Sequence Neural Network-based Prediction & Transductive\cr
% \midrule
% \cmidrule{2-6}
% & ... & ... & ... & ... & ...\cr
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table*}

==> sections/bak/sec4.3_bak.tex <==
\subsection{Temporal Knowledge Graph Reasoning}~\label{sec:4.3}
The reasoning  task of temporal knowledge includes two parts\cite{vila1994survey}: the explanation of  the world at some past time and the determination of  the world at a given future time. Based on this, this paper classifies the methods for temporal knowledge graph reasoning into two categories: temporal knowledge graph reasoning methods for completion and prediction. The following sections will provide detailed introductions to these two types of methods.

\subsubsection{Temporal Knowledge Graph Completion}
The key to the completion task of temporal knowledge graphs is to enable the model to understand the time information and integrate it into the complex semantic and structural information in the knowledge graph for reasoning. Reasoning methods for completion tasks learn the representation of entities at specific moments to complete missing knowledge, which can be divided into tensor decomposition-based completion methods, and translation-based completion methods.

The completion method based on tensor decomposition learns the evolution law of the entire graph from a macroscopic perspective, obtaining the representation of entities, relations, and time through predefined decomposition methods.

The completion method based on transition representation learns the evolution law of entities from a microscopic perspective, obtaining the representation of entities, relations, and time from temporal knowledge data. The rule-based reasoning method expresses reasoning rules explicitly and deduces missing knowledge through the knowledge already in the graph. The above methods are utilized to complete the task of temporal knowledge graph completion.

\textbf{Tensor Decomposition-based Completion Methods.}
As the temporal knowledge graph is represented as discrete dynamic forms, each snapshot of the knowledge graph can be modeled as a sequence of matrices or high-dimensional tensors. The corresponding vectors of entities and time are obtained by tensor decomposition, and the hidden knowledge is mined by reconstructing the tensor. The element values in the reconstructed tensor represent the confidence scores of the corresponding knowledge, achieving completion of the temporal knowledge graph.

Parallel decomposition-based inference does not focus on the state of the temporal knowledge graph at a particular moment, but directly stacks snapshots into high-dimensional tensors, treating time as one dimension. The representations of entities and time are obtained by one-time tensor decomposition. The dot product of the corresponding entity and time representations yields the representation of the entity at a specific time. The representative methods for high-dimensional tensor decomposition are CP decomposition~\cite{1927The} and Tucker decomposition~\cite{tucker1966some}. The former decomposes high-dimensional tensors into a series of rank tensors, and the latter, based on CP decomposition, considers the core tensor, which represents the main properties of the original tensor, like the principal component factors in PCA. When the core tensor is a hyper-diagonal matrix, Tucker decomposition is a special case of CP decomposition.

Dunlavy et al. ~\cite{dunlavy2011temporal} and UPD~\cite{rafailidis2014modeling} modeled the dynamic social interaction network and the user-item network in the recommendation system as a 3D real tensor $G \in R^{|E|\times|E|\times|T|}$ and decomposed it using CP decomposition to obtain the representations of entities and time. Lacroix et al.~\cite{lacroix2020tensor} represented the temporal knowledge graph as a 4D real tensor $G \in R^{|E|\times|R|\times|E|\times|T|}$ and extended the non-temporal knowledge graph inference method ComplEX to the temporal knowledge graph inference, proposing the CP decomposition method TComplEX based on the complex field. TComplEX achieved better performance in entity inference tasks.

Compared to CP decomposition, Tucker decomposition has better inference performance, but its decomposition efficiency is lower due to the operations involving the core tensor. Tresp et al. ~\cite{tresp2017embedding} and ConT~\cite{ma2019embedding} used a 4th-order Tucker decomposition to obtain the representations of entities, relationships, and time. Shao et al.~\cite{shao2022tucker} added regularization constraints on the distance between adjacent time vectors based on Tucker decomposition. TIMEPLEX~\cite{TIMEPLEX} considered that different relationships may have different temporal properties, such as some relationships being periodic (e.g., the "Olympic Games" relationship appearing every four years), and there may be temporal dependencies among different relationships. Based on the work of Tresp et al. ~\cite{tresp2017embedding}, TIMEPLEX considered the periodicity scores and temporal correlation scores of the relationships when inferring the temporal knowledge, thus achieving better performance in entity and time inference tasks.

In summary, tensor decomposition-based inference methods learn the evolution rules of temporal knowledge graphs from the entire graph perspective and obtain semantic representations of entities, relationships, and time by decomposition. This type of method is relatively mature and has stable performance. However, tensor decomposition algorithms have high time complexity and occupy a large amount of computing resources, making it difficult to apply to large-scale knowledge graph data. Moreover, this type of method has poor flexibility and can only learn representations for entities and time points that appear in the training set, lacking generalization representation ability and limited application performance.

\textbf{Translation-based Completion Methods.}
This type of method is similar to the translation-based representation method of static knowledge graphs. The representation of entities, relations, and time elements is not decomposed, but is learned in the form of vectors, matrices, and other representations that map to high-dimensional semantic space (this process is called transfer representation) to fit the semantic and temporal features in temporal knowledge graphs.
Compared to the transfer representation method in static knowledge graphs, this method needs to consider how to transfer time information to high-dimensional semantic space to reflect the dynamic evolution of the graph or individual. According to the different ways of representing time information, this paper categorizes transfer-based reasoning methods into two types: reasoning with explicitly represented time information and implicitly represented time information.

\textit{Completion with Explicit Time Information.}
Reasoning methods with explicit time information represent the time information in temporal knowledge graphs in the form of temporal transition matrices, embedded vectors, and time mapping matrices.
The representation of time is independent of the representation of entities and relations, and represents the evolutionary information of the temporal knowledge graph at each moment from a macroscopic level.
The representation of entities and relations is static and remains unchanged, independent of time.

Reference~\cite{TAE2016} observes that there is temporal information between the relationships of the same entity, such as the temporal sequence of \textit{(Albert Einstein, born in, Ulm, 1879)}, \textit{(Albert Einstein, awarded, Nobel Prize in Physics, 1922)}, and \textit{(Albert Einstein, passed away in, Princeton, 1955)} represent the temporal sequence of \textit{born in, awarded, passed away}. Considering that this temporal sequence information can better describe the dependence properties between relationships, the Temporal Attentional Embedding (TAE) model is proposed. Based on the classic transition representation model, the TAE model incorporates the temporal information of relationships using a temporal matrix to learn relationship representations that contain temporal information. Building on TAE, TAE-ILP~\cite{jiang2016towards} considers the effective time intervals of knowledge and uses Integer Linear Programming (ILP) to restrict the temporal knowledge of shared head entities to non-overlapping time intervals.

TAE and TAE-ILP only extract temporal information to better learn the representation of relationships, and the model cannot utilize specific time information. Leblay et al.~\cite{leblay} proposed the TTransE model, which was the earliest work to add time information representation to the transition representation model. Specifically, TTransE adds and learns the representation of time information based on the classical static knowledge reasoning model TransE. By combining the representation of entities, relationships, and time to calculate confidence, the representation of entities and relationships is completely disconnected from the representation of time information, making it difficult to accurately reflect the entity and relationship information at a specific moment. Based on this, Dasgupta et al.~\cite{HyTE} proposed the temporal hyperplane method HyTE.

%TODO 这里补一个HyTE的示意图
\begin{figure}[h]
	\centering
	\includegraphics[width=1\columnwidth]{img/figure_HyTE.png}
	\caption{TBD HyTE}
	\label{fig:figure_HyTE}
\end{figure}

As shown in Figure~\ref{fig:figure_HyTE}, in the reasoning process, HyTE transfers the head entity, relationship, and tail entity vectors $e_h$, $e_r$, and $e_t$ to the corresponding hyperplane in the high-dimensional space at the time information $T_1$, $T_2$ to obtain the entity and relationship representation at a specific moment. This time modeling method can effectively help the model to distinguish time-sensitive relationships, such as "born in" and "passed away in" relationships, and achieve better performance in knowledge-level reasoning tasks, especially relationship prediction tasks. To enhance the representation ability of the transition representation and reflect the evolutionary process of entity information in the temporal knowledge graph, TeRo~\cite{TERO} represents time as complex vectors and defines the representation of entities at different moments as rotation in the complex vector space, which is the Hermitian dot product of entity complex vectors and time complex vectors, to reflect the evolutionary process of entities.

%TODO 这里补一个TOKEI的示意图
\begin{figure}[h]
	\centering
	\includegraphics[width=1\columnwidth]{img/figure_TOKEI.png}
	\caption{TBD TOKEI}
	\label{fig:figure_TOKEI}
\end{figure}

The temporal information in knowledge graphs can be represented at different granularities, for example, temporal information such as \textit{(Germany, capital, Berlin, 1980s)} and \textit{(Germany, capital, Berlin, January 16, 1989)} have granularities at the level of decade and day, respectively.
To address this issue, TOKEI~\cite{leblay2020towards} designed a mapping matrix that is adaptable to different time granularities based on a custom hierarchical system for time information (e.g., year-month-day or year-quarter-month-week-day).
As shown in Figure~\ref{fig:figure_TOKEI}, the same entity or relation is represented by different mapping matrices for \textit{1980s} and \textit{January 16, 1989} at different time granularities to calculate the knowledge confidence score under different granularities.

TA-TRANSE~\cite{TA-TransE} model takes into account that temporal information at different granularities is of unequal lengths, such as \textit{1989} with the granularity of year and \textit{January 16, 1989} with the granularity of day. It converts temporal information into a sequence of time tokens, such as converting \textit{January 16, 1989} into \textit{[1989, 1, 16]}, and uses an LSTM to encode the unequal length sequence as the temporal information of knowledge on top of TransE. This approach can effectively inject time information into relations and achieves better performance in entity inference tasks compared to static knowledge reasoning models.

However, the aforementioned methods ignore the correlation between temporal information. TeLM~\cite{TeLM} assumes that time is a linear transformation, and the difference between representations of adjacent moments should be as small as possible. Based on this, TeLM introduces a temporal smoothing mechanism into the loss function, which constrains the change in the vector representation of adjacent moments. Similarly, TIME2BOX~\cite{cai2021time} and RTGE~\cite{RTGE} also use temporal smoothing mechanisms to constrain the change in adjacent time vectors. Experimental results demonstrate that the temporal smoothing mechanism effectively captures the correlation between adjacent time points, and that the vectors of adjacent times are closer in high-dimensional space, indicating a better representation of the temporal correlation.

In summary, in the temporal knowledge graph reasoning methods with explicit representation of time, the representation of time is independent of the representation of entities and relations, and it contains macroscopic evolutionary information of the temporal knowledge graph at that moment. This type of method requires training the corresponding representation for all temporal information in the training set and is not suitable for knowledge graphs that are frequently changing and have rich temporal information. When the granularity of temporal information is too fine, although it can improve the reasoning performance of the model, it can also result in a large amount of training computational overhead.

\textit{Completion with Implicit Time Information.}
The reasoning of implicitly represented time information models the evolution of entities or relationships with time as functions, which can reason the evolution trend of each entity at each moment.
The time information is incorporated in the representation of entities or relationships, but does not have an explicit representation on its own. TRESCAL~\cite{leblay} extends the static knowledge graph reasoning method RESCAL~\cite{RESCAL} to temporal knowledge graph reasoning, which considers that the information of relationships will evolve over time, and the time information depends on the existence of the relationship. For each type of relationship, the mapping matrix $W_{r,t}$ is trained at different moments. However, the combination of relationship and time is enormous, which means that TRESCAL has high temporal and spatial complexity, and cannot learn the correlation of time information. DE~\cite{goel2020diachronic} proposes a diachronic embedding method in that both entities and relationships should be represented as functions of time, changing over time. Based on this, it uses a parameterizable Fourier function sequence to encode the entity and relationship vectors at any time, and this encoding method has been proven to reflect the correlation between time information, effectively modeling the linear and periodic changes in the evolution process, and significantly reducing the number of model parameters. Compared to the TTransE and HyTE models, the MRR indicator in the entity inference task is increased by an average of 19.4\%. 

Similarly, ATiSE~\cite{ATiSE} also represents entities and relationships as functions of time, considering uncertainty in the evolution process, and adding random noise to the representation of entities and relationships to simulate random interference factors. It conducts reasoning by learning the parameters of a multi-dimensional Gaussian distribution composed of three factors: linear trend, periodic trend, and noise. The above reasoning methods directly model entities and relationships as functions of time, making the reasoning process a black box without interpretability. T-GAP~\cite{T-GAP} attempts to give the model interpretability: starting from the target entity $u$ in the incomplete knowledge $(u,r,?,t)$, it iteratively expands the subgraph using attention pruning strategies and dynamically updates the representations and attention scores of each entity in the subgraph through a time-aware graph neural network. The attention score can explain the reasoning process to some extent. After the expansion process ends, the entity with the highest attention score in the subgraph is chosen as the correct answer for completion. In summary, reasoning with implicitly represented time information assumes that the representation of entities or relationships dynamically changes over time, and does not require an explicit representation method specifically designed for time. Such methods model the evolution features of specific entities or relationships over time at a microscopic level, which has greater flexibility. However, when the observable time span of the knowledge graph is large, it is often difficult to train high-quality entity representations~\cite{T-GAP}.

\subsubsection{Temporal Knowledge Graph Prediction}
Temporal knowledge graph prediction methods aim to learn the unidirectional evolution patterns of TKG historical information to predict future states.
These methods can be further categorized based on how they model the unidirectional evolution patterns, including path-based prediction methods, point process-based prediction methods, and sequence network-based prediction methods.

\subsubsection{Path-based Prediction Methods}
Due to the graph nature of temporal knowledge graphs, the sampled time-constrained random walk paths in temporal knowledge graphs can be viewed as multi-hop relations between entities and to some extent represent reasoning rules.

As the relationships between entities have temporal dynamics, time constraints should be considered when collecting traversal paths. Based on the constraints obeyed during path collection, path-based reasoning methods can be divided into snapshot-based path reasoning and temporal-constraint-based path reasoning. For the former, the temporal information within a path is the same because the collected paths are constrained within a snapshot. For the latter, the temporal information within a path follows certain rules to reflect the evolution of the graph.

The path-based prediction methods of temporal knowledge graphs mainly follow the time-constrained random walk module, which believes that temporal order information reflects the evolution rules of entities.
These methods consider the unidirectional property of time when sampling paths, and sample paths that follow temporal constraints to learn the unidirectional evolution rules of the knowledge graph over time in order to predict the future.

The concept of the temporal walk was first proposed by CTDNE~\cite{nguyen2018dynamic}. In a temporal walk, the adjacent temporal edges should satisfy the time-sequential constraint relationship, ensuring that the sampled path contains the temporal dependency information of dynamic interactions between entities. For a temporal path of length $L$ $(v_{i_1}, v_{i_2}, t_{i_1}), (v_{i_2}, v_{i_3}, t_{i_2}), ..., (v_{i_L}, v_{i_{L+1}}, t_{i_L})$ the partial order of time information in the path is $t_{i_1} \leq t_{i_2} \leq ... \leq t_{i_L}$.
Experimental results show that compared to random walk methods that do not consider temporal constraints, CTDNE improves the AUC score by 15.6\% in knowledge reasoning tasks.

The sampling method with temporal constraints can extract the temporal-dependent topological features in a knowledge graph in an unsupervised manner. Liu et al. ~\cite{TLogic} considered the temporal properties of multi-hop relationship reasoning and proposed the concept of Cyclic Temporal Logical Rules, represented as:

$P_1(u, z_1, t) \wedge P_2(z_1, z_2, t+1) \wedge \ldots \wedge P_n(z_{n-1}, v, t+(n-1)) \\
\rightarrow P(u, v, t+n), $

The proposed concept of Cyclic Temporal Logical Rules (CTL), which strictly follows the temporal increment constraint, considers the temporal properties of multi-hop relation reasoning.
Based on the CTL, the author proposed the TLogic model. uses frequency statistics to learn the confidence of cyclic temporal logical rules and selects high-confidence paths as reasoning rules. In the ICEWS international political event knowledge graph, TLogic can mine cyclic temporal logical rules such as: $(E_1, instigates, E_2, t) \wedge (E_2, declares, E_1, t+1) \wedge (E_1, instigates, E_2, t+2) \rightarrow (E_1, protests, E_2, t+3)$ to infer the future development trend of events.

When the graph data is sparse, the efficiency of random walk-based temporal path sampling methods is low, and it is necessary to design specific sampling methods for different reasoning tasks to improve model training efficiency. T-EDGE~\cite{T-edge} designed a temporal constraint sampling method for weighted graphs, where entities connected by high-weight edges have a higher probability of being sampled. FiGTNE~\cite{liu2020towards} proposed a time-enhanced random walk sampling method, which dynamically changes the sampling probability based on the number of times an entity has been sampled to avoid bias in path collection and better capture the evolutionary patterns of temporal knowledge graphs. ATGEB~\cite{wu2021node} believes that the activity level of entity evolution is uneven, and ranks the active time of entities and uses DBSCAN for unsupervised clustering to obtain several active time periods for sampling walks within those periods.

The above methods are all heuristic path sampling methods, which cannot learn patterns from data and adaptively sample temporal paths. HIN\_DRL~\cite{meilian2020hin_drl} considers that different types of entities in the knowledge graph have different characteristics, and these characteristics will continue to evolve. Therefore, HIN\_DRL proposes a meta-path sampling method that combines entity type and temporal information. During sampling, the transition probability between entities is dynamically calculated based on their entity type and the temporal information of their relationships. Experimental results show that, compared with random walk sampling methods, HIN\_DRL can capture rich semantic and evolutionary information in the graph. TITer~\cite{sun2021timetraveler} and CluSTeR~\cite{li2021search} design reinforcement learning-based temporal path sampling methods, which design policy functions to encourage the efficient search for inference paths that lead to the correct answer.

DHNE~\cite{yin2019dhne} is applied to dynamic node classification tasks by constructing a Historical-Current subgraph of the target entity's neighbors prior to time t, which includes the target entity's neighbor information at the current time t and historical snapshots. DHNE learns the weight of the influence of the historical neighbors in the Historical subgraph $(G_{t-1}, G_{t-2}, G_{t-3})$ on the target entity at time t and adaptively samples time-constrained meta-paths based on the influence weight in the Historical-Current subgraph. The Skip-Gram path encoding method is used to calculate the vector representation of entity t at time t, in order to predict the entity's category at time $t+1$.

To extract reasoning rules from sampled temporal paths, it is necessary to encode temporal information in the paths. The Skip-gram based temporal path encoding method can only learn co-occurrence relationships among entities in the sampled paths, but cannot reflect time information such as the time difference between adjacent temporal edges and the temporal order between edges. TITer~\cite{sun2021timetraveler} and CluSTeR~\cite{li2021search} designed LSTM-based temporal path encoders to learn temporal order relationships. DEMS~\cite{yuan2022dynamic} used self-attention mechanisms to consider time differences based on modeling temporal order relationships. Different weights were assigned to entities at different positions and with different time information in the path during entity representation training to better learn the association between entity topology and time information. Wang et al.~\cite{wang2021inductive} proposed the Causal Anonymous Walk (CAW), which anonymizes local structural information in the path and extracts abstract temporal evolution rules from the anonymous path. xERTE~\cite{han2021explainable} samples temporal paths from the target entity and propagates attention scores along the paths while continuously pruning and expanding the query subgraph. xERTE designed a Temporal Relation Graph Attention mechanism to guide subgraph expansion in the direction that benefits query prediction, and the expanded subgraph can be viewed as an explanation for predicting the entity.

In summary, the temporal path reasoning method based on temporal constraints samples paths with temporal dependency relationships to mine reasoning rules contained in the paths. Temporal paths are essentially a chain of events that contains part of the evolution rules of the knowledge graph. However, only the temporal order between adjacent temporal edges is guaranteed in the event chain, and it cannot ensure the existence of causal relationships between events. Extracting purer causal relationships from temporal paths can help to mine the essential rules of knowledge graph evolution.

\subsubsection{Temporal Point Process-based Prediction Methods}
Temporal Point Process (TPP) is a probabilistic modeling method for random events. The reasoning methods based on TPP treat the occurrences and disappearances of entities and relationships in temporal knowledge graphs as sequences of random events, where the probability of an event depends on the historical evolution characteristics of relevant entities, including topology structure, entity features, and time interval features of events.

In TPP-based methods, the expected existence probability of knowledge at time $t$ is represented as the product of the conditional intensity function and the survival function, i.e., $f(t)=\lambda(t)S(t)$. The conditional intensity function $\lambda(t)$ represents the expected existence probability in the time window $[t, t+\Delta t)$ at time $t$, given the event history information $H(t)$.

$$\lambda (t | H(t)){dt}=\mathbb{E}[N(t, t+dt) | H(t)]$$

The survival function $S(t)$ evaluates the conditional probability that events do not exist in the time window $[t, t+\Delta t)$. The conditional intensity function is key to the temporal point process, providing the ability to predict the future based on historical data. Different methods such as Poisson Process, Hawkes Process, Rayleigh Process, and Neural Point Process~\cite{yan2019modeling} have proposed different modeling methods for the conditional intensity function.

When inferring temporal knowledge $(u,v,t)$ for a single relationship, temporal point process-based methods first use historical interaction data of entities to calculate the vector representations of entities, $u_t$ and $v_t$, using temporal point process methods at time t. By calculating the dot product of entity vectors, the conditional intensity function of temporal edges is computed, and the expected occurrence probability is calculated in conjunction with the survival function. In 2016, Dai et al.~\cite{dai2016deep} proposed the Deep Coevolutionary Network, which was the first to use temporal point processes for relation inference tasks. They proposed a framework based on the interaction process to continuously update the representations of user and item entities, using an RNN model to encode the evolution of user and item representations, and using the joint non-negative likelihood probability function based on Rayleigh processes to calculate the loss. By modeling the evolution information in the knowledge graph, the deep coevolutionary network achieved better results than traditional temporal point process inference methods in item recommendation and click time recommendation (corresponding to entity inference and time point inference tasks, respectively) in the recommendation system. HTNE~\cite{HTNE} used attention mechanisms to model the influence of historical neighbors on entities at different time periods, and used Hawkes processes to model the sequential generation process of entity neighbors. MTNE~\cite{huang2020motif} believed that the mesoscopic dynamic structure can better model the evolutionary interaction process of knowledge, and used the open triad motif based on Hawkes processes to reconstruct the probability as the loss function to train entity representations and learn the evolutionary rules contained in the mesoscopic dynamic structure.

Know-evolve~\cite{Know-evolve} was the first work to apply temporal point processes to multi-relation categorical reasoning. It treats transient knowledge $(u,r,v,t)$ as a probability event and, in addition to representing entity vectors, models the mapping matrices representing each type of relationship. It uses a loss function based on a multivariate Riemann point process to model the probability of event occurrence in the temporal knowledge graph, serving relationship inference and temporal point prediction tasks.
Han et al.~\cite{han2020graph} proposed the Graph Hawkes Neural Network (GHNN) to model multi-relation temporal knowledge graphs, which can effectively aggregate information from current entity neighbors to predict the future.
Unlike the parameterized temporal point process models mentioned above that rely on hand-designed conditional intensity functions, neural point process methods use neural networks to simulate the conditional intensity function. When prior knowledge is lacking or data features are numerous, the distribution is complex, and the true conditional intensity function cannot be predicted, neural networks can fit the true conditional intensity function from a data-driven perspective, mining hidden temporal knowledge evolution patterns and leading to stronger prediction performance.
Currently, neural temporal point processes have become a popular research direction for inference methods based on temporal point processes. Representative works including DyRep~\cite{trivedi2018dyrep}, M$^2$DNE~\cite{lu2019temporal}, TDIG~\cite{TDIG}, and EvoKG~\cite{EvoKG} have discovered the applications of neural temporal point processes mechanism.

%TODO 这里补一个DyRep的示意图
\begin{figure}[h]
	\centering
	\includegraphics[width=1\columnwidth]{img/figure_DyRep.png}
	\caption{TBD DyRep}
	\label{fig:figure_DyRep}
\end{figure}

As shown in Figure~\ref{fig:figure_DyRep}, DyRep models both steady-state and transient relationships between individuals in social networks using two types of event knowledge: association and communication. The former changes the network topology, representing long-term stable relationships, while the latter represents temporary, short-term contacts. The events that occur are propagated through three information propagation modes: Localized Embedding Propagation, Self-propagation, and Exogenous Drive. The entity representation involved in the event is changed accordingly. The entity $v$ at time $t_p$ is represented as follows:

$$
{z}^v(t_p)=\sigma({W}^{struct } {h}_{struct }^u(\bar{t}_p)+{W}^{rec } {z}^v(\bar{t}_p^v)+{W}^t(t_p-t_p^{\bar{v}})),
$$
where ${W}^{struct }$, ${W}^{rec } $, and ${W}^t$ denote the mapping matrices of the entity neighbor aggregation information, entity self-information, and exogenous drive, respectively.
${h}_{struct }^u(\bar{t}_p)$ represents the latest neighbor structure information before time $t_p$, and ${z}^v(\bar{t}_p^v)$ represents the latest representation vector of entity $v$ before time $t_p$.

DyRep uses neural networks to model the conditional intensity function $\lambda_k^{(u,v)}(t)$, which calculates the probability of the existence of associated knowledge between entities (u,v) at time t (k denotes the relationship type). The model parameters are updated using a loss function based on conditional density and survival probability. Here, $w_k$ is the vector representation of the relationship type $k$, and $\psi_k$ is the scalar time-scale parameter corresponding to the relationship type $k$:

\begin{equation}
\begin{gathered}
\lambda_k^{u, v}(t)=f_k\left(g_k^{u, v}(\bar{t})\right) \\
g_k^{u, v}(\bar{t})=\omega_k^T \cdot\left[z^u(\bar{t}) ; z^v(\bar{t})\right] \\
f_k(x)=\psi_k \log \left(1+\exp \left(\frac{x}{\psi_k}\right)\right)
\end{gathered}
\end{equation}

Empirical studies show that due to modeling more complex information propagation mechanisms, DyRep achieves better performance than the Know-evolve model in both relationship inference tasks and time point inference tasks.

M$^2$DNE learns entity representations by modeling evolutionary trends at both macro and micro levels. At the macro level, M$^2$DNE imposes constraints on the model through network dynamical indicators, such as the number of newly added knowledge at time $t$ is determined by the number of knowledge at time $t-1$. At the micro level, M$^2$DNE captures the evolutionary patterns of entity pairs forming associations, using a neural network-based conditional intensity function $\tilde{\lambda_{i,j}}(t)$ to calculate the probability of forming edges between entity pairs:

\begin{equation}
\begin{gathered}
\tilde{\lambda}_{i, j}(t)=g\left(\boldsymbol{u}_i, \boldsymbol{u}_j\right) \\
+\beta_{i j} \sum_{p \in N^i(t)} \alpha_{p i}(t) g\left(\boldsymbol{u}_p, \boldsymbol{u}_j\right) \kappa\left(t-t_p\right) \\
+\left(1-\beta_{i j}\right) \sum_{q \in N^j(t)} \alpha_{q j}(t) g\left(\boldsymbol{u}_q, \boldsymbol{u}_i\right) \kappa\left(t-t_q\right),
\end{gathered}
\end{equation}

where $u_i$ and $u_j$ are the vector representations of entities $i$ and $j$ at time $t$. $g(.)$ is the matching function for node pairs, and $\kappa(.)$ is the time-distance function. $p$ and $q$ denote the neighbor entities of entity $i$ and $j$ at time $t$, respectively. $\alpha$ is the learned attention factor, and $\beta$ is the factor that regulates the influence of the head and tail node neighbor information.

\begin{equation}
\begin{aligned}
\lambda^{u, v}\left(t \mid H_t^{u, v}\right)= & \text { Softplus }\left(\boldsymbol{w}_{add}^{\top}\left(\overline{\boldsymbol{h}}_{u\left(t^{u-}\right)}^r+\overline{\boldsymbol{h}}_{v\left(t^{v-}\right)}^r\right)\right. \\
& \left.+\boldsymbol{w}_{m u l}^{\top}\left(\overline{\boldsymbol{h}}_{u\left(t^{u-}\right)}^r \odot \overline{\boldsymbol{h}}_{v\left(t^{v-}\right)}^r\right)+b_\lambda^{u, v}\right),
\end{aligned}
\end{equation}

where $H_t^{u, v}$ is the historical interaction data between $u$ and $v$, $\overline{\boldsymbol{h}}{u\left(t^{u-}\right)}^r$ and $\overline{\boldsymbol{h}}{v\left(t^{v-}\right)}^r$ are the latest historical representations of entities $u$ and $v$ at time $t$, $\boldsymbol{w}{a d d}$ and $\boldsymbol{w}{m u l}$ are trainable parameter vectors, and $b_\lambda^{u, v}$ is a trainable bias parameter. The loss function of TDIG is the sum of the negative log-likelihood joint probability of positive instance pairs and the survival probability of negative instance pairs:

\begin{equation}
L=-\sum_i^N \log \lambda^{u_i v_i}\left(t_i \mid H_{t_i}^{u_i v_i}\right)+\int_0^T \Sigma_{u, v} \lambda^{u, v}(t) d t
\end{equation}

Similarly, EvoKG uses graph neural networks and gated recurrent neural networks to model neural temporal point processes for tasks such as relation inference and temporal information reasoning.

In summary, inference methods based on temporal point processes treat temporal knowledge as an asynchronous event sequence in the continuous time domain, and use the conditional intensity function and survival function in the loss function to calculate the confidence of knowledge at time $t$. Since time is a parameter of the density function, this type of method belongs to the interpolation inference method ~\cite{dai2016deep} and can predict the probability of knowledge occurrence at any time with flexibility in the prediction format. However, this type of method has the cold-start problem~\cite{liu2020towards}, and cannot learn high-quality representations for entities with sparse knowledge, leading to poor inference performance.

\subsubsection{Sequence Neural Network-based Prediction Methods}
Due to the powerful learning and fitting ability of neural networks, in recent years, inference methods based on neural networks have been proven to effectively learn semantic and structural features of knowledge graphs for reasoning. Inference methods based on sequence neural networks view temporal knowledge graphs as discrete dynamic graphs, and use neural networks to extract features of snapshot sequences in the discrete dynamic graphs to learn the evolution information.
From the perspective of model architecture, sequence neural networks consist of snapshot encoders and temporal encoders: snapshot encoders extract representations of the temporal knowledge graph at different times from the snapshot sequence; temporal encoders integrate the snapshot representations to learn the entity evolution information from them.

These methods assume that the constantly changing entity representations reflect the evolution pattern of the temporal knowledge graph, and attempt to explore this evolution pattern from the representations of entities at different times. Based on the types of temporal encoders, these methods can be divided into concatenation-based temporal encoding methods, RNN-based temporal encoding methods, CNN-based temporal encoding methods, and self-attention-based temporal encoding methods.

Dyngraph2vec~\cite{goyal2020dyngraph2vec} proposed uses the autoencoder to extract knowledge graph snapshot features, and simply concatenates the entity representations at time $t$ and before as historical information. The latter two combinations both use RNN as the temporal encoder. Compared to the simple concatenation of the sequence, RNN can better capture the temporal dependencies between snapshots and achieve better performance in relationship inference tasks. 

RE\_NET~\cite{jin2019recurrent} aggregates the representations of neighbors in historical time steps, concatenates them with the vector representations of the head entity $s$ and relationship $r$, encodes the evolving information through RNN to obtain the latest representation of the tail entity, which is used to predict the possible tail entity that may establish a relationship with it in the next time step.

To better extract the topological features of knowledge graphs at each stage, RE-GCN~\cite{RE-GCN} uses a relation-aware graph convolutional network (RGCN) to encode snapshot features in the knowledge graph and then learns the evolution patterns of features through a recurrent neural network. CEN~\cite{CEN} builds on RE-GCN by considering the length diversity and temporal variability of temporal patterns. It encodes multiple lengths using a relation-aware graph convolutional network to model the length diversity and trains the model online to address temporal variability. HiSMatch~\cite{HiSMatch} uses relation-aware graph neural networks and recurrent neural networks to distinguish between graph sequences relevant to queries and those relevant to candidate entities, and proposes a matching framework for temporal reasoning. Similarly, methods~\cite{taheri2019learning, manessi2020dynamic, gao2022modeling} all adopt the combination of graph neural networks and recurrent neural networks. However, recurrent neural networks suffer from the problem of information forgetting when encoding long-distance temporal information, and perform poorly in multi-step prediction tasks~\cite{DGNN5}.

Convolutional neural networks (CNNs) have the excellent capability for extracting local features, and their weight-sharing and sampling properties can effectively reduce the number of model parameters, making them widely used in time-series data modeling. STGCN~\cite{STGCN} uses Graph CNN and Temporal CNN modules to respectively extract and fuse spatial and temporal features in traffic networks for predicting dynamic changes in traffic network flow. Compared to traditional sequence prediction models such as ARIMA, STGCN increased the MAPE indicator by 5.5\% while reducing the number of parameters.
DynGraphGAN~\cite{xiong2019dyngraphgan}, TNDCN~\cite{wang2020generic}, and other works also use CNNs to encode the temporal sequence features in the evolution process of knowledge graphs. However, the local feature perception property of CNNs leads to limited effectiveness in encoding long-distance time series.

%TBD Temp, DySAT

In summary, due to the powerful learning ability of neural networks, inference methods based on sequence neural network models can effectively learn the dynamic evolution patterns of entities. However, such methods strongly rely on training data, and the model performance is poor when the training data is insufficient. In addition, the lack of interpretability in inference due to the black-box nature of neural networks is also a problem for this type of method.




==> sections/bak/sec5_LM_KG.tex <==
\section{Comparison between KGs and LLMs}\label{sec:5}
Knowledge Graphs and Large Language Models represent contrasting paradigms in knowledge representation. KGs are the most representative symbolic knowledge form, which provides interpretability through structured information, yet may lack flexibility. LLMs are the most powerful parameter knowledge form, which excels in generativity and adaptability, handling diverse tasks, but can be opaque in decision-making.

This section is dedicated to a comprehensive comparison between KGs and LLMs, aiming to gain a deeper understanding of their similarities and differences, guiding the future integration and application of both.

% \subsection{Comparison between KG and LLM}\label{sec:5.1}
\subsection{Similarities}\label{sec:5.1}
The main similarities between KGs and LLMs are three-fold: 1. both of their data sources come from massive amounts of unstructured data; 2. both of them can represent entity semantics, and store relational knowledge between entities; 3. both of them can be used as knowledge sources for downstream applications, e.g., question answering.

The training of LLMs requires large amounts of textual data, which are often obtained from publicly available Internet websites. The construction of large-scale KGs also relies on information extraction from unstructured open data. Some LLMs and large-scale KGs even use the same data sources. For example, Wikipedia is the most important training corpus for a lot of LLMs like BERT, and also the main data source for general KGs, e.g., DBpedia, and YAGO.

KGs express the semantic information of entities by recording their types, attributes, and descriptions, as well as relations between them. On the other hand, LLMs are trained on text data to obtain character-level embeddings or word-level embeddings of entities, which can also represent the semantics of entities. LLMs~\cite{KGLM2} have also been shown to be able to recall relational knowledge without fine-tuning. Specifically, to answer a query (\textit{Joe Biden}, \textit{place\_of\_birth}, \textit{?}) using an LLM, one can input a masking sentence \textit{"Joe Biden was born in [MASK]"} or a natural language generation (NLG) task \textit{"Where was Joe Biden born? [MASK]"} to probe relational knowledge, where \textit{MASK} is a placeholder for the object entity to be predicted and \textit{"was born in"} is the prompt string of relation \textit{"place\_of\_birth"}. Previous studies have shown that such paradigms can perform well on some knowledge probing benchmarks like LAMA~\cite{KGLM1}. Moreover, some follow-up works propose various automatic prompt generation methods to further improve probing performances of LLMs~\cite{knowprob1,knowprob2,knowprob3,knowprob4,knowprob5}.

Large-scale KGs are often the main knowledge sources of some downstream applications, e.g., a knowledge base question answering (KBQA) system. The rise of LLMs makes it possible to perform such downstream tasks without access to external knowledge, e.g., closed-book QA. For instance, BERT has been proven to do remarkably well on open-domain QA~\cite{KGLM1}. Some literature shows that such LLMs can further improve their performances on open-domain QA after fine-tuning~\cite{LMQA}. 

\subsection{Differences}\label{sec:5.2}
To demonstrate the differences between LLMs and KGs, we discuss the limitations of KGs concerning LLMs and the current limitations of LLMs relative to the capabilities of KGs, separately. We conclude the limitations of KGs as follows,
\begin{itemize}
    \item \textbf{High construction cost:} The construction of knowledge graphs requires complex NLP techniques to process the text and quality testing to ensure the accuracy of the knowledge. Thus, the construction and maintenance of a large-scale KG often need significant human effort.
    \item \textbf{Data Sparsity:} Due to the high labor cost, the domain and data volume covered by a KG are limited, which leads to a large amount of missing data in the KG.
    \item \textbf{Lack of flexibility:} The storage structure and query method of a KG are relatively fixed, and it is difficult to adapt to various data structures and query requirements. By contrast, LLMs can offer better extendability and expressibility to different kinds of downstream tasks and thus have a broader range of application scenarios.
\end{itemize}

Although LLMs demonstrate superior reasoning capabilities and versatility over KGs, there are still some obvious limitations of LLMs that can be addressed by combining them with different types of KGs,
\begin{itemize}
    \item \textbf{LLM vs SKG:} LLMs are black-box models in nature. It is difficult to know the basis of the answers given by an LLM and the corresponding reasoning process. Meanwhile, one of the main advantages of KGs is their \textbf{explainability}. It would be easier to know how the answers are inferred over a KG. Moreover, regardless of knowledge updating and revision, an SKG will give a consistent answer to a query no matter how many times this query is performed. By contrast, LLMs might show different answers to the same question due to their \textbf{randomness} and the nature of probabilistic models. And the training corpus used for LLM might be noisy. The training processes of LLMs have the risk of learning incorrect or toxic knowledge~\cite{LMdanger}, while the \textbf{reliability of knowledge} is ensured by quality assessment for a KG, especially for small-scale domain-specific KGs.
    \item \textbf{LLM vs DKG:} LLMs might suffer from \textbf{outdated knowledge and information} since they are pre-trained based on Internet data at a specific time. And LLMs have \textbf{limited editability}, that is to say, it is difficult for LLMs to frequently learn new knowledge and information due to their \textbf{unaffordable training cost}. For example, the largest GPT3 model~\cite{gpt3} has a parametric count of 175B and costs 10 million dollars for a single training session. By contrast, it is much easier for DKGs to revise and update the knowledge they have stored. Thus, the cost of knowledge updating will be significantly reduced for LLMs if LLMs and DKGs can be effectively combined without expensive training processes.
    \item \textbf{LLM vs TKG:} LLMs face three main challenges when dealing with temporal information~\cite{TKGLM}. The first challenge is \textbf{averaging}, i.e., the model may see conflicting information about time ranges. The second challenge is \textbf{forgetting}, where the model may not remember facts that are valid only for a representative period of time, and therefore performs poorly when asked questions about the more distant past. The third challenge is \textbf{poor temporal calibration}, i.e., as LLMs become "stale", they are increasingly likely to be queried for facts that are outside the time range of their training data. Relatively, TKGs tend to have longer time scopes and the factual knowledge in TKGs is much more time-sensitive.
    \item \textbf{LLM vs EKG:} LLMs have achieved noticeable success on many NLP tasks, but they still struggle for event-centric tasks. One of the main disadvantages of LLMs on learning event-centric knowledge is that they may not be able to capture the temporal relations between events effectively. This is because LLMs are trained on large text corpora via self-supervised learning methods and may not have access to structured data that can help them learn about \textbf{event temporal relations}~\cite{econet}. Moreover, event-centric knowledge is updated very quickly, and it is difficult for LLMs to learn from the constant addition of new event-centric knowledge.
\end{itemize}   

In addition to their respective limitations, KGs and LLMs have different representation forms to store knowledge, and different ways of performing knowledge reasoning. And although LLMs obtain decent knowledge probing performances on LAMA, some follow-up works propose more difficult and domain-specific probing datasets~\cite{BioLAMA,MedLAMA} for LLMs and demonstrate that current LLMs are not reliable in factual knowledge extraction~\cite{KGLM3, EBERT}, which is contrary to the perspective that LLMs can be seen as knowledge bases. Therefore, we believe that it is very necessary to address the existing limitations of LLMs to combine LLMs with different types of KGs.

% \begin{figure*}[t]
% \centering
% \includegraphics[width=15cm]{img/kg4llm.pdf} 
% \caption{Illustration of three categories of KG-augmented LLMs.}
% \label{fig:kg4llm}
% \end{figure*}


% \begin{table*}[t]
% \begin{center}
% \caption{Existing combinations of LLMs and KGs, related learning tasks, and specific task description, as well as representative methods.}\label{table:LLM&KG}
% \begin{tabular}{l|p{4.5cm}|p{5.45cm}|p{1.3cm}|p{3.1cm}}
% \toprule
%  Combinations & Tasks & Descriptions & KG Type& Representative Methods\cr 
% \midrule
%  \multirow{12}{*}{LLM for KG}& Knowledge Extraction & Input text to LLMs and recognize entities, relations and events within text& All Types & \cite{bert_NER,ANL_NER}\cr
%  \cmidrule{2-5}
%  & Knowledge Reasoning &Perform reasoning by inputting textual sequences generated from triples or triple paths to LLMs&SKG\&DKG & KBERT\cite{KBERT}, StAR\cite{StAR},  BERTRL\cite{BERTRL}, KG-BERT\cite{KG-BERT}, Bi-Link\cite{Bi-Link}\cr
%   \cmidrule{2-5}
%   & Entity Typing &Classify entity mentions extracted from text using LLM-base sequence labeling models &All Types & LME~\cite{entitytype1}, $\quad\quad\quad\quad\quad$ MLMET~\cite{entitytype2}\cr
%  \cmidrule{2-5}
%  & Entity Linking &Link the entity mentions extracted from text to the entities on KGs using LLM-based sequence labeling models&All Types & GENRE\cite{entitylink1}, $\quad\quad\quad\quad$ EPGEL~\cite{entitylink2}\cr
%  \cmidrule{2-5}
%   & Entity Alignment &Find entity pairs with similar literal information using LLMs &All Types & BERT-INT~\cite{BERTINT}\cr
%    \cmidrule{2-5}
% & Quality Assessment &Use LLMs to determine the correctness of  textual sequences generated from triples&All Types & KGRepair\cite{arnaout2022utilizing}\cr
%  \midrule
%  \multirow{6}{*}{KG for LLM}& Knowledge-Enhanced LLM &Enrich input text of LLMs with background knowledge from KGs &SKG &KALM\cite{KALM}, LUKE\cite{LUKE}, EBERT\cite{EBERT}\cr
%  \cmidrule{2-5}
% & Knowledge-Encoded LLM &Adapt the architecture of LLMs to encode structured knowledge from KGs &SKG &ERNIE\cite{ERINE}, Knowbert\cite{Knowbert}, K-Adapter\cite{K-Adapter}\cr
%  \cmidrule{2-5}
%  & Knowledge Task-based LLM &Use knowledge-constrained pretraining tasks to optimize LLMs &SKG &ERNIE3\cite{Ernie3}, KEPLER\cite{KEPLER}, K-PLUG\cite{-k-plug}\cr
%  % \cmidrule{2-5}
%  % & TKG/EKG-augmented LLM & Force LLMs to learn temporal knowledge and event-centric knowledge from TKGs and EKGs &TKG\&EKG &To be explored\cr
%  % \cmidrule{2-5}
%  %  & KG-augmented Prompt Learning &Retrieve factual knowledge related to the input text of LLMs from KGs and generate textual knowledge prompts &All Types &To be explored\cr
%  % \cmidrule{2-5}
%  %  & KG-based Hallucination Measuring & Measure the hallucination of LLM-generated texts based on relevant factual knowledge from KGs &All Types &To be explored\cr
%  \bottomrule
% \end{tabular}
% \end{center}
% \end{table*}

% \subsection{Existing Combinations of KG and LLM}
% \subsubsection{LLM for KG}
% In the early stage, the construction of KGs mainly relied on manual work and used to be very costly. With the development of AI technology, the automated KG construction technology based on deep learning has been widely used. However, most KGs still suffer from data sparsity, and their data quality needs to be improved. LLMs recently have shown to be an effective tool to extract, fuse and process structured knowledge due to their powerful capabilities of text processing and semantic expression.

% In the previous sections, we have discussed in detail the application of LLMs to various tasks of knowledge extraction and reasoning, including NER, relation extraction, event extraction, SKGR, and DKGR. As for knowledge extraction, LLMs can assist in extracting entities, relations and events from text by learning semantic representations of words and contextual associations between them. On the other hand, the rich semantic information of entities and the contextual relationships between entities contained in LLMs can be used to enhance the performance of the KGR model as a complement to the structured information of KGs.

% In addition to knowledge extraction and knowledge reasoning, LLMs are also used in other important parts of the KG construction process, such as entity typing, entity linking, entity alignment and quality assessment. For example,  LME~\cite{entitytype1} and MLMET~\cite{entitytype2} have shown that LLMs can be used to perform the task of entity typing by leveraging literal information of context sentences and type labels. GENRE~\cite{entitylink1} and EPGEL~\cite{entitylink2} use BART-based sequence-to-sequence models to link the entity mentions extracted from text to the entities on KGs. BERT-INT~\cite{BERTINT} is a neural entity alignment method, which leverage the literal information of entities, especially entity names, entity descriptions and attributes, with a BERT-based interaction model to match equivalent entities across different KGs. Other works~\cite{arnaout2022utilizing} have looked into how to use LLMs to detect incorrect triples and replace them with likely correct ones for the assessment and improvement of the quality of the KG. In summary, a lot of studies have been done on using LLMs to support KG curation. While LLMs have stronger multi-tasking capability and greater versatility, fully automated knowledge extraction, knowledge fusion, knowledge update and knowledge inference for KGs using LLMs will greatly reduce the cost of KG construction.


% \subsubsection{KG for LLM}
% Although LLMs can learn generic knowledge from massive texts, they still have disadvantages such as unreliablity of knowledge, and lack of interpretability. The introduction of structured knowledge from KGs can effectively alleviate these deficiencies. Motivated by this, KG-augmented LLMs have been born. Fusing LLMs and KGs allows KG-augmented LLMs to combine generic semantic knowledge, common sense knowledge, factual knowledge, and domain knowledge, which enable effective response to downstream knowledge-driven tasks. 

% As neural networks, LLMs consist of three kinds of network layers: the input layer, the hidden layer and the output layer. Based on this structure, the existing KG-augmented LLMs can be classified into three main categories: knowledge-enhanced LLMs, knowledge-encoded LLMs, and knowledge task-based LLMs, as shown in Figure~\ref{fig:kg4llm}. Different types of KG-augmented LLMs embed knowledge into different network layers.

% \textbf{Knowledge-Enhanced LLMs:} Knowledge-enhanced LLMs aims to enrich contextual information with background knowledge from KGs as supplementary input to help the model better understand the text. Such LLMs can be further divided into two sub-categories. The first category directly converts structured knowledge into text form to construct new training corpus~\cite{ye2019align} or concatenate it into existing text~\cite{KBERT,colake}. Another class of knowledge-enhanced LLMs represent entities and relationships in a KG as vectors and combines them with the text embeddings corresponding to the input text. Specific combinations include concatenating or adding entity embeddings with text embeddings~\cite{EBERT,LUKE,KALM}, concatenating entity type embeddings~\cite{KALM2}, special marker embeddings or positional embeddings with text embeddings~\cite{OAG-BERT}, etc.

% \textbf{Knowledge-Encoded LLMs:} Knowledge-encoded LLMs adapt the architecture of the transformer layers of the LLMs so that they have the ability to encode and integrate effective features of both text corpus and structured knowledge. There are three ways to encode structured knowledge into the transformer layers of LLMs, i.e., adding external knowledge encoding modules, modifying original encoding modules, and using standalone neural adapters. By connecting the output of the transformer layers to an external knowledge encoding module, some knowledge-encoded LLMs can encode both text and structured knowledge, and output a feature representation that incorporates valid information from both~\cite{ERINE,CokeBERT,BERT-MK,Ernie3}. There is also a part of LLMs that directly modify the internal structure of the Transformer layers so that they have the ability to handle structured knowledge. Specific modifications include inserting additional knowledge encoding module at specific locations in the middle layers~\cite{Knowbert}, and adapting the Transformer's original encoding mechanism to structured knowledge~\cite{KBERT,colake}. Other knowledge-encoded LLMs use neural adapters that store specific knowledge to encode knowledge from different resources. These adapters are plug-and-play and can operate independently from the LLMs~\cite{K-Adapter,lauscher-etal-2020-common}.

% \textbf{Knowledge Task-based LLMs:} A large amount of recent works have attempted to use knowledge-constrained pre-training tasks and push LLMs to learn more knowledge by completing these tasks during the pre-training process. There are two main types of such knowledge-constrained tasks, namely, knowledge masking tasks and knowledge representation tasks. The knowledge masking task uses various types of knowledge to develop a masking strategy and select masking targets, thus forcing LLMs to have specific knowledge in order to accurately predict what is to be masked~\cite{ERINE,-k-plug,CorefBert,Ernie3}.  The knowledge representation task attempts to combine the learning process of knowledge representation with the training process of LLMs. By establishing a connection between text and structured knowledge and setting up a joint multi-task training mechanism for both knowledge representation learning and language representation learning, it is possible to train the model parameters while learning the knowledge representation~\cite{KEPLER,jaket,eae,fae,mtb,erica,KG-BERT}.

% A KG-augmented LLM can use more than one ways to integrate structured knowledge into the LLM. For example, ERNIE3.0~\cite{Ernie3} adds a knowledge encoding module on top of the original encoding layers, and proposes a pre-training framework in which the language representation module and the knowledge task module run collaboratively, and thus can be considered as both a knowledge-encoded LLM and a knowledge task-based LLM.

% KG-augmented LLMs are equipped with enhanced semantic understanding by learning knowledge from SKGs. 
% However, the way they learn knowledge is still to update the large-scale neural networks, which is very costly and unexplainable. Since most of KG-augmented LLMs need to be retrained to update the knowledge they have learned when real-world knowledge changes, they still suffer from the issues of unreliable knowledge, limited editability and low explainability. Moreover, both LLMs and SKGs have limitations in understanding time information and event information. It is necessary to go into new approaches with can more effectively combine different types of KGs with LLMs.











==> sections/bak/sec5_applications.tex <==
% 应用：
% 1. 作为领域知识的载体，支持丰富的领域应用（金融投资、交通、安全、军事、医疗），满足高可信、强实时的应用需求
% 2. 作为个性化信息的载体，支持个性化的应用需求，例如个性化推荐、智能助手
% 3. 结构化的知识建模方式，能够服务于药物发现、社交挖掘、金融风险分析等依赖于结构信息分析的应用

% 改为case的形式
% 1. 介绍信息抽取在金融领域的应用，从金融文档（例如财报、财经新闻、研报）中抽取企业相关知识，构建或更新金融知识图谱。这里知识抽取的对象包括金融实体、较为稳定的概念、具有时效性、动态演化的知识、以及金融事件等等，通过知识抽取后，能够将巨量的金融数据转化为高质量的金融知识，并且以知识图谱为载体呈现；
% 2. 介绍在构建好的金融知识图谱基础上，可以结合图数据挖掘等算法进行金融知识推理，并在具体的金融应用中落地，例如基于事件知识的量化投资（如图所示）。
% 3. 金融知识图谱还能够结合大预言模型进行智能问答，通过动态更新的金融知识图谱的引入，提升大语言模型的金融领域实时知识以及解决金融领域任务的能力，并且对于回答进行事实一致性检测，提升大语言模型生成内容的事实性，并能够结合大语言模型，提升用户的交互体验。



\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{img/EKGR_Example.pdf}
    \caption{In an application of EKGR in event-driven quantitative investment, a piece of news concerning "Pharmaceutical A" (Phar. A) triggers the extraction and mapping of the event triple ("negative report", "relates to", "Phar. A") onto the EKG. Subsequently, link prediction is used to assess potential outcomes, such as the link ("Price drop", "relates to", "Phar. A"). Risk links, denoted as ("Phar. A", "Potential risk", $\ast$), are predicted for neighboring entities within the EKG, including upstream and downstream partners in the supply chain. Multi-hop reasoning is applied to analyze risk propagation among stocks within the same industry. These reasoning results are then utilized in risk analysis and investment decisions. For instance, negative effects propagating through Phar. A's supply chain may suggest short positions ("Med. C" and "Biotech D"), while long positions could be considered for companies offering alternative products ("Phar. B"). This illustration's depicted news contents, company names, and numerical values are purely fictional and solely serve illustrative purposes.}
    \label{fig:ekgr_example}
\end{figure*}

\section{Applications}~\label{sec:5}
Knowledge graphs have become integral parts of several areas of technology, from structured data management to artificial intelligence. They encapsulate structured information in a way that both humans and machines can comprehend, enabling a multitude of practical applications. Their seamless integration with LLMs has expanded these applications even further, making them indispensable in the landscape of data and AI. 

This section will first take the financial as a case to illustrate the applications of KG, and highlight the main application domains of KGs.

\subsection{Application in Finance}
The application of knowledge graphs in the finance sector serves as an exemplary illustration of how structured knowledge representation can transform data-driven industries. Specifically, knowledge extraction, knowledge reasoning, and intelligent QA systems that combine KGs with LLMs play a vital role in this domain.

\subsubsection{Financial Information Extraction and Knowledge Graph Construction}
The first essential step involves extracting information from financial documents, such as financial reports, economic news, and research papers, to construct or update a financial knowledge graph. In this context, information extraction targets various elements, including financial entities (e.g., stocks, bonds, corporations), relatively stable concepts (e.g., market indices, financial instruments), dynamically evolving knowledge (e.g., stock prices, economic indicators), temporal information (e.g., trade dates), and financial events (e.g., mergers, acquisitions, dividends announcements).

The extracted knowledge is then organized into a KG. This process transforms massive amounts of unstructured financial data into high-quality, structured financial knowledge, which is then effectively represented and made easily accessible through the KG.

\subsubsection{Financial Knowledge Reasoning}
Upon constructing the financial knowledge graph, graph-based data mining algorithms can be applied to infer new knowledge. For instance, the graph can be analyzed to detect patterns and trends based on historical financial events. One practical application of this is event-driven quantitative investment, where investment strategies are formulated based on the relationships and patterns identified within the KGs.

% Mapping application scenarios to EKGR-specific problems
Figure~\ref{fig:ekgr_example} showcases an instance of EKGR application within the context of event-driven quantitative investment. This example demonstrates how investment decisions can be based on streaming events associated with entities in the financial market. Real-time news and reports serve as the data source, feeding relevant events into the investment system. Information in these events is then extracted and mapped to triples on the event knowledge graph. Subsequently, link prediction techniques are employed to analyze the potential impact of these events. By examining the links between events and associated stocks, the system can predict outcomes and assess risks. Additionally, multi-hop reasoning enables the analysis of risk propagation, particularly among stocks within the same industry. The results of this reasoning process are valuable for downstream applications, including risk analysis, stock trend prediction, and informing investment decisions such as determining long or short positions on specific stocks.

\subsubsection{Integration with LLMs for Financial QA}
Financial knowledge graphs can also be integrated with large language models to enable intelligent QA systems tailored for the finance sector. Through dynamically updated financial knowledge graphs, LLMs can be kept current with real-time financial knowledge. This integration not only enhances the ability of LLMs to perform tasks in the financial domain but also allows for fact-consistency checks, ensuring the factual accuracy of the content generated by LLMs.

Furthermore, the interaction with LLMs becomes more engaging and informative for users. For instance, a user can query the intelligent QA system regarding investment strategies based on recent financial events, and the system can provide insightful responses grounded in the data represented within the knowledge graph.

In conclusion, the finance sector benefits immensely from knowledge graphs by streamlining information extraction, enabling sophisticated knowledge reasoning, and enhancing user interaction through the integration of large language models. This amalgamation of technologies paves the way for more informed decision-making and a deeper understanding of complex financial ecosystems.

\subsection{Other Applications}
Knowledge graphs have widespread applications beyond finance, notably in healthcare, transportation, retail, manufacturing, legal, and personalized services.

\textbf{Healthcare}.
Knowledge graphs amalgamate patient records, medical literature, and drug information, paving the way for enhanced diagnosis, smart treatments, and drug discovery by elucidating relationships between diseases, symptoms, medications, and patient histories.

\textbf{Transportation}.
In transportation, knowledge graphs structure data encompassing routes, traffic conditions, and vehicle statuses, empowering intelligent systems to optimize route planning, manage traffic efficiently, and predict maintenance needs.

\textbf{Manufacturing}.
Within manufacturing, knowledge graphs assimilate data on product components, manufacturing processes, and supply chains, supporting predictive maintenance, quality control, and optimized production planning by analyzing relationships between machine performances, material availability, and production schedules.

\textbf{Legal}.
In the legal domain, knowledge graphs consolidate statutes, case law, and legal doctrines, aiding in legal research, case preparation, and regulatory compliance by structuring and analyzing the relationships between different legal entities and concepts.

\textbf{Personalized Services}.
Through social knowledge graphs modeling users' cognition and preferences, personalized services have burgeoned across sectors like education, psychotherapy, and personalized recommendations. These graphs facilitate a tailored user experience by aligning services and content with individual user preferences and behaviors, thereby enhancing engagement and satisfaction.

In summation, KGs significantly contribute to data organization and analysis across disparate sectors. The interplay between KGs and advanced technologies like LLMs further amplifies their application spectrum, propelling innovation and efficiency.

% % Potential methods: extending TKGR to EKGR, some algorithmic challenges
% Despite the promising value of EKGR in practical applications, several challenges need to be addressed to enable its effective implementation in the real world. Firstly, the development of a robust EKG embedding model is crucial as it forms the foundational platform for accurate EKG reasoning. Secondly, suitable data structures and storage techniques must be employed to handle the continuously growing influx of event information. Adequate accommodations are needed to ensure efficient storage and retrieval of large volumes of event data. Lastly, the real-time nature of many applications necessitates the resolution of algorithmic and engineering challenges to improve the execution speed of EKGR algorithms.

% In summary, knowledge graphs are a versatile tool with a broad array of applications across multiple domains. Their ability to represent and analyze complex, structured information makes them a vital asset in the ever-increasing data-driven landscape.


% \subsection{Knowledge Retrieval for LLMs} %领域
% For both KG-augmented prompt learning and KG-based hallucination measuring, one of the most important parts is to retrieve relevant knowledge from KGs based on the input or output text of the LLM. Taking knowledge base question answering as an example, a lot of state-of-the-art approaches are based on information retrieval, which first sample subgraphs based on relevant entities and relations in questions, and then perform reasoning in the subgraph and find the answer to the question. However, since the input length of LLM is limited, it must be ensured that the sampled subgraphs or the retrieved knowledge must be translatable into text within a specified number of words. Thus, efficient knowledge retrieval and prompting methods are needed. This challenge has not been solved by the existing methods, and is worth exploring in-depth in the future.


% \subsection{Domain-specific KG Applications} %领域
% In knowledge-intensive domains such as finance, medicine and law, general LLMs are prone to give incorrect output results during use due to their issues of hallucination and limited domain knowledge, thus misleading users to make wrong judgments. On the other hand, the knowledge in these domains is updated rapidly. To avoid outdated knowledge, high-frequent fine-tuning for domain-specific LLMs inevitably leads to high consumption during training. Therefore, combining domain-specific DKGs with LLMs will be a promising future research trend. At the same time, temporal and event information are extremely valuable knowledge in these domains. Learning and applying such knowledge can be significantly helpful for reasoning processes in downstream tasks. For example, learning the causal relationships between financial events will help risk control in the financial domain. Learning the change of relations between financial entities can help users to make better investment decisions. We deem that the application of domain-specific KGs or domain-specific kG-augmented LLMs in relevant downstream tasks should receive more attention.


==> sections/bak/sec6_future.tex <==
\section{The Future Directions of Knowledge Engineering}~\label{sec:6}
Existing researches on knowledge extraction, reasoning, and augmentation with LLMs for knowledge graphs have made significant progress in various aspects. However, as the forms of KGs have evolving, the corresponding techniques still face various challenges and open problems in the future. In this section, we try to point out promising research directions for future work.

\subsection{On the Evolution of Knowledge Representation}
%补充知识工程的下一个形态
The evolution of KGs illuminates the gradual understanding and also the limitations of this knowledge representation paradigm. Current challenges faced by KGs include: (1) the inability to directly and accurately model higher-order logic knowledge and apply it in higher-order knowledge reasoning; (2) ineffective handling and direct computation of numerical knowledge through KGs; (3) from a knowledge management perspective, the demand for a representation that supports continuous business iteration while effectively avoiding combinatorial explosion and redundant construction, challenges the existing KGs in unifying different granularities and types of knowledge and modeling their interactions, with RDF/OWL-based knowledge modeling being overly complex and prone to redundancy in rapidly evolving scenarios; and (4) unlike LLMs that store and reason knowledge through parameterization, the segregation of knowledge storage and reasoning in existing KGs lacks a unified framework integrating large-scale knowledge storage with efficient knowledge reasoning, hindering the maximization of knowledge utilization.

To address these challenges, exploring innovative knowledge representation paradigms is crucial. The notion of knowledge programmability, representing knowledge through programming languages, emerges as a potential avenue warranting further exploration. This proposition aligns with the broader goal of enhancing the granularity and expressiveness of knowledge representation, fostering a more nuanced understanding and management of the evolving knowledge landscape. By leveraging the latest advancements in knowledge representation technology, especially within the context of artificial intelligence and machine learning, both the academic and industrial sectors are poised to unveil new dimensions of knowledge representation transcending the traditional boundaries of KGs, paving the way for more dynamic, scalable, and comprehensive knowledge engineering systems.

\subsection{On the Evolution of Knowledge Extraction}
The construction of KGs relies on various knowledge extraction techniques. Most of the existing knowledge extraction methods are supervised models needing a large amount of labeled data. In order to effectively reduce the construction cost of KGs, it is necessary to go into zero-shot/unsupervised knowledge extraction methods and knowledge graph maintenance.

\subsubsection{From Supervised to Zero-shot/ Unsupervised Knowledge Extraction}
Most supervised knowledge extraction methods are based on contextualized LLMs fine-tuned by labeled data and corresponding tasks. However, these labeled data often need to be annotated by humans, especially for some knowledge-intensive texts, the annotation process requires certain domain knowledge and could be very costly. Meanwhile, generative LLM models have been viewed as a kind of strong zero-shot learners that can be applied to various types of downstream tasks in scenarios where labeled data is lacking. Nevertheless, the existing generative LLMs still significantly underperform fully-supervised baseline models on knowledge extraction tasks. This is because most of the knowledge extraction tasks are labeling tasks, while generative LLMs are good at generation tasks. To achieve zero-shot or unsupervised knowledge extraction for low-cost knowledge graph construction, it is essential future direction to fill this gap by efficiently transforming different types of knowledge extraction tasks into generation tasks and solving them using generative LLMs.

\subsubsection{Potential Direction of Knowledge Quality Control and Maintenance}
Quality control and maintenance are crucial in knowledge engineering, affecting KG usability in real-world applications because it is hard to ensure the completeness and correctness of extracted knowledge. The advent of LLMs provides new perspectives on addressing these challenges, which leverages parameterized knowledge of LLMs learned from vast corpora for KGs' quality control and maintenance through an unsupervised way.

\subsection{On the Evolution of Knowledge Reasoning}
The existing knowledge reasoning techniques mainly focus on SKGs. With the formal evolution of KGs, knowledge reasoning techniques for DKGs and TKGs have received more attention, but still remain to be improved. It is also worth noting that reasoning over EKGs is largely unexplored. Besides, neural-symbolic knowledge reasoning is also remain to be exploring.

\subsubsection{Non-static Knowledge Graph Reasoning}
Recent advances have prompted a shift from SKGs to more dynamic structures like DKGs and TKGs, aiming to accurately represent and reason over the dynamic nature of real-world knowledge. However, reasoning techniques for DKGs and TKGs are still nascent, with temporal knowledge completion and extrapolation emerging as notable endeavors. The development of techniques to navigate the temporal and dynamic dimensions of knowledge is crucial, presenting a fertile ground for future research.

A significant avenue for future research is to unravel the evolution logic behind temporal knowledge, promising to enrich the reasoning frameworks for these non-static KGs. This includes developing advanced algorithms for tracking and modeling temporal evolution of facts and relationships, and exploring how different types of temporal knowledge, such as dynamic relations and interactions, interconnect and influence each other.

\subsubsection{Event Knowledge Graph Reasoning} %领域
In recent years, research on knowledge reasoning in SKGs, DKGs, and TKGs has attracted widespread interest. With the rise of EKGs, EKG reasoning (EKGR) will inevitably become a new research hotspot. EKGR could probably predict potential future events based on the existing relations between entities and events, which is very important for many practical application scenarios. However, how to develop an EKG embedding model to model events, a new kind of knowledge element, has never been discussed in previous research. It will also be interesting to explore the utility of event logic and LLMs for the task of EKGR since EKGs contain a lot of logical relationships and textual descriptions between events.

Despite the promising value of EKGR in practical applications, several challenges need to be addressed to enable its effective implementation in the real world. Firstly, the development of a robust EKG embedding model is crucial as it forms the foundational platform for accurate EKG reasoning. Secondly, suitable data structures and storage techniques must be employed to handle the continuously growing influx of event information. Adequate accommodations are needed to ensure efficient storage and retrieval of large volumes of event data. Lastly, the real-time nature of many applications necessitates the resolution of algorithmic and engineering challenges to improve the execution speed of EKGR algorithms.

\subsubsection{From Neural or Symbolic to Neural-Symbolic Knowledge Reasoning}
Recent advancements in neural or symbolic reasoning have highlighted the potential of integrating neural networks' data-driven learning with symbolic reasoning's structured logic, to enhance reasoning on various KGs. This fusion aims to overcome limitations posed by exclusively neural or symbolic approaches, particularly in representing the dynamic and time-variant nature of real-world knowledge in DKGs and TKGs.

Besides factual knowledge, a considerable amount of logical knowledge is implied in KGs, encompassing a vast number of first-order or temporal logical rules between relations and events. The application of these logical rules, when combined with various KG embedding models, can significantly improve the performance and interpretability of these models. Some existing works have demonstrated substantial improvements in static knowledge graph reasoning tasks by applying first-order logical rules. Yet, the application of static and temporal logical rules to KG reasoning tasks remains an open avenue for exploration. Furthermore, the emergence of LLMs presents an opportunity to uncover underlying patterns in knowledge, aiding in reasoning tasks. The blend of neural-symbolic paradigms and the pattern recognition capabilities of LLMs could potentially pave the way for more effective and interpretable KG reasoning techniques, tailored to the evolving nature of knowledge in various types of KGs.

\subsection{Potential Combinations of KGs and LLMs}
Knowledge Graphs and Large Language Models represent contrasting paradigms in knowledge representation. KGs are the most representative symbolic knowledge form, which provides interpretability through structured information, yet may lack flexibility.
LLMs are the most powerful parameter knowledge form, which excels in generativity and adaptability, handling diverse tasks, but can be opaque in decision-making.
To gain a deeper understanding of the KG and LLM's similarities and differences, and guide the future integration and application of both, we propose a comprehensive comparison.

\subsubsection{Similarities}\label{sec:5.1}
The main similarities between KGs and LLMs are three-fold: 
(1) both of their data sources come from massive amounts of unstructured data; 
(2) both of them can represent entity semantics, and store correlations between entities; 
(3) both of them can be used as knowledge sources for downstream applications, e.g., question answering.

The training of LLMs requires large amounts of textual data, which are often obtained from publicly available Internet websites. The construction of large-scale KGs also relies on information extraction from unstructured open data. Some LLMs and large-scale KGs even use the same data sources. For example, Wikipedia is the most important training corpus for a lot of LLMs like BERT, and also the main data source for general KGs, e.g., DBpedia, and YAGO.

KGs express the semantic information of entities by recording their types, attributes, and descriptions, as well as relations between them. On the other hand, LLMs are trained on text data to obtain character-level embeddings or word-level embeddings of entities, which can also represent the semantics of entities. LLMs~\cite{KGLM2} have also been shown to be able to recall relational knowledge without fine-tuning. Specifically, to answer a query (\textit{Joe Biden}, \textit{place\_of\_birth}, \textit{?}) using an LLM, one can input a masking sentence \textit{"Joe Biden was born in [MASK]"} or a natural language generation (NLG) task \textit{"Where was Joe Biden born? [MASK]"} to probe relational knowledge, where \textit{MASK} is a placeholder for the object entity to be predicted and \textit{"was born in"} is the prompt string of relation \textit{"place\_of\_birth"}. Previous studies have shown that such paradigms can perform well on some knowledge probing benchmarks like LAMA~\cite{KGLM1}. Moreover, some follow-up works propose various automatic prompt generation methods to further improve probing performances of LLMs~\cite{knowprob1,knowprob2,knowprob3,knowprob4,knowprob5}.

Large-scale KGs are often the main knowledge sources of some downstream applications, e.g., a knowledge base question answering (KBQA) system. The rise of LLMs makes it possible to perform such downstream tasks without access to external knowledge, e.g., closed-book QA. For instance, BERT has been proven to do remarkably well on open-domain QA~\cite{KGLM1}. Some literature shows that such LLMs can further improve their performances on open-domain QA after fine-tuning~\cite{LMQA}. 

\subsubsection{Differences}\label{sec:5.2}
To illustrate the differences between LLMs and KGs, we discuss the limitations of KGs with respect to LLMs and the current limitations of LLMs relative to the capabilities of KGs, separately. We conclude the limitations of KGs as follows:

\textbf{(1) High construction cost:} The construction of knowledge graphs requires complex NLP techniques to process the text and quality testing to ensure the accuracy of the knowledge. Thus, the construction and maintenance of a large-scale KG often need significant human effort.

\textbf{(2) Data Sparsity:} Due to the high labor cost, the domain and data volume covered by a KG are limited, which leads to a large amount of missing data in the KG.

\textbf{(3) Lack of flexibility:} The storage structure and query method of a KG are relatively fixed, and it is difficult to adapt to various data structures and query requirements. By contrast, LLMs can offer better extendability and expressibility to different kinds of downstream tasks and thus have a broader range of application scenarios.

Although LLMs demonstrate superior reasoning capabilities and versatility over KGs, there are still some obvious limitations of LLMs that can be addressed by combining them with different types of KGs,

\textbf{LLM vs SKG:} LLMs are black-box models in nature. It is difficult to know the basis of the answers given by an LLM and the corresponding reasoning process. Meanwhile, one of the main advantages of KGs is their explainability. It would be easier to know how the answers are inferred over a KG. Moreover, regardless of knowledge updating and revision, an SKG will give a consistent answer to a query no matter how many times this query is performed. By contrast, LLMs might show different answers to the same question due to their randomness and nature of probabilistic models. And the training corpus used for LLM might be noisy. The training processes of LLMs have the risk of learning incorrect or toxic knowledge~\cite{LMdanger}, while the \textbf{reliability of knowledge} is ensured by quality assessment for a KG, especially for small-scale domain-specific KGs.

\textbf{LLM vs DKG:} LLMs might suffer from \textbf{outdated knowledge and information} since they are pre-trained based on Internet data at a specific time. And LLMs have \textbf{limited editability}, that is to say it is difficult for LLMs to frequently learn new knowledge and information due to their \textbf{unaffordable training cost}. For example, the largest GPT3 model~\cite{gpt3} has a parametric count of 175B and costs 10 million dollars for a single training session. By contrast, it is much easier for DKGs to revise and update the knowledge they have stored. Thus, the cost of knowledge updating will be significantly reduced for LLMs if LLMs and DKGs can be effectively combined without expensive training processes.

\textbf{LLM vs TKG:} LLMs face three main challenges when dealing with temporal information~\cite{TKGLM}. The first challenge is averaging, i.e., the model may see conflicting information about time ranges. The second challenge is forgetting, where the model may not remember facts that are valid only for a representative period of time, and therefore performs poorly when asked questions about the more distant past. The third challenge is poor temporal calibration, i.e., as LLMs become "stale", they are increasingly likely to be queried for facts that are outside the time range of their training data. Relatively, TKGs tend to have longer time scopes and the factual knowledge in TKGs is much more time-sensitive.

\textbf{LLM vs EKG:} LLMs have achieved noticeable success on many NLP tasks, but they still struggle with event-centric tasks. One of the main disadvantages of LLMs in learning event-centric knowledge is that they may not be able to capture the temporal relations between events effectively. This is because LLMs are trained on large text corpora via self-supervised learning methods and may not have access to structured data that can help them learn about event temporal relations~\cite{econet}. Moreover, event-centric knowledge is updated very quickly, and it is difficult for LLMs to learn from the constant addition of new event-centric knowledge.  

In addition to their respective limitations, KGs and LLMs have different representation forms to store knowledge and different ways of performing knowledge reasoning. And although LLMs obtain decent knowledge probing performances on LAMA, some follow-up works propose more difficult and domain-specific probing datasets~\cite{BioLAMA, MedLAMA} for LLMs and demonstrate that current LLMs are not reliable in factual knowledge extraction~\cite{KGLM3, EBERT}, which is contrary to the perspective that LLMs can be seen as knowledge bases. Therefore, it is necessary to address the existing limitations of LLMs to combine various KGs.

\subsubsection{The Combination of LLMs and Different KGs}\label{sec:5.2}
In summary, despite the distinct characteristics and functionalities of KGs and LLMs, there is significant potential for integration between the two, as illustrated in Figure~\ref{fig:KGLLM}.

Specifically, from the perspective of \textbf{LLM aided KG construction}: Utilizing the text processing capabilities of LLMs, KGs can achieve more efficient unsupervised knowledge extraction during their construction phase, thereby enhancing their automated building and editing capabilities. Additionally, LLMs can offer unsupervised quality control and maintenance for KGs, ensuring the quality and accuracy of knowledge. In terms of knowledge inference, the pattern induction capabilities of LLMs present new opportunities for neural-symbolic reasoning.

From the perspective of knowledge-driven LLM reasoning: KGs serve as a repository containing both logical and factual knowledge, providing a richer source of information. During the training phase, future research will increasingly explore how to integrate structured, high-quality knowledge with LLMs, such as using graph neural networks for knowledge encoding or adopting new encoding strategies. Such methods not only enrich the model's knowledge base but also optimize its structure and training objectives. In the inference phase, integrating KGs to detect and reduce knowledge illusions and enhance the reliability and accuracy of model outputs will be a pivotal research direction~\cite{sun2023think, wen2023mindmap}.

In conclusion, the integration of KGs and LLMs will bring innovation to the AI domain. By complementing each other, both entities have the potential to achieve superior performance and broader application scenarios.

\begin{figure}[t]
\centering
\includegraphics[width=0.85\linewidth]{img/fig_KGLLM.png} 
\caption{The potential integration framework of KGs and LLMs.}
\label{fig:KGLLM}
\end{figure}

==> sections/sec5_LM_KG.tex <==
\section{Comparison between KGs and LLMs}\label{sec:5}
Knowledge Graphs and Large Language Models represent contrasting paradigms in knowledge representation. KGs are the most representative symbolic knowledge form, which provides interpretability through structured information, yet may lack flexibility. LLMs are the most powerful parameter knowledge form, which excels in generativity and adaptability, handling diverse tasks, but can be opaque in decision-making.

This section is dedicated to a comprehensive comparison between KGs and LLMs, aiming to gain a deeper understanding of their similarities and differences, guiding the future integration and application of both.

% \subsection{Comparison between KG and LLM}\label{sec:5.1}
\subsection{Similarities}\label{sec:5.1}
The main similarities between KGs and LLMs are three-fold: 1. both of their data sources come from massive amounts of unstructured data; 2. both of them can represent entity semantics, and store relational knowledge between entities; 3. both of them can be used as knowledge sources for downstream applications, e.g., question answering.

The training of LLMs requires large amounts of textual data, which are often obtained from publicly available Internet websites. The construction of large-scale KGs also relies on information extraction from unstructured open data. Some LLMs and large-scale KGs even use the same data sources. For example, Wikipedia is the most important training corpus for a lot of LLMs like BERT, and also the main data source for general KGs, e.g., DBpedia, and YAGO.

KGs express the semantic information of entities by recording their types, attributes, and descriptions, as well as relations between them. On the other hand, LLMs are trained on text data to obtain character-level embeddings or word-level embeddings of entities, which can also represent the semantics of entities. LLMs~\cite{KGLM2} have also been shown to be able to recall relational knowledge without fine-tuning. Specifically, to answer a query (\textit{Joe Biden}, \textit{place\_of\_birth}, \textit{?}) using an LLM, one can input a masking sentence \textit{"Joe Biden was born in [MASK]"} or a natural language generation (NLG) task \textit{"Where was Joe Biden born? [MASK]"} to probe relational knowledge, where \textit{MASK} is a placeholder for the object entity to be predicted and \textit{"was born in"} is the prompt string of relation \textit{"place\_of\_birth"}. Previous studies have shown that such paradigms can perform well on some knowledge probing benchmarks like LAMA~\cite{KGLM1}. Moreover, some follow-up works propose various automatic prompt generation methods to further improve probing performances of LLMs~\cite{knowprob1,knowprob2,knowprob3,knowprob4,knowprob5}.

Large-scale KGs are often the main knowledge sources of some downstream applications, e.g., a knowledge base question answering (KBQA) system. The rise of LLMs makes it possible to perform such downstream tasks without access to external knowledge, e.g., closed-book QA. For instance, BERT has been proven to do remarkably well on open-domain QA~\cite{KGLM1}. Some literature shows that such LLMs can further improve their performances on open-domain QA after fine-tuning~\cite{LMQA}. 

\subsection{Differences}\label{sec:5.2}
To demonstrate the differences between LLMs and KGs, we discuss the limitations of KGs concerning LLMs and the current limitations of LLMs relative to the capabilities of KGs, separately. We conclude the limitations of KGs as follows,
\begin{itemize}
    \item \textbf{High construction cost:} The construction of knowledge graphs requires complex NLP techniques to process the text and quality testing to ensure the accuracy of the knowledge. Thus, the construction and maintenance of a large-scale KG often need significant human effort.
    \item \textbf{Data Sparsity:} Due to the high labor cost, the domain and data volume covered by a KG are limited, which leads to a large amount of missing data in the KG.
    \item \textbf{Lack of flexibility:} The storage structure and query method of a KG are relatively fixed, and it is difficult to adapt to various data structures and query requirements. By contrast, LLMs can offer better extendability and expressibility to different kinds of downstream tasks and thus have a broader range of application scenarios.
\end{itemize}

Although LLMs demonstrate superior reasoning capabilities and versatility over KGs, there are still some obvious limitations of LLMs that can be addressed by combining them with different types of KGs,
\begin{itemize}
    \item \textbf{LLM vs SKG:} LLMs are black-box models in nature. It is difficult to know the basis of the answers given by an LLM and the corresponding reasoning process. Meanwhile, one of the main advantages of KGs is their \textbf{explainability}. It would be easier to know how the answers are inferred over a KG. Moreover, regardless of knowledge updating and revision, an SKG will give a consistent answer to a query no matter how many times this query is performed. By contrast, LLMs might show different answers to the same question due to their \textbf{randomness} and the nature of probabilistic models. And the training corpus used for LLM might be noisy. The training processes of LLMs have the risk of learning incorrect or toxic knowledge~\cite{LMdanger}, while the \textbf{reliability of knowledge} is ensured by quality assessment for a KG, especially for small-scale domain-specific KGs.
    \item \textbf{LLM vs DKG:} LLMs might suffer from \textbf{outdated knowledge and information} since they are pre-trained based on Internet data at a specific time. And LLMs have \textbf{limited editability}, that is to say, it is difficult for LLMs to frequently learn new knowledge and information due to their \textbf{unaffordable training cost}. For example, the largest GPT3 model~\cite{gpt3} has a parametric count of 175B and costs 10 million dollars for a single training session. By contrast, it is much easier for DKGs to revise and update the knowledge they have stored. Thus, the cost of knowledge updating will be significantly reduced for LLMs if LLMs and DKGs can be effectively combined without expensive training processes.
    \item \textbf{LLM vs TKG:} LLMs face three main challenges when dealing with temporal information~\cite{TKGLM}. The first challenge is \textbf{averaging}, i.e., the model may see conflicting information about time ranges. The second challenge is \textbf{forgetting}, where the model may not remember facts that are valid only for a representative period of time, and therefore performs poorly when asked questions about the more distant past. The third challenge is \textbf{poor temporal calibration}, i.e., as LLMs become "stale", they are increasingly likely to be queried for facts that are outside the time range of their training data. Relatively, TKGs tend to have longer time scopes and the factual knowledge in TKGs is much more time-sensitive.
    \item \textbf{LLM vs EKG:} LLMs have achieved noticeable success on many NLP tasks, but they still struggle for event-centric tasks. One of the main disadvantages of LLMs on learning event-centric knowledge is that they may not be able to capture the temporal relations between events effectively. This is because LLMs are trained on large text corpora via self-supervised learning methods and may not have access to structured data that can help them learn about \textbf{event temporal relations}~\cite{econet}. Moreover, event-centric knowledge is updated very quickly, and it is difficult for LLMs to learn from the constant addition of new event-centric knowledge.
\end{itemize}   

In addition to their respective limitations, KGs and LLMs have different representation forms to store knowledge, and different ways of performing knowledge reasoning. And although LLMs obtain decent knowledge probing performances on LAMA, some follow-up works propose more difficult and domain-specific probing datasets~\cite{BioLAMA,MedLAMA} for LLMs and demonstrate that current LLMs are not reliable in factual knowledge extraction~\cite{KGLM3, EBERT}, which is contrary to the perspective that LLMs can be seen as knowledge bases. Therefore, we believe that it is very necessary to address the existing limitations of LLMs to combine LLMs with different types of KGs.

% \begin{figure*}[t]
% \centering
% \includegraphics[width=15cm]{img/kg4llm.pdf} 
% \caption{Illustration of three categories of KG-augmented LLMs.}
% \label{fig:kg4llm}
% \end{figure*}


% \begin{table*}[t]
% \begin{center}
% \caption{Existing combinations of LLMs and KGs, related learning tasks, and specific task description, as well as representative methods.}\label{table:LLM&KG}
% \begin{tabular}{l|p{4.5cm}|p{5.45cm}|p{1.3cm}|p{3.1cm}}
% \toprule
%  Combinations & Tasks & Descriptions & KG Type& Representative Methods\cr 
% \midrule
%  \multirow{12}{*}{LLM for KG}& Knowledge Extraction & Input text to LLMs and recognize entities, relations and events within text& All Types & \cite{bert_NER,ANL_NER}\cr
%  \cmidrule{2-5}
%  & Knowledge Reasoning &Perform reasoning by inputting textual sequences generated from triples or triple paths to LLMs&SKG\&DKG & KBERT\cite{KBERT}, StAR\cite{StAR},  BERTRL\cite{BERTRL}, KG-BERT\cite{KG-BERT}, Bi-Link\cite{Bi-Link}\cr
%   \cmidrule{2-5}
%   & Entity Typing &Classify entity mentions extracted from text using LLM-base sequence labeling models &All Types & LME~\cite{entitytype1}, $\quad\quad\quad\quad\quad$ MLMET~\cite{entitytype2}\cr
%  \cmidrule{2-5}
%  & Entity Linking &Link the entity mentions extracted from text to the entities on KGs using LLM-based sequence labeling models&All Types & GENRE\cite{entitylink1}, $\quad\quad\quad\quad$ EPGEL~\cite{entitylink2}\cr
%  \cmidrule{2-5}
%   & Entity Alignment &Find entity pairs with similar literal information using LLMs &All Types & BERT-INT~\cite{BERTINT}\cr
%    \cmidrule{2-5}
% & Quality Assessment &Use LLMs to determine the correctness of  textual sequences generated from triples&All Types & KGRepair\cite{arnaout2022utilizing}\cr
%  \midrule
%  \multirow{6}{*}{KG for LLM}& Knowledge-Enhanced LLM &Enrich input text of LLMs with background knowledge from KGs &SKG &KALM\cite{KALM}, LUKE\cite{LUKE}, EBERT\cite{EBERT}\cr
%  \cmidrule{2-5}
% & Knowledge-Encoded LLM &Adapt the architecture of LLMs to encode structured knowledge from KGs &SKG &ERNIE\cite{ERINE}, Knowbert\cite{Knowbert}, K-Adapter\cite{K-Adapter}\cr
%  \cmidrule{2-5}
%  & Knowledge Task-based LLM &Use knowledge-constrained pretraining tasks to optimize LLMs &SKG &ERNIE3\cite{Ernie3}, KEPLER\cite{KEPLER}, K-PLUG\cite{-k-plug}\cr
%  % \cmidrule{2-5}
%  % & TKG/EKG-augmented LLM & Force LLMs to learn temporal knowledge and event-centric knowledge from TKGs and EKGs &TKG\&EKG &To be explored\cr
%  % \cmidrule{2-5}
%  %  & KG-augmented Prompt Learning &Retrieve factual knowledge related to the input text of LLMs from KGs and generate textual knowledge prompts &All Types &To be explored\cr
%  % \cmidrule{2-5}
%  %  & KG-based Hallucination Measuring & Measure the hallucination of LLM-generated texts based on relevant factual knowledge from KGs &All Types &To be explored\cr
%  \bottomrule
% \end{tabular}
% \end{center}
% \end{table*}

% \subsection{Existing Combinations of KG and LLM}
% \subsubsection{LLM for KG}
% In the early stage, the construction of KGs mainly relied on manual work and used to be very costly. With the development of AI technology, the automated KG construction technology based on deep learning has been widely used. However, most KGs still suffer from data sparsity, and their data quality needs to be improved. LLMs recently have shown to be an effective tool to extract, fuse and process structured knowledge due to their powerful capabilities of text processing and semantic expression.

% In the previous sections, we have discussed in detail the application of LLMs to various tasks of knowledge extraction and reasoning, including NER, relation extraction, event extraction, SKGR, and DKGR. As for knowledge extraction, LLMs can assist in extracting entities, relations and events from text by learning semantic representations of words and contextual associations between them. On the other hand, the rich semantic information of entities and the contextual relationships between entities contained in LLMs can be used to enhance the performance of the KGR model as a complement to the structured information of KGs.

% In addition to knowledge extraction and knowledge reasoning, LLMs are also used in other important parts of the KG construction process, such as entity typing, entity linking, entity alignment and quality assessment. For example,  LME~\cite{entitytype1} and MLMET~\cite{entitytype2} have shown that LLMs can be used to perform the task of entity typing by leveraging literal information of context sentences and type labels. GENRE~\cite{entitylink1} and EPGEL~\cite{entitylink2} use BART-based sequence-to-sequence models to link the entity mentions extracted from text to the entities on KGs. BERT-INT~\cite{BERTINT} is a neural entity alignment method, which leverage the literal information of entities, especially entity names, entity descriptions and attributes, with a BERT-based interaction model to match equivalent entities across different KGs. Other works~\cite{arnaout2022utilizing} have looked into how to use LLMs to detect incorrect triples and replace them with likely correct ones for the assessment and improvement of the quality of the KG. In summary, a lot of studies have been done on using LLMs to support KG curation. While LLMs have stronger multi-tasking capability and greater versatility, fully automated knowledge extraction, knowledge fusion, knowledge update and knowledge inference for KGs using LLMs will greatly reduce the cost of KG construction.


% \subsubsection{KG for LLM}
% Although LLMs can learn generic knowledge from massive texts, they still have disadvantages such as unreliablity of knowledge, and lack of interpretability. The introduction of structured knowledge from KGs can effectively alleviate these deficiencies. Motivated by this, KG-augmented LLMs have been born. Fusing LLMs and KGs allows KG-augmented LLMs to combine generic semantic knowledge, common sense knowledge, factual knowledge, and domain knowledge, which enable effective response to downstream knowledge-driven tasks. 

% As neural networks, LLMs consist of three kinds of network layers: the input layer, the hidden layer and the output layer. Based on this structure, the existing KG-augmented LLMs can be classified into three main categories: knowledge-enhanced LLMs, knowledge-encoded LLMs, and knowledge task-based LLMs, as shown in Figure~\ref{fig:kg4llm}. Different types of KG-augmented LLMs embed knowledge into different network layers.

% \textbf{Knowledge-Enhanced LLMs:} Knowledge-enhanced LLMs aims to enrich contextual information with background knowledge from KGs as supplementary input to help the model better understand the text. Such LLMs can be further divided into two sub-categories. The first category directly converts structured knowledge into text form to construct new training corpus~\cite{ye2019align} or concatenate it into existing text~\cite{KBERT,colake}. Another class of knowledge-enhanced LLMs represent entities and relationships in a KG as vectors and combines them with the text embeddings corresponding to the input text. Specific combinations include concatenating or adding entity embeddings with text embeddings~\cite{EBERT,LUKE,KALM}, concatenating entity type embeddings~\cite{KALM2}, special marker embeddings or positional embeddings with text embeddings~\cite{OAG-BERT}, etc.

% \textbf{Knowledge-Encoded LLMs:} Knowledge-encoded LLMs adapt the architecture of the transformer layers of the LLMs so that they have the ability to encode and integrate effective features of both text corpus and structured knowledge. There are three ways to encode structured knowledge into the transformer layers of LLMs, i.e., adding external knowledge encoding modules, modifying original encoding modules, and using standalone neural adapters. By connecting the output of the transformer layers to an external knowledge encoding module, some knowledge-encoded LLMs can encode both text and structured knowledge, and output a feature representation that incorporates valid information from both~\cite{ERINE,CokeBERT,BERT-MK,Ernie3}. There is also a part of LLMs that directly modify the internal structure of the Transformer layers so that they have the ability to handle structured knowledge. Specific modifications include inserting additional knowledge encoding module at specific locations in the middle layers~\cite{Knowbert}, and adapting the Transformer's original encoding mechanism to structured knowledge~\cite{KBERT,colake}. Other knowledge-encoded LLMs use neural adapters that store specific knowledge to encode knowledge from different resources. These adapters are plug-and-play and can operate independently from the LLMs~\cite{K-Adapter,lauscher-etal-2020-common}.

% \textbf{Knowledge Task-based LLMs:} A large amount of recent works have attempted to use knowledge-constrained pre-training tasks and push LLMs to learn more knowledge by completing these tasks during the pre-training process. There are two main types of such knowledge-constrained tasks, namely, knowledge masking tasks and knowledge representation tasks. The knowledge masking task uses various types of knowledge to develop a masking strategy and select masking targets, thus forcing LLMs to have specific knowledge in order to accurately predict what is to be masked~\cite{ERINE,-k-plug,CorefBert,Ernie3}.  The knowledge representation task attempts to combine the learning process of knowledge representation with the training process of LLMs. By establishing a connection between text and structured knowledge and setting up a joint multi-task training mechanism for both knowledge representation learning and language representation learning, it is possible to train the model parameters while learning the knowledge representation~\cite{KEPLER,jaket,eae,fae,mtb,erica,KG-BERT}.

% A KG-augmented LLM can use more than one ways to integrate structured knowledge into the LLM. For example, ERNIE3.0~\cite{Ernie3} adds a knowledge encoding module on top of the original encoding layers, and proposes a pre-training framework in which the language representation module and the knowledge task module run collaboratively, and thus can be considered as both a knowledge-encoded LLM and a knowledge task-based LLM.

% KG-augmented LLMs are equipped with enhanced semantic understanding by learning knowledge from SKGs. 
% However, the way they learn knowledge is still to update the large-scale neural networks, which is very costly and unexplainable. Since most of KG-augmented LLMs need to be retrained to update the knowledge they have learned when real-world knowledge changes, they still suffer from the issues of unreliable knowledge, limited editability and low explainability. Moreover, both LLMs and SKGs have limitations in understanding time information and event information. It is necessary to go into new approaches with can more effectively combine different types of KGs with LLMs.










